Advancing Robot Autonomy for Long-Horizon Tasks

Autonomous robots have real-world applications in diverse fields, such as mobile manipulation and environmental exploration, and many such tasks benefit from a hands-off approach in terms of human user involvement over a long task horizon. However, the level of autonomy achievable by a deployment is limited in part by the problem definition or task specification required by the system. Task specifications often require technical, low-level information that is unintuitive to describe and may result in generic solutions, burdening the user technically both before and after task completion. In this thesis, we aim to advance task specification abstraction toward the goal of increasing robot autonomy in real-world scenarios. We do so by tackling problems that address several different angles of this goal. First, we develop a way for the automatic discovery of optimal transition points between subtasks in the context of constrained mobile manipulation, removing the need for the human to hand-specify these in the task specification. We further propose a way to automatically describe constraints on robot motion by using demonstrated data as opposed to manually-defined constraints. Then, within the context of environmental exploration, we propose a flexible task specification framework, requiring just a set of quantiles of interest from the user that allows the robot to directly suggest locations in the environment for the user to study. We next systematically study the effect of including a robot team in the task specification and show that multirobot teams have the ability to improve performance under certain specification conditions, including enabling inter-robot communication. Finally, we propose methods for a communication protocol that autonomously selects useful but limited information to share with the other robots.

==> comms.tex <==
% abstract
% We find that multirobot teams improve performance in this task over single robots, and communication-enabled teams further over communication-deprived teams;
% however, real robots are resource-constrained, and communication networks cannot support arbitrary message loads, making na\"ive, constant information-sharing but also complex modeling and decision-making infeasible.
% With this in mind, we propose online, locally computable metrics for determining the utility of transmitting a given message to the other team members and a decision-theoretic approach that chooses to transmit only the most useful messages, using a decentralized and independent framework for maintaining beliefs of other teammates.
% We validate our approach in simulation on a real-world aquatic dataset, 
% and show that restricting communication via a utility estimation method based on the expected impact of a message on future teammate behavior results in a 42\% decrease in network load while simultaneously decreasing quantile estimation error by 1.84\%.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
\label{sec:intro}
Quantile estimation is useful for gaining an understanding of natural environments~\cite{rayas2022informative}, and the use of multirobot teams has shown promise for effectively planning exploration and accurately estimating the quantile values~\cite{rayas2023study}.
% We are interested in using a team of communication-enabled mobile robots to collaboratively explore a natural environment such that we achieve an accurate estimate of quantile values in that environment.
However, realistic multirobot deployments must consider limitations in communication capabilities; here, we focus on reducing the network load as measured by the number of attempted transmitted messages with the goal of sacrificing minimal quantile estimation accuracy. 
We address the question of how to decide whether a message is worth sending.
Specifically, we:
\begin{itemize}
    \item Propose methods to reduce network load for bandwidth- and resource-constrained decentralized multirobot teams that leverage utility-based message evaluation, with no guarantees on information from teammates;
    \item Describe a decision-theoretic approach to choosing whether to transmit a message to the network based on the utility-based evaluation and a cost of transmission;
    \item Present results showing significant reductions in network load are achievable with minor corresponding drops in performance on the problem task of estimating quantile values, even with probabilistic transmission failure and a distance-based transmission probability, on a dataset from a real aquatic environment;
    \item Discuss results in the context of real-world applications.
\end{itemize}

%we make several assumptions.
% First, we assume the robots are given the same task (set of quantiles) and operate in a cooperative manner in the same environment.
We assume a decentralized team -- each robot plans independently and is not guaranteed to receive information from  others.
However, we assume a communication protocol such that a robot can, at each step, decide to broadcast its newly acquired measurements to the network. 
The network has limited bandwidth, so robots are incentivized to only send those that will be most beneficial to the others.
We encode the cost of loading the network with a message through a threshold value, where utilities higher than the threshold have a higher benefit than cost.
With these assumptions in place, the question of how to evaluate a potential message for its utility emerges as a key consideration to this problem; in this work, we propose several approaches to solve this problem.

\section{Background}
There is extensive literature in utility-based
communication, and our methods share similarities with previously proposed
approaches (see \Cref{ssec:multirobot-comms-background}).
% specifically, we employ techniques using the difference of expected reward as well as the expected effect on robot actions in this work to model information utility.
In particular, some other works have
made use of a measure of utility based on expected reward or expected effect on robot actions, and the teams are
decentralized in terms of planning and reward calculation \cite{marcotte2020optimizing,unhelkar2016contact}. 
While our work in this chapter employs these as well, a major difference is
that our end goal is to explore the environment in whatever way results in the
best quantile estimates, while those works define a static goal location for the robots to reach. 
We also exclusively choose to plan using a
greedy algorithm for computational efficiency and tractability as opposed to using MDPs, motivated by
resource-constrained systems, and do not forward-simulate the models of other
robots while~\cite{marcotte2020optimizing} does. 
Significantly, we make the (more realistic)
assumption of stochastic communication on top of the communication decision; just because a robot decides to send a message does not guarantee
reception by all or any of the recipients. We further do not assume perfect measurement sensing. 
Despite our relatively simple planning and modeling methods and more
failure-prone communication assumptions, we are able to achieve a significant
decrease in network loading while maintaining reasonable, and in some case improving, task performance.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Methods}
\label{sec:methods}

Our formulation extends the setup used in the previous \Cref{ch:quantiles,ch:multirobot}; we briefly mention relevant definitions here. 
%
The team consists of $\nrobots$ aerial robots, each operating with a fixed planning budget $B_T$ at a fixed height in a discretized environment
$\gtlocations \subset
\mathbb{R}^2$. 
Robots can take one of four possible actions at each step: $\pm x$ or $\pm y$.
Since our focus is on inter-robot communications, we assume a low-level controller, a collision avoidance routine, and perfect localization.
The human operator supplies a set of arbitrary quantiles of interest $\quantiles$, and the end goal is to produce accurate estimates $\estimatedquantilevalues$ of $\quantiles$ where the true values are
defined as $\quantilevalues = \textit{quantiles}(\gtsensedvalues,\quantiles)$, 
the set of all possible locations a robot can measure with its sensor are $\gtsensedlocations$, and 
 the corresponding true values at those locations are $\gtsensedvalues$.
Each robot has a camera with which it can take noisy measurements $\sensedvalues$ representing the concentration of algae at those pixel locations in the environment $\sensedlocations$.
Throughout the deployment, each robot collects measurements $\sensedlocations, \sensedvalues$ both firsthand via its camera and via any messages received from others through the network.
The robots use all their collected measurements to construct and update their internal Gaussian process (GP) model of the environment.
%
% We define $(\sensedlocations_{0:t}, \sensedvalues_{0:t})$ as the measured locations and values collected by $n$ up to time $t$, which are used to condition $GP^n$. 
% Adding a new  to any robot model results in an updated GP of the environment, which can be used both
% to predict the value $\mu^{(n)}_{GP}(\sensedlocation)$ at arbitrary locations in the environment $\sensedlocation$ as well as
% to hypothesize the utility of including that $(\sensedlocations, \sensedvalues)$ in another robot's GP.
Robot $\ego$'s estimate of the quantile values 
% at time $t$  % removing the dependency on time for clarity
is given by
\begin{equation}
    \estimatedquantilevalues_{\ego} = quantiles(\mu_{GP^{\ego}}(\gtsensedlocations),\quantiles)
\end{equation}
where $\mu_{GP^{\ego}}(\gtsensedlocations)$ is the estimate of all possible locations
using the GP conditioned on the measurements $\sensedlocations^{\ego}$ and $\sensedvalues^{\ego}$ that $\ego$ has collected thus far.

%We would like to pause for a moment to clarify our notation.
% to clarify how the approach will be described. 
In what follows, when viewing the problem from the perspective of a given robot, we will refer to it as $\ego$ or the ego robot and to any of the other $\nrobots$ as $\other$. 
Variables superscripted with $\other$ such as $GP^{\other}$ indicate the GP for $\other$ \textit{from the perspective of $\ego$}.

Motivated by the computational constraints of resource-constrained systems, we opt to use a locally computable, online, greedy planning policy.
At each planning step $t$, $\ego$ maximizes an objective function $\objectivefunction$ over feasible next measurement locations.
We use a modified version of the quantile standard error objective function
to evaluate a proposed location for time $t$
proposed in \Cref{ch:quantiles},
which measures the difference in the standard error of the estimated quantile values using 
two versions of the robot model: the current model $\mu_{GP^{\ego}_{t-1}}$, and the model updated with the hypothetical new values at the proposed locations $\mu_{GP^{\ego}_{t}}$.
 % which is the same model but updated with an additional set of data points.
We modify $\objectivefunction$ such that it is conditioned not only on the proposed measurement locations $\sensedlocations$, but also the values associated with the locations (denoted by $\newobjectivevalues$ generally) and the GP to be used.
The reasoning is that $\objectivefunction$ is also used later in the process for computing message utilities, and this allows it to generalize to these cases when $\newobjectivevalues$ and $GP$ may take on different values.
% Depending on how this objective is used, the values $\newobjectivevalues$ will differ.
When $\objectivefunction$ is used in the planning step by $\ego$ to select $\ego$'s next location, $\newobjectivevalues$ are the expected values at the proposed location $\sensedlocations$: $\mu_{GP^{\ego}_{t-1}}(\sensedlocations)$ (just like in \cite{rayas2022informative}).
However, when $\objectivefunction$ is used by $\ego$ to determine the utility of $\other$ receiving a real measurement that $\ego$ has already acquired, $\newobjectivevalues$ are those $\sensedvalues$, and the GP may be either $GP^{\ego}$ or $GP^{\other}$ (see \Cref{ssec:modeling}).
The final term encourages exploration of high-variance areas.
\begin{equation}
\label{eq:objective}
    \objectivefunction(\sensedlocations_i; \newobjectivevalues, GP) =
\frac{d}{\numtiles} +
\sum_{\sensedlocation_j \in \sensedlocations_i} c\sigma^2(\sensedlocation_j)
\end{equation}
\begin{equation}
    d =
\|se(\mu_{GP_{i-1}}(\gtsensedlocations),\quantiles) -
se(\mu_{GP_{i}}(\gtsensedlocations),\quantiles) \|_{1}
\end{equation}

\subsection{Summary of Process}
\label{ssec:procedure}
The approach consists of 3 phases: Initialization, Exploration, and Aggregation.
These are described at a high level here; further details are in the sections following.

\subsubsection{Initialization}
\label{sssec:procedure-init}
Robots begin distributed in the environment according to the initial location spread $\spread$ (\Cref{ssec:alpha-expt} provides details). \imr{double check this reference} 
We assume each robot is given the number of other robots and their corresponding starting locations.

\subsubsection{Exploration}
\label{sssec:procedure-explore}
The bulk of the work happens during the decentralized exploration phase, where robots repeatedly choose the next location to visit, measure the environment, optionally broadcast the measurement in a message, and update their models until their budget $B_T$ is exhausted. The next measurement locations at $t$ are selected according to
\begin{equation}
\label{eq:greedy-planning}
    \sensedlocations^{\ego}_t = \argmax_{\sensedlocations \subset \sensedlocations^{\ego}_{\textrm{next}}} \objectivefunction (\sensedlocations;  \mu_{GP^{\ego}}(\sensedlocations), GP^{\ego})
\end{equation}
where $\sensedlocations_{\textrm{next}}$ contains the sets of locations that could be sensed one step from the current location, $\location^{\ego}_t$.
On top of this planning cycle, $\ego$ may receive a message from another $\other$ at any point, leading to further model updates (\Cref{ssec:modeling}).

\subsubsection{Aggregation}
\label{sssec:procedure-aggregate}
Once the robots have reached the allotted budgets, their data is collected. The operator can produce an aggregate GP model of the environment offline using it and, with that, obtain final estimates of quantile values:
\begin{equation}
\label{eq:final-qest}
    \estimatedquantilevaluesfinal = quantiles(\mu_{GP_\textrm{aggregate}}(\gtsensedlocations),\quantiles)
\end{equation}

\subsection{Communication Framework}
\label{ssec:comms}
The communication network consists of $\nrobots$ robots, each with the ability to broadcast a message at each step in its path. 
A message $\msg_t^{\ego} = (\ego, \location^{\ego}_t, \sensedlocations^{\ego}_t, \sensedvalues^{\ego}_t)$ sent by $\ego$ at time $t$ is composed of a header containing the sending robot's ID number and current location, and a body containing the current set of measurements. 
Messages are transmitted successfully to every other robot $\other$ in the network subject to the probability 
depending on distance and parameterized by the dropoff rate $\eta$ and communication radius $r$ \cite{rayas2023study}:
\begin{equation}
\label{eq:comms-probability}
    \successprob(distance) = \frac{1}{1 + e^{\eta (distance - r)}}
\end{equation}
and a successfully transmitted message will be received whole, uncorrupted, and without delay. 
In general, we assume $\ego$ does not receive a handshake or confirmation of whether its message was received successfully or not by $\other$.
We assume that robots can self-localize and that, within the radius $r$, they can accurately sense $\location^{\other}$, which they do at each step. 

\subsection{Modeling Others and Updating Models}
\label{ssec:modeling}
A central consideration is how to model other robots using incomplete information since such a model is necessary to adequately assess the utility any given message will have for others. 
%
The ego robot $\ego$ maintains a separate model $(\location^{\other},~ GP^{\other})$ for each $\other$. 
$\location^{\other}$ is the most up-to-date location $\ego$ has, and is updated in two cases.
First, by $\ego$'s sensing capabilities at each step if $\other$ is within radius $r$, 
and second, anytime $\ego$ receives a message from $\other$, via the header.
$GP^{\other}$ is a GP based on the measurements $\ego$ believes $\other$ has.
We denote this set of measurements as $\othermeasurements := (\sensedlocations^{\other}, \sensedvalues^{\other})$.
% $(\sensedlocations, \sensedvalues) \in \othermeasurements$ is a set of individual measurements (in the case of a camera sensor, pixel locations and values) taken from one location in the environment. 
%
$\othermeasurements$, and $GP^{\other}$, which is defined by it, can also be updated in two scenarios.
The first is when $\ego$ receives a message $\msg$ from $\other$, since it is clear that $\other$ must possess the data contained.
The second is more uncertain. If $\ego$ broadcasts $\msg$ to the network, it does not know whether it was successfully transmitted to any $\other$; however, recall that $\ego$ can sense the location of $\other$ within $r$. We use this to determine a proxy for reasonable confidence of transmission success: If $\other$ is within $r$, $\ego$ believes $\msg$ was received and thus updates $\othermeasurements$.%
% with the measurements in $\msg$.

\subsection{Computing Message Utility}
\label{ssec:utility}
We introduce several methods for computing the utility $\utility^{\other}$ of $\msg^{\ego} = (\ego, \location^{\ego}, \sensedlocations, \sensedvalues)$ (dropping the super- and subscripts for readability). 
The first,
\textit{Reward}, defines $\utility_{rw}$ as the reward $\ego$ believes $\other$ would receive, using the objective function $\objectivefunction$:
\begin{equation}
    \utility_{rw}(\sensedlocations, \sensedvalues, \other) = 
    \begin{cases}
      \infty, & \text{if} \quad | \sensedlocations^{\other} | = 0\\
      \objectivefunction(\sensedlocations ; \sensedvalues, GP^{\other}), & \text{otherwise}
    \end{cases}
\end{equation}

We call the second method \textit{Action}. Intuitively, it considers a message utile if $\ego$ believes that adding it to $GP^{\other}$ would result in $\other$ taking a different action than it would without those measurements. 
% Specifically, it considers the actions $\other$ would take when planning with $GP^o$ and with $GP^o$ conditioned on $\sensedlocations, \sensedvalues$. 
Then $\utility_{ac}$ is defined as $\infty$ if the actions $\sensedlocations_{\textrm{next,w/o}}$ and $\sensedlocations_{\textrm{next,w/}}$ differ as computed using \Cref{eq:greedy-planning}, and if they do not, $\utility_{ac}$ takes the value of $\utility_{rw}$:
\begin{equation}
    \utility_{ac}(\sensedlocations, \sensedvalues, \other) = 
    \begin{cases}
      \infty, & \text{if} ~ | \sensedlocations^{\other} | = 0\\
      \infty, & \text{if} ~ \sensedlocations_{\textrm{next,w/o}} \neq \sensedlocations_{\textrm{next,w/}} \\
      \utility_{rw}(\sensedlocations, \sensedvalues , \other), & \text{otherwise}
    \end{cases}
\end{equation}
Both $\utility_{rw}$ and $\utility_{ac}$ include the caveat that, if $\ego$ believes $\other$ has collected no measurements yet, the message should be sent.

The last three methods presented are simpler in that they do not make use of the model of $\other$.
The third method, \textit{Ego-reward}, uses the reward $\ego$ received from its measurement:
\begin{equation}
    \utility_{ego}(\sensedlocations, \sensedvalues, \other) = 
     \objectivefunction(\sensedlocations, \sensedvalues ; GP^{\ego})
\end{equation}
Finally, \textit{Always} and \textit{Never} are constant baselines, which always assign either $\infty$ or $0$:
\begin{equation}
    \utility_{al}(\sensedlocations, \sensedvalues, \other) = 
     \infty
\end{equation}
\begin{equation}
    \utility_{nv}(\sensedlocations, \sensedvalues, \other) = 
     0
\end{equation}

\subsection{Deciding to Communicate}
With the utilities of a message $\{\utility^{\other}\}$ computed for each $\other$, $\ego$ now faces the problem of deciding whether the utility overcomes the cost of loading the network with a message. 
Since the communication is broadcast-based rather than point-to-point, $\ego$ must first compute a single utility value $\aggutility$ for the team and then determine if it crosses a utility threshold $\utilthresh$ representing the cost.
For this, we describe a method 
for aggregating a set of utilities 
which computes 
% a measure of 
\textit{expected utility}, weighting utilities by the estimated transmission success probability:
\begin{equation}
\label{eq:expected-utility}
    \aggutility_{EU}(\{\utility^{\other}\}) = \frac{1}{\nrobots - 1} \sum_{\other} (p_{est}(\other) \cdot \utility^{\other})
\end{equation}
\begin{equation}
\label{eq:estimated-success-probability}
    p_{est}(\other) = 
    \begin{cases}
      \successprob(d^{\other}), & \text{if} \quad d^{\other} \leq r \\
      \successprob(r), & \text{otherwise}
    \end{cases}
\end{equation}
where $d^{\other} = ||\location^{\ego} - \location^{\other}||_2$ and $r$ is as defined in \Cref{ssec:comms}.
The estimated success probability, computed in \Cref{eq:estimated-success-probability}, directly uses the probability based on the distance to $\other$ if it is known (i.e., if $\other$ is within the sensing radius $r$), but defaults to an optimistic probability estimate for any $\other$ that is beyond the sensing radius by using $r$ as the assumed distance.
This optimistic heuristic prevents overly restrictive utility values in the face of unknown teammate positions.
% The second method simply considers the \textit{Maximum}:
% \begin{equation}
%     \aggutility_{max} = \max (\{\utility^{\other}\})
% \end{equation}
%
Note that 
% for both, 
if any $\utility^{\other}$ is $\infty$, then $\aggutility$ is considered past the threshold $\utilthresh$.
If $\aggutility \geq \utilthresh$, $\ego$ decides to transmit $\msg$.%

% \begin{itemize}
%     \item GP updates with measurements r1 sends to r2 (within comms radius) and with measurements received from r2
%     \item Augmented: GP still updates as above, but augment the GP with hallucinated dataset with r1's current recorded quantile estimate from r2 (see below)
% \end{itemize}
% \subsubsection{Hallucinating dataset: Algorithm}
% \begin{itemize}
%     \item given: quantile estimates $\estimatedquantilevalues$, quantile SE estimates, and the number of measurements (M) r2 has.
%     \item m = r1's model of r2
%     \item if $M \leq |m.measurements|$, do not hallucinate data (return).
%     \item $M' = M - |m.measurements|$
%     \item construct 2 KDEs: one of the values in m ($kde_v$), one of the locations in m ($kde_l$).
%     \item sample $M'$ values from $kde_v$. This is the hallucinated dataset $H_v$
%     \item iteratively update $H_v$ via some optimization algorithm (simulated annealing in our case), where the acceptance criteria is $RMSE(quantiles(m.measurements \cup H_v), \estimatedquantilevalues) < RMSE(quantiles(m.measurements \cup H_v^{prev}), \estimatedquantilevalues)$
%     \item sample $M'$ locations from $kde_l$. These are the locations for the hallucinated dataset $H_l$ \imr{this isn't quite right}
%     \item query $H_l$ using m to get the values produced by the current model
%     \item sort $H_l$, ordered by query values
%     \item sort $H_v$
%     \item return $H_l, H_v$ as the hallucinated data
% \end{itemize}

\section{Experiments and Discussion}

\begin{table*}
  \begin{tabular}{c||cc|cc|c}
  % method | attmpted avg, std | % lt always | succeeded avg, std | % lt always | % lt always (RMSE)
    \textit{Method} & \textit{Attempted} & \textit{Median} & \textit{Successful} & \textit{Median} & \textit{Median} \\ 
     & \textit{($\mu, \sigma$)} & \textit{Decrease} & \textit{($\mu, \sigma$)} &  \textit{Decrease} &  \textit{RMSE Increase} \\ 
    \hline 
    %
    % These results are from averaging all trials and then comparing means (no pairing of trials)
% Action & (1.66, 1.49) & 44.5 & (0.96, 1.09) & 14.99 & -2.16 \\
% Always & (3.0, 0.0) & 0.0 & (1.12, 0.93) & 0.0 & 0.0 \\
% Ego-reward & (1.9, 1.44) & 36.5 & (0.86, 1.02) & 23.44 & -0.63 \\
% Never & (0.0, 0.0) & 100.0 & (0.0, 0.0) & 100.0 & -27.02 \\
% Reward & (1.7, 1.49) & 43.17 & (0.9, 1.04) & 19.88 & -4.65 \\
%
% These results are from pairing experiments together for %R columns, sorted by their parameters. Then numbers are over 3 possible attempts * 40 steps = 120 total. Still comparing means.
% Method & (att mu, att std) & \%R  & (succ mu, succ std) & \%R & RMSE \%R \\
% Action & (66.6, 27.95) & 44.5 & (38.2, 23.85) & -4.57 & -11.17 \\
% Always & (120.0, 0.0) & 0.0 & (44.93, 16.78) & 0.0 & 0.0 \\
% Ego-reward & (76.2, 28.33) & 36.5 & (34.4, 20.27) & 18.43 & -7.87 \\
% Never & (0.0, 0.0) & 100.0 & (0.0, 0.0) & 100.0 & -50.86 \\
% Reward & (68.2, 32.1) & 43.17 & (36.0, 22.77) & 14.88 & -16.28 \\
%
% These results are from pairing experiments together, but reporting median change. Reduction for Attempted and Successful, but Increase in RMSE.
Action & (66.6, 27.95) & 42.5\% & (38.2, 23.85) & 24.32\% & -1.84\% \\
Always & (120.0, 0.0) & -- & (44.93, 16.78) & -- & -- \\
Ego-reward & (76.2, 28.33) & 27.5\% & (34.4, 20.27) & 32.2\% & 5.96\% \\
Never & (0.0, 0.0) & 100.0\% & (0.0, 0.0) & 100.0 & 73.98\% \\
Reward & (68.2, 32.1) & 52.5\% & (36.0, 22.77) & 35.96\% & 16.03\% \\
  \end{tabular}
  \caption{
  Number of attempted and successful transmitted messages per utility method. 
  Restricting transmissions with Action results in more than $40\%$ reduction in network load (attempted) while improving mean final quantile estimation error  by $1.84\%$ and only resulting in a less than $25\%$ decrease in successful transmissions.
  Results reported from $60$ experiments total of length 40 steps.
  All experiments use $\nrobots=4$, so 
  the most messages possibly sent total is $40\times(\nrobots-1)=120$.
  }
  \label{tab:comms}
\end{table*}

\begin{figure}
  \centering
 \includegraphics[width=\columnwidth]{figures/comms_pct_boxplot/utility-methods-handshake.pdf}
  \caption{
  Tradeoff in network load vs. task performance for different utility methods, compared to always sending messages.
  Top: Percent decrease in messages sent (network load). Higher is better.
  Bottom: Percent increase in final quantile estimation error. Lower is better. 
  }
  \label{fig:comms-tradeoff}
\end{figure}

\begin{figure}
  \centering
 \includegraphics[width=\columnwidth]{figures/comms-pointplot/utility-methods-handshake-Handshake_False_cumulative.pdf}
  \caption{
  Cumulative network load, as measured by messages sent, over time. 
  Each step on the x-axis represents a robot taking a planning step. 
  }
  \label{fig:comms-cumulative}
\end{figure}

\begin{figure}
  \centering
  % this one includes Never (a blank plot)
 \includegraphics[width=\columnwidth]{figures/comms-pointplot/utility-methods-handshake-Handshake_False.pdf}
  \caption{
  Amount of attempted and successful transmissions over time for different utility methods.
  Each step on the x-axis represents a robot taking a planning step. 
  }
  \label{fig:comms}
\end{figure}

We now present experimental results for the methods described in \Cref{sec:methods}.
% For thresholding, we only use Expected Utility (excluding Maximum), as we found it experimentally to perform better. 
%
We test performance on 3 sets of quantiles $\quantiles$: Quartiles (0.25, 0.5, 0.75), Median-Extrema (0.5, 0.9, 0.99), and Extrema (0.9, 0.95, 0.99).
For each combination of parameters, we run 5 seeds, resulting in 60 total instances.
We fix the following parameters: $\nrobots = 4$; budget $B_T = 10$ ($40$ steps total); initial spread $\spread = 0.2$; $\eta = 0.4$; communication radius $r = 15.0$; thresholds $\utilthresh_{rw} = 2.8 \times 10^{-4}$ and $\utilthresh_{ego} = 8.3 \times 10^{-5}$.
$\utilthresh_{rw}$ is used for Reward and Action, while $\utilthresh_{ego}$ is used for Ego-reward.
We selected these $\utilthresh$ experimentally by observing the received $\utility$ values during testing and setting $\utilthresh$ to the approximate 25th percentile of observed rewards. 
This can be interpreted as only messages that are in the top 75\% of utility being worth the cost of sending to the network, while those in the lower quarter are not.

The robots operate in simulation using a real-world dataset collected with a hyperspectral camera mounted on a drone from a lake in California. The environment is roughly $80 \times 60$ meters, discretized to $\gtlocations = 25 \times 25$ locations. Each set of measurements is an image of $5 \times 5$ pixel intensities for the 400nm channel of the hyperspectral image, normalized to $[0,1]$. To each measurement, we add zero-mean Gaussian noise with a standard deviation $0.05$.%


\subsection{Utility Methods Comparison}
We investigate the effectiveness of the different methods on performance in terms of both the network load as well as the final error (RMSE) between the estimated quantile values $\estimatedquantilevaluesfinal$ and $\quantilevalues$.
%
\Cref{tab:comms} displays numerical results, including a comparison of each method to Always in terms of the median percent change of each reported metric. 
These results are shown graphically in \Cref{fig:comms-tradeoff}, illustrating the tradeoff between network load and task performance.
\Cref{fig:comms} shows the number of attempted and successful message transmissions plotted over time, while 
\Cref{fig:comms-cumulative} shows the cumulative network load as measured by the attempted transmissions over time.
\Cref{fig:rmse-utility} shows boxplots of the final RMSE for different utility methods.
%
\Cref{fig:rasters} illustrates example paths taken 
% for utility methods Action and Reward, 
superimposed on the hyperspectral image of the lake.


We observe in \Cref{fig:comms} that 
across all methods, successful transmissions generally decrease over time due to robots spreading out.
Comparing Never to the other methods in \Cref{fig:rmse-utility}, we can confirm our previous findings that inter-robot communication improves performance.
However, we are mainly interested in the effect of decreasing network load.

When we analyze results in \Cref{tab:comms} and \Cref{fig:comms-tradeoff}, we see that severe reductions in communication do not necessarily result in severe decreases in performance. 
We see that Action results in the best performance: 
Compared to Always, there is more than $40\%$ decrease in network load as measured by attempted message transmissions, but this translates to less than $25\%$ decrease in actual (successful) message transmissions. 
Most notably, in terms of final error, there is a $1.84\%$ decrease in mean RMSE, indicating that performance, on average, improves slightly even with restricted communication.

Other reward-based methods, Reward and Ego-reward, also perform favorably.
\Cref{fig:comms,fig:comms-cumulative} suggest that all three proposed methods have message transmission rates that generally decrease over time.
We speculate that this may be due to two reasons.
First, as robots explore more of the environment and receive more information from the others, their beliefs of their teammates will change such that $|\sensedlocations^{\other}|$ increases, leading to more accurate environment models and thus less value in receiving an additional set of measurements.
Second, with more exploration time, robots are more likely to be situated at further distances from each other. With distance, the expected utility will decrease according to the transmission probability, and even messages believed to be useful may not be deemed worthy because of their unlikelihood of successful delivery. 
We note, however, that the optimistic assumption in \Cref{eq:estimated-success-probability} will prevent a highly useful message from not being sent due to distance.

As shown qualitatively in \Cref{fig:comms,fig:comms-cumulative} and quantitatively in \Cref{tab:comms}, Action, Reward, and Ego-reward all have lower network load than Always, but their relative loads vary as do their final estimation error.
In particular, Reward results in the highest decrease in network load (excluding Never) at $52.5\%$, but also the largest increase in final error of more than $16\%$. 
Thus, such a metric may be valuable when network bandwidth is severely limited.
Ego-reward, on the other hand, has the smallest decrease in network load at $27.5\%$, but a relatively small increase in error at less than $6\%$. 
Ego-reward has the benefit of not requiring any onboard modeling of teammate beliefs; thus, this method could be powerful when onboard compute is limited. 
Action is the overall best performer, with a decrease in network load of $42.5\%$ and a decrease in final error of $1.84\%$. 
We suspect Action performs better because it directly considers the impact of a message on future behavior, leading to more informed and targeted measurement acquisition at the next step. 
We note that the comparison of relative network loads is more valuable here than the absolute value, as the threshold values used in \Cref{eq:expected-utility} are tunable parameters that should reflect actual network constraints in a real deployment.

\begin{figure}
  \centering
         \includegraphics[width=\columnwidth]{figures/boxplot/utility-methods-handshake-Handshake_False RMSE_by_Comms Utility Method.pdf}
  \caption{
  Final estimation error for different utility methods. 
  }
  \label{fig:rmse-utility}
  \end{figure}
     
\begin{figure}
         \centering
         \includegraphics[width=\columnwidth]{figures/boxplot/utility-methods-handshake_stats: Wilcoxon_greater_adjacent RMSE_by_Handshake.pdf}
  \caption{
  Right: the sender receives an oracle handshake
  when a message is successfully transmitted.
  Bar indicates significance under one-sided Wilcoxon signed-rank test; *: $\psig$.
  }
  \label{fig:handshake}
\end{figure}


%%%%%%
% Raster plots for visualizing an example
%%%%%%
\begin{figure}
  \centering
 %  % Quartiles, Action
 % \includegraphics[trim={0.5cm 3cm 0.5cm 3.5cm}, clip, width=\boxwidth]{figures/raster/all_utility-methods-handshake_EnvA_Quartiles_step40_a0.2_c2e-08_seed0_N4_radius15.0_Action_expected_utility_hallucinateFalse_handshakeFalse.pdf}
 %   %
 %  % Quartiles, Reward
 % \includegraphics[trim={0.5cm 3cm 0.5cm 3.5cm}, clip, width=\boxwidth]{figures/raster/all_utility-methods-handshake_EnvA_Quartiles_step40_a0.2_c2e-08_seed0_N4_radius15.0_Reward_expected_utility_hallucinateFalse_handshakeFalse.pdf}
  %
  % Extrema, Action
 \includegraphics[trim={0.5cm 3cm 0.5cm 3.5cm}, clip, width=\columnwidth]{figures/raster/all_utility-methods-handshake_EnvA_Extrema_step40_a0.2_c2e-08_seed0_N4_radius15.0_Action_expected_utility_hallucinateFalse_handshakeFalse.pdf}
  %
  % Extrema, Reward
 \includegraphics[trim={0.5cm 3cm 0.5cm 3.5cm}, clip, width=\columnwidth]{figures/raster/all_utility-methods-handshake_EnvA_Extrema_step40_a0.2_c2e-08_seed0_N4_radius15.0_Reward_expected_utility_hallucinateFalse_handshakeFalse.pdf}
  %
  \caption{
  Example paths using two different utility methods with $\quantiles$ = $(0.9, 0.95, 0.99)$.
  Top: Action. Bottom: Reward.
  % Top: $\quantiles$ = $(0.25, 0.5, 0.75)$.
  % Bottom: $\quantiles$ = $(0.9, 0.95, 0.99)$.
}
  \label{fig:rasters}
\end{figure}

\subsection{Oracle Handshaking}
We implement a modification to the communication protocol where we assume an oracle handshaking routine, which gives $\ego$ an accurate confirmation handshake from each $\other$ indicating whether the message was successfully received; $\ego$ then only updates $M^{\other}$ when successful, leading to likely more correct models.
\Cref{fig:handshake} shows the final RMSE comparing the two; we see that there is a significant improvement with oracle handshaking (Wilcoxon signed-rank test $\wpres{1143}{0.05}$).
Though practically impossible, this suggests that implementing such a (probabilistic) routine in the network could improve performance further; however, the resulting burden of these messages must also be taken into account.

% \begin{figure}
%     \vspace{-0.2in}
%   \centering
%  \includegraphics[width=0.4\textwidth,height=\boxheight]{figures/boxplot/utility-methods-handshake_stats: Wilcoxon_greater_adjacent RMSE_by_Handshake.pdf}
%   \caption{
%   Comparison against a baseline where the sender receives an oracle handshake.
%   % when a message is successfully transmitted
%   Bar above indicates significance under the one-sided Wilcoxon signed-rank test; *: $\psig$.
%   }
%   \label{fig:handshake}
%   % \vspace{-0.3in}
% \end{figure}

\section{Conclusion and Future Work}
In this chapter, 
we presented a study on restricted communication in the context of quantile estimation for environmental analysis.
We show that restricting message transmission based on whether the actions that the sender believes other robots will take at the next state would change with the message results in a $42\%$ decrease in network load while also decreasing quantile estimation error by $1.84\%$, when compared to transmitting every message possible.

Our analysis indicates that targeted communication during quantile estimation can have real benefits to real-world multirobot deployments when robots and their network are resource-constrained.
Importantly, these results allow users to relegate the task of deciding which messages to send to a network in an intelligent manner to the robots.

In addition to receipt handshaking, there are several interesting directions of future work.
First, we have chosen to implement robot planning using greedy action selection, but it would be valuable to extend this method to use a non-myopic planning strategy.
We also believe allowing the sender to choose the most valuable measurements from its collected data rather than restricting it to the most recent measurements may improve performance. 
However, this would lead to challenges in scalability as the environment is explored, and could be addressed by applying a rolling window over the previous measurements to mitigate this or by keeping and updating a limited set of high-utility measurements from which messages are selected.
Further, we are interested in methods for better approximating the models that a robot maintains for each of its teammates, which could be achieved by augmenting message headers with metadata such as that robot's current dataset size or current quantile estimates.
Finally, choosing the threshold value $\utilthresh$ is an important hyperparameter choice. It would be interesting and valuable to investigate ways in which this value could be automatically extracted or learned either offline or during exploration.


==> ecomann.tex <==
\section{Introduction}
Robots must be able to plan motions that follow various constraints in order for them to be useful in real-world environments.
Constraints such as holding an object, maintaining an orientation, or staying within a certain distance of an object of interest are just some examples of possible restrictions on a robot's motion.
In general, two approaches to many robotics problems can be described. One is the traditional approach of using handwritten models to
capture environments, physics, and other aspects of the problem mathematically or analytically, and then solving or optimizing these to find a solution. 
The other, popularized more recently, involves the use of machine learning to replace, enhance, or simplify these hand-built parts.
Both have challenges: Acquiring training data for learning can be difficult and expensive, while describing precise models analytically can range from tedious to impossible.
Here, we approach the problem from a machine learning perspective and propose a solution to learn constraints from demonstrations. The learned constraints can be used alongside analytical solutions within a motion planning framework.
%We are motivated to investigate methods for learning constraints from demonstrations in order to be used in a motion planning framework. 

%Constrained motion planning is an essential part to most practical robotic systems.
%Some constraints may be difficult to describe analytically, for example the task of pouring a liquid from a cup to a container. 
%For this reason, 
%Learning from demonstrations has the advantages of not requiring as much expert knowledge and of being simpler compared with generating simulated instances of complex constraints.

% talk about the methods we investigate
% \begin{itemize}
%     \item In this work, we investigate ways of learning constraint manifolds for planning from demonstrations of constrained tasks. 
%     \item Our work consists of two main threads, which we use within a motion planning framework
%     \item First, we propose a new learning-based method for describing kinematic motion constraints, called {\ecmnnlong} (\ecmnn). {\ecmnn} learns a function which evaluates a robot configuration on whether or not it meets the constraint. 
%     \item Second, we use a generative model called a variational autoencoder (VAE) to produce new configurations that meet the constraint.
% \end{itemize}
% Other methods: vector fields for control; penalty functions; extra state variables; motion constraint vectors C (mike stilman 2007); reachability graphs; constraint graphs
% explain that we choose to do this in a LfD manner
% \begin{itemize}
%     \item We use {\lfd} because generating training data in simulation may be infeasible for complex constraints
%     \item {\lfd} also doesn't require expert knowledge to encode constraints analytically.
% \end{itemize}
% explain how we use/evaluate our methods
% \begin{itemize}
%     \item We use a motion planning framework, SMP, to solve motion planning problems that are both constrained and sequential in nature
%     \item {\ecmnn} is used in SMP to evaluate sampled points.
%     \item The VAE is used in SMP to generate new points that meet the constraint.
% \end{itemize}

In this work, we propose a new learning-based method for describing motion constraints, called {\ecmnnlong} (\ecmnn). {\ecmnn} learns a function which evaluates a robot configuration on whether or not it meets the constraint, and for configurations near the constraint, on how far away it is. 
We train {\ecmnn} with datasets consisting of configurations that adhere to constraints, and show results for tasks learned from demonstrations of robot tasks. 
We use a sequential motion planning framework 
to solve motion planning problems that are both constrained and sequential in nature, 
and incorporate the learned manifolds into it. We evaluate the constraints learned by \mbox{\ecmnn} with various datasets on their representation quality. Further, we investigate the usability of learned constraints in sequential motion planning problems.

%===============================================================================
\subsection{Background}
The work described in this chapter combines ideas from many fields, including constrained sampling-based motion planning (SBMP), manifold learning, and learning from demonstrations, as described in \Cref{ch:motion-planning-background}.

As opposed to other constrained SBMP methods, our method differs in that {\ecmnn} learns an implicit description of a constraint manifold via a level set function, and during planning, we assume this representation for each task. We note that our method could be combined with others, e.g. learned sampling distributions, to further improve planning results.

Our work is related to many of the manifold learning approaches described in \cref{ssec:manifold-learning}; in particular, the tangent space alignment in LTSA is an idea that {\ecmnn} uses extensively. 
Similar to the ideas presented in this chapter, the work in \cite{osa2020learning} delineates an approach to solve motion planning problems by learning the solution manifold of an optimization problem. 
In contrast to others, our work focuses on learning implicit functions of equality constraint manifolds, which is a generalization of the learning representations of Signed Distance Fields (SDF) \cite{park2019deepsdf, mahler2015gp}, up to a scale, but for higher-dimensional manifolds.

Further, our work can be seen as a special case of inverse optimal control (IOC) where the task is only represented in form of constraints. Instead of using the extracted constraints in optimal control methods, we integrate them into 
%sequential 
sampling-based motion planning methods, which are not parameterized by time and do not suffer from poor initializations.

\subsection{Motion planning on manifolds}
\label{subsec:smp}
In this work, we aim to integrate learned constraint manifolds into 
the \smp framework from \Cref{ch:psm}, using the same problem formulation and notation as described in \Cref{sec:problem_formulation}.
% The motion planner considers kinematic motion planning problems in a configuration space $\configspace \subseteq \Re^{\dimambient}$. A robot configuration 
% % $q\in C$ 
% $\jointposition \in \configspace$
% describes the state of one or more robots with 
% % $k$ 
% $\dimambient$
% degrees of freedom in total.
% A manifold $\constraintmanifold$
% is represented as an equality constraint $\constraintfunction(\jointposition) = \vct{0}$.
% %where 
% % $h_{M}(q) : \R^{k} \to \R^{l}$. 
% %$\constraintfunction: \Re^{\dimambient} \rightarrow \Re^{\dimconstraint}$
% %and $\dimambient - \dimconstraint$ is the dimensionality of the implicit manifold.
% The set of robot configurations that are on a manifold $\constraintmanifold$ is given by 
% \mbox{$\onconstraintconfigspace = \{ \jointposition \in \configspace \mid \constraintfunction(\jointposition) = \vct{0}\}\period$}
% %
% %SMP defines the planning problem as a sequence of   % camera-ready
% The planning problem is defined as a sequence of
% $(\numconstraintmanifold+1)$
% such manifolds 
% \mbox{$\mathcal{\constraintmanifold} = \{\constraintmanifold_1, \constraintmanifold_2, \dots, \constraintmanifold_{\numconstraintmanifold+1}\}$}
% and an initial configuration 
% $\jointposition_\t{start} \in \configspace_{{\constraintmanifold}_1}$ 
% on the first manifold.
% The goal is to find a path from 
% $\jointposition_\t{start}$ 
% that traverses the manifold sequence 
% $\constraintmanifoldsequence$
% and reaches a configuration on the goal manifold 
% $\constraintmanifold_{\numconstraintmanifold+1}$. 
% A path on the $i$-th manifold is defined as 
% $\tpath_i : [0, 1] \to {\onconstraintconfigspace}_{i}$
% and 
% $\cost(\tpath_i)$ 
% is the cost function of a path
% $\costfunctional : \tpathspace \to \Re_{\geq 0}$
% where 
% $\tpathspace$ 
% is the set of all non-trivial paths. The problem is formulated as an optimization over a set of paths 
% $\tpathset = (\tpath_1, \dots, \tpath_{\numconstraintmanifold})$ 
% that minimizes the sum of path costs under the constraints of traversing 
% $\constraintmanifoldsequence$ \ref{eq:smp_problem}.
% % \begin{align} %
% % 	\begin{alignedat}{2} %	
% % 	\label{eq:smp_problem}
% % 	&\vct\tau^{\star} = \argmin_{\vct\tau} \sum_{i=1}^n J(\tau_i) &&\\
% % 	\st\quad &\tau_1 (0) = q_\t{start} &\\
% % 	&\tau_i(1) = \tau_{i+1}(0)  &&\forall_{i=1,\dots,n-1} \\ 
% % 	&C_{\t{free}, i+1} = \Upsilon(C_{\t{free}, i}, \tau_{i})~~~~ &&\forall_{i=1,\dots,n}\\
% % 	&\tau_i(s) \in C_{M_i} \cap C_{\t{free}, i} &&\forall_{i=1,\dots,n}~ \forall_{s \in [0, 1]}\\
% % 	&\tau_{n}(1) \in C_{M_{n+1}} \cap C_{\t{free}, n+1} &&
% % 	\end{alignedat} %
% % \end{align}
% %
% % \begin{align} %
% 	% \begin{alignedat}{2} %	
% 	% \label{eq:smp_problem}
% 	% &\tpathset^{\star} = \argmin_{\tpathset} \sum_{i=1}^{\numconstraintmanifold} \cost(\tpath_i) &&\\
% 	% \st\quad &{\tpath}_1 (0) = {\jointposition}_\t{start} &\\
% 	% &\tpath_i(1) = \tpath_{i+1}(0)  &&\forall_{i=1,\dots,\numconstraintmanifold-1} \\ 
% 	% &\configspace_{\t{free}, i+1} = \freeconfigspaceoperator(\configspace_{\t{free}, i}, \tpath_{i})~~~~ &&\forall_{i=1,\dots,\numconstraintmanifold}\\
% 	% &\tpath_i(s) \in {\onconstraintconfigspace}_{i} \cap \configspace_{\t{free}, i} &&\forall_{i=1,\dots,\numconstraintmanifold}~ \forall_{s \in [0, 1]}\\
% 	% &\tpath_{\numconstraintmanifold}(1) \in {\onconstraintconfigspace}_{\numconstraintmanifold+1} \cap \configspace_{\t{free}, \numconstraintmanifold+1} &&
% 	% \end{alignedat} %
% % \end{align}
% $\freeconfigspaceoperator$ is an operator that describes the change in the free
% configuration space (the space of all configurations that are not in collision
% with the environment)
% $\configspace_\t{free}$ 
% when transitioning to the next manifold. 
% %The SMP  % camera-ready
% This algorithm is able to solve this problem for a certain class of problems. It
% iteratively applies RRT${}^\star$ to find a path that reaches the next manifold
% while staying on the current manifold.
% %For further details of the SMP algorithm, we refer the reader to \citep{englert2020sampling}. 
%
We employ data-driven learning methods to learn individual
manifolds $M$ from demonstrations with the goal to integrate them with
analytically defined manifolds into this framework. 

%===============================================================================

\section{{\ecmnnlong} (\ecmnn)}
\label{ssec:ecmnn}

We propose a novel neural network structure, called \emph{\ecmnnlong} (\ecmnn),
which is a (global) equality constraint manifold learning representation that
enforces the alignment of the (local) tangent spaces and normal spaces with the
information extracted from the Local Principal Component Analysis (Local PCA)
\cite{Kambhatla_LocalPCA} of the data. 
{\ecmnn} takes a configuration $\jointposition$ as input and outputs the
prediction of the implicit function $\constraintfunction(\jointposition)$.
We train {\ecmnn} in a supervised manner, from demonstrations. 
One of the challenges is that the supervised training dataset is collected only
from demonstrations of data points which are on the equality constraint manifold
$\onconstraintconfigspace$, called the \emph{on-manifold} dataset.
Collecting both the on-manifold $\onconstraintconfigspace$ and off-manifold
$\offconstraintconfigspace = \{ \jointposition \in \configspace \mid
\constraintfunction(\jointposition) \neq \vct{0} \}$ datasets for supervised
training would be tedious because the implicit function $\constraintfunction$
values of points in $\offconstraintconfigspace$ are typically unknown and hard
to label, so this is a reasonable assumption.
We show that, though our approach is only given data on
$\onconstraintconfigspace$, it can still learn a useful and sufficient
representation of the manifold for use in planning.


\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{ecomann_figures/tangent_space_augmentation}
    \caption{A visualization of data augmentation along the 1D normal space of a
    point $\jointposition$ in 3D space. Here, purple points are the dataset,
    pink points are the $\numnearestneighbor$NN of $\jointposition$, and the
    dark red point is $\augjointposition$. $\jointposition$ is at the axes
    origin, and the green plane is the approximated tangent space at that
    point.}
    \label{fig:localpca}
\end{figure}
Our goal is to learn a single global representation of the constraint manifold $M$ in the form of a neural network. 
%A manifold can be defined as a collection of local neighborhoods which resemble Euclidean spaces (\citep{Lee00_IntroToSmoothManifolds}). 
%Therefore, a global representation of the manifold can be developed by constructing characterizations for its Euclidean-like local neighborhoods. 
Our approach leverages local information on the manifold in the form of the
tangent and normal spaces \cite{Deutsch2015_TensorVotingGraph}.
With regard to $\constraintfunction$, the tangent and normal spaces are
equivalent to the null and row space, respectively, of the Jacobian matrix 
$\constraintmanifoldjacobian(\acute{\jointposition}) = \left. \frac{\partial
\constraintfunction({\jointposition})}{\partial
{\jointposition}}\right|_{{\jointposition} = \acute{\jointposition}}$, 
and valid in a small neighborhood around the point $\acute{\jointposition}$.
%
Using on-manifold data, the local information of the manifold can be analyzed
using Local PCA. For each data point $\jointposition$ in the on-manifold
dataset, we establish a local neighborhood using $\numnearestneighbor$-nearest
neighbors ($\numnearestneighbor$NN) $\origKNN =
\{\nearestneighborjointposition_1, \nearestneighborjointposition_2, \dots,
\nearestneighborjointposition_\numnearestneighbor\}$, with $\numnearestneighbor
\geq \dimambient$. 
After a change of coordinates, $\jointposition$ becomes the origin of a new
local coordinate frame $\lpcacoordframe$, and the $\numnearestneighbor$NN
becomes $\recenteredKNN = \{\recenterednearestneighborjointposition_1,
\recenterednearestneighborjointposition_2, \dots,
\recenterednearestneighborjointposition_\numnearestneighbor\}$ with
$\recenterednearestneighborjointposition_\idxnearestneighbor =
\nearestneighborjointposition_\idxnearestneighbor - \jointposition$ for all
values of $\idxnearestneighbor$. Defining the matrix 
$\designmatrix = 
\begin{bmatrix} 
\recenterednearestneighborjointposition_1 & \recenterednearestneighborjointposition_2 & \hdots & \recenterednearestneighborjointposition_\numnearestneighbor \\
\end{bmatrix}\T \in \Re^{\numnearestneighbor \times \dimambient}
$, we can compute the covariance matrix $\samplecovariancematrix = \frac{1}{\numnearestneighbor-1} \designmatrix\T \designmatrix \in \Re^{\dimambient \times \dimambient}$.
The eigendecomposition of $\samplecovariancematrix = \covrighteigmat
\covdiagsingularvalues \covrighteigmat\T$ gives us the Local PCA. 
The matrix $\covrighteigmat$ contains the eigenvectors of
$\samplecovariancematrix$ as its columns in decreasing order w.r.t.\ the
corresponding eigenvalues in the diagonal matrix $\covdiagsingularvalues$. These
eigenvectors form the basis of the coordinate frame $\lpcacoordframe$.

This local coordinate frame $\lpcacoordframe$ is tightly related to the tangent
and normal spaces of the manifold at $\jointposition$. That is, the
$(\dimambient - \dimconstraint)$ eigenvectors corresponding to the $(\dimambient
- \dimconstraint)$ biggest eigenvalues of $\covdiagsingularvalues$ form a basis
of the tangent space, while the remaining $\dimconstraint$ eigenvectors form the
basis of the normal space. 
Furthermore, 
%due to the characteristics of the manifold from which the dataset was collected, 
the $\dimconstraint$ smallest eigenvalues of $\covdiagsingularvalues$ will be
close to zero, resulting in the $\dimconstraint$ eigenvectors associated with
them forming the basis of the null space of $\samplecovariancematrix$. On the
other hand, the remaining $(\dimambient - \dimconstraint)$ eigenvectors form the
basis of the row space of $\samplecovariancematrix$. 
We follow the same technique as \cite{Deutsch2015_TensorVotingGraph} for
automatically determining the number of constraints $\dimconstraint$ from data,
which is also the number of outputs of {\ecmnn}\footnote{Here we assume that the
intrinsic dimensionality of the manifold at each point remains constant.}. 
Suppose the eigenvalues of $\samplecovariancematrix$ are $\{\coveigval_1,
\coveigval_2, \dots, \coveigval_\dimambient\}$ (in decreasing order w.r.t.
magnitude). Then the number of constraints can be determined as $\dimconstraint
= \argmax{\left(\left[\coveigval_1 - \coveigval_2, \coveigval_2 - \coveigval_3,
\dots, \coveigval_{\dimambient-1} - \coveigval_{\dimambient}
\right]\right)}$.

We now present several methods to define and train \ecmnn, as follows:
%\subsection{Determination of the Number of Constraints}
%

\subsection{Alignment of local tangent and normal spaces}
%
{\ecmnn} aims to align the following:
\begin{enumerate}%[(a)]
    \item the null space of $\constraintmanifoldjacobian$ and the row space of
        $\samplecovariancematrix$ (which must be equivalent to the tangent space)
    \item the row space of $\constraintmanifoldjacobian$ and the null space of
        $\samplecovariancematrix$ (which must be equivalent to the normal space)
\end{enumerate}
for the local neighborhood of each point $\jointposition$ in the on-manifold dataset. 
Suppose the eigenvectors of $\samplecovariancematrix$ are $\{\coveigvec_1, \coveigvec_2, \dots, \coveigvec_\dimambient\}$ and the singular vectors of $\constraintmanifoldjacobian$ are $\{\constrjaceigvec_1, \constrjaceigvec_2, \dots, \constrjaceigvec_\dimambient\}$, where the indices indicate decreasing order w.r.t. the eigenvalue/singular value magnitude. The null spaces of $\samplecovariancematrix$ and $\constraintmanifoldjacobian$ are spanned by $\{\coveigvec_{\dimambient-\dimconstraint+1}, \dots, \coveigvec_\dimambient\}$ and $\{\constrjaceigvec_{\dimconstraint+1}, \dots, \constrjaceigvec_\dimambient\}$, respectively. The two conditions above imply that the projection of the null space eigenvectors of $\constraintmanifoldjacobian$ into the null space of $\samplecovariancematrix$ should be $\vct{0}$, and similarly for the row spaces. 
Hence, we achieve this by training {\ecmnn} to minimize projection errors $\norm{\covnullspaceeigmat \covnullspaceeigmat\T \constrjacnullspaceeigmat}_2^2$ and $\norm{ \constrjacnullspaceeigmat \constrjacnullspaceeigmat\T \covnullspaceeigmat}_2^2$ with 
$\covnullspaceeigmat = 
\begin{bmatrix}
    \coveigvec_{\dimambient-\dimconstraint+1} & \dots & \coveigvec_\dimambient
\end{bmatrix}$
and 
$\constrjacnullspaceeigmat =  
\begin{bmatrix}
    \constrjaceigvec_{\dimconstraint+1} & \dots & \constrjaceigvec_\dimambient
\end{bmatrix}$.
%
% To-Do: also point out that the eigenvectors of Local PCA does NOT encode orientation, since sample covariance matrix is positive semi-definite, and hence the SVD has the left and right eigenvectors being the same --flipping the polarity of one of the eigenvectors will still lead to the same sample covariance matrix (SVD eigenvector v and -v is the same thing)--. On the other hand, the eigen decomposition of the Jacobian matrix results in eigenvectors who has polarity information, i.e. with eigenvalue fixed and positive, the eigenvector v and -v is NOT the same.
% To-Do: also point out that SVD result (in terms of eigenvectors ordering) for Local PCA is sensitive to the K-nearest-neighbors involved. For example on the case of 3D line constraint, the dimensionality of the constraints is 2, and neither of the eigenvectors in the normal space are dominant; however, a slight bit of noise in the data involved nearby point q1 and q2 (both on the manifold, and q1 != q2), can lead to two different eigenvector decompositions by SVD at q1 and q2. Hence, we cannot align each individual eigenvector of Local PCA with an eigenvector of the Jacobian J, as they may not correspond one another; what we can do is to align the null space of the Local PCA with the row space of the Jacobian, and to align the row space of the Jacobian with the null space of Local PCA, e.g. using projection error minimization.

\subsection{Data augmentation with off-manifold data}
% ~\\
The training dataset is on-manifold, i.e., each point $\jointposition$ in the dataset satisfies $\constraintfunction(\jointposition) = \vct{0}$. 
Through Local PCA on each of these points, we know the data-driven approximation of the normal space of the manifold at $\jointposition$. 
Hence, we know the directions where the violation of the equality constraint increases, i.e., the same direction as any vector picked from the approximate normal space. 
Since our future use of the learned constraint manifold on motion planning does not require the acquisition of the near-ground-truth value of $\constraintfunction(\jointposition) \neq \vct{0}$, we can set this off-manifold valuation of $\constraintfunction$ arbitrarily, as long as it does not interfere with the utility for projecting an off-manifold point onto the manifold. 
Therefore, we can augment our dataset with off-manifold data to achieve a more robust learning of {\ecmnn}. 
For each point $\jointposition$ in the on-manifold dataset, and for each random unit vector $\randunitvec$ picked from the normal space at $\jointposition$, we can add an off-manifold point $\augjointposition = \jointposition + \augidx \augmagnitude \randunitvec$ with a positive integer $\augidx$ and 
% a small positive scalar $\augmagnitude$ proportional to the square root of the biggest eigenvalue of $\samplecovariancematrix$. 
a small positive scalar $\augmagnitude$ (see Figure \ref{fig:localpca} for a visualization). 
However, if the
closest on-manifold data point to an augmented point
$\augjointposition = \jointposition + \augidx \augmagnitude \randunitvec$ 
is not $\jointposition$, we reject it.
This prevents situations like augmenting a point on a sphere beyond the center of the sphere. 
With this data augmentation, we now define several losses used to train {\ecmnn}.
%
\subsubsection{Training losses}
\label{sssec:losses}
\imr{rename siamese losses}
\textbf{Loss based on the norm of the output vector of {\ecmnn}} 
For the augmented data point $\augjointposition = \jointposition + \augidx \augmagnitude \randunitvec$, we set the label satisfying $\norm{\constraintfunction(\augjointposition)}_2 = \augidx \augmagnitude$. During training, we minimize the norm prediction error $\normloss = \norm{(\norm{\constraintfunction(\augjointposition)}_2 - \augidx \augmagnitude)}_2^2$ for each augmented point $\augjointposition$.
\\
\textbf{Siamese loss for reflection pairs}
For the augmented data point $\augjointposition = \jointposition + \augidx \augmagnitude \randunitvec$ and its reflection pair $\jointposition - \augidx \augmagnitude \randunitvec$, we can expect that $\constraintfunction(\jointposition + \augidx \augmagnitude \randunitvec) = -\constraintfunction(\jointposition - \augidx \augmagnitude \randunitvec)$. Therefore, during training we also try to minimize the siamese loss $\siamreflectionloss = \norm{\constraintfunction(\jointposition + \augidx \augmagnitude \randunitvec) + \constraintfunction(\jointposition - \augidx \augmagnitude \randunitvec)}_2^2$.
\\
\textbf{Siamese loss for augmentation fraction pairs}
Similarly, between the pair $\augjointposition = \jointposition + \augidx \augmagnitude \randunitvec$ and $\jointposition + \frac{a}{b} \augidx \augmagnitude \randunitvec$, where $a$ and $b$ are positive integers satisfying $0 < \frac{a}{b} < 1$, we can expect that $\frac{\constraintfunction(\jointposition + \augidx \augmagnitude \randunitvec)}{\norm{\constraintfunction(\jointposition + \augidx \augmagnitude \randunitvec)}_2} = \frac{\constraintfunction(\jointposition + \frac{a}{b} \augidx \augmagnitude \randunitvec)}{\norm{\constraintfunction(\jointposition + \frac{a}{b} \augidx \augmagnitude \randunitvec)}_2}$. Hence, during training we also try to minimize the siamese loss $\siamfracloss = \norm{\frac{\constraintfunction(\jointposition + \augidx \augmagnitude \randunitvec)}{\norm{\constraintfunction(\jointposition + \augidx \augmagnitude \randunitvec)}_2} - \frac{\constraintfunction(\jointposition + \frac{a}{b} \augidx \augmagnitude \randunitvec)}{\norm{\constraintfunction(\jointposition + \frac{a}{b} \augidx \augmagnitude \randunitvec)}_2}}_2^2$.
\\
\textbf{Siamese loss for similar augmentation pairs}
Suppose for nearby on-manifold data points $\jointposition_a$ and $\jointposition_c$, their approximate normal spaces $\normalspaceid_{\jointposition_a}\constraintmanifold$ and $\normalspaceid_{\jointposition_c}\constraintmanifold$ are spanned by eigenvector bases $\lnormalcoordframe^a = \{\coveigvec^a_{\dimambient-\dimconstraint+1}, \dots, \coveigvec^a_\dimambient\}$ and $\lnormalcoordframe^c = \{\coveigvec^c_{\dimambient-\dimconstraint+1}, \dots, \coveigvec^c_\dimambient\}$, respectively\footnote{$\normalspaceatjointposition$ is the normal space at point $\jointposition$ on manifold $\constraintmanifold$.}. 
If $\lnormalcoordframe^a$ and $\lnormalcoordframe^c$ are closely aligned, the random unit vectors
$\randunitvec_a$ from $\lnormalcoordframe^a$ and $\randunitvec_c$ from $\lnormalcoordframe^c$ can be obtained by 
$\randunitvec_a = \frac{\sum_{j=\dimambient-\dimconstraint+1}^\dimambient \randscalarweight_j \coveigvec^a_j}{\norm{\sum_{j=\dimambient-\dimconstraint+1}^\dimambient \randscalarweight_j \coveigvec^a_j}_2}$ 
and $\randunitvec_c = \frac{\sum_{j=\dimambient-\dimconstraint+1}^\dimambient \randscalarweight_j \coveigvec^c_j}{\norm{\sum_{j=\dimambient-\dimconstraint+1}^\dimambient \randscalarweight_j \coveigvec^c_j}_2}$, 
where $\{\randscalarweight_{\dimambient-\dimconstraint+1}, \dots, \randscalarweight_\dimambient\}$ 
are random scalar weights from a standard normal distribution common to both the bases of $\lnormalcoordframe^a$ and $\lnormalcoordframe^c$. This will ensure that $\randunitvec_a$ and $\randunitvec_c$ are aligned as well, and we can expect that  $\constraintfunction(\jointposition_a + \augidx \augmagnitude \randunitvec_a) = \constraintfunction(\jointposition_c + \augidx \augmagnitude \randunitvec_c)$. Therefore, during training we also try to minimize the siamese loss $\siamsimilarloss = \norm{\constraintfunction(\jointposition_a + \augidx \augmagnitude \randunitvec_a) - \constraintfunction(\jointposition_c + \augidx \augmagnitude \randunitvec_c)}_2^2$. 
In general, the alignment of $\lnormalcoordframe^a$ and $\lnormalcoordframe^c$ is not guaranteed, 
for example due to the numerical sensitivity of singular value/eigen decomposition. 
Therefore, we introduce an algorithm for Orthogonal Subspace Alignment (OSA) in the Supplementary Material to ensure that this assumption is satisfied.

While $\normloss$ governs only the norm of {\ecmnn}'s output, the other three losses $\siamreflectionloss$, $\siamfracloss$, and $\siamsimilarloss$ constrain the (vector) outputs of {\ecmnn} based on pairwise input data points without explicitly hand-coding the desired output itself. We avoid the hand-coding of the desired output because this is difficult for high-dimensional manifolds, except when we have prior knowledge about the manifold, such as in the case of Signed Distance Fields (SDF) manifolds.

%===============================================================================

% \section{Data generation}
% \label{sec:data}
% %\subsection{From demonstrations}


%===============================================================================
\section{Experiments}
\label{sec:ecomann_experiments}
%
\begin{figure}
\centering
% \begin{subfigure}{0.25\textwidth}
% \includegraphics[trim={1cm 1cm 1cm 1cm}, clip, width=\textwidth]
% {figures/ecmnn_viz_1.png} 
% \caption{Training set and reconstructed training set from {\ecmnn}}
% \label{fig:vae_3dof_recon}
% \end{subfigure}
\begin{subfigure}{0.4\textwidth}
\includegraphics[trim={1cm 1cm 1cm 1cm}, clip, height=0.7\textwidth]
{ecomann_figures/ecmnn_viz_sample.png}
\caption{Projected samples from {\ecmnn}}
\label{fig:ecomann_3dof_sample}
\end{subfigure}
% \begin{subfigure}{0.25\textwidth}
% \includegraphics[trim={1cm 1cm 1cm 1cm}, clip, width=\textwidth]
% {figures/vae_3dof_recon.png} 
% \caption{Training set and reconstructed training set from {\ecmnn}}
% \label{fig:vae_3dof_recon}
% \end{subfigure}
\hspace{2em}
\begin{subfigure}{0.4\textwidth}
\includegraphics[trim={1cm 1cm 1cm 1cm}, clip, height=0.7\textwidth]
{ecomann_figures/vae_3dof_samples.png}
\caption{New samples from VAE}
\label{fig:vae_3dof_sample}
\end{subfigure}
%\begin{figure}
%\begin{subfigure}{0.5\textwidth}
%\includegraphics[trim={5cm 2cm 5cm 4cm}, clip, width=\textwidth]
%{figures/vae_3dof_recon_viz.png} 
%\caption{Training set and reconstructed training set from VAE}
%\label{fig:vae_3dof_recon}
%\end{subfigure}
%\begin{subfigure}{0.5\textwidth}
%\includegraphics[trim={5cm 2cm 5cm 4cm}, clip, width=\textwidth]
%{figures/vae_3dof_samples_viz.png}
%\caption{New samples from VAE}
%\label{fig:vae_3dof_sample}
%\end{subfigure}
\caption{Visualization for experiment \ref{sec:experiment1}, Plane dataset. Red points are the training dataset and blue points are samples generated from the learned manifolds.}
\label{fig:samples}
\end{figure}
%We collected a dataset of human demonstrations performing a pouring task from a
%cup to a bowl on a table using an HTC Vive device. We recorded 48
%demonstrations, each consisting of two pours from the same initial position.
%The 48 demonstrations covered pours from all locations around the bowl;
%however, we restrict the data used in this paper to the 22 pours performed from
%the left side from the robot's perspective. The position ($xyz$) and
%orientation (quaternion) of the cup were recorded at 60 Hz \imr{someone please
%fact check me} resulting in 13200 individual configurations. We then used
%PyBullet \citep{coumans2019} to generate robot joint configurations
%corresponding to each of these task space configurations using inverse
%kinematics for the 6 DoF xArm. The result is the dataset used for learning the
%pouring constraint.
%
%\subsection{From simulation}
We use the robot simulator MuJoCo \cite{todorov2012mujoco} to generate four
datasets. For each dataset, we define a ground truth constraint $\bar{h}_M$,
randomly sample points in the configuration (joint) space, and use a constrained
motion planner to find robot configurations in $\onconstraintconfigspace$ that
produce the on-manifold datasets:
    \textbf{Sphere}: 3D point that has to stay on the surface of a sphere. $N=5000, d=3, l=1$.
    \textbf{3D Circle}: A point that has to stay on a circle in 3D space. $N=1000, d=3, l=2$.
    % renaming all 3DOF to "Plane" 
    \textbf{Plane}: Robot arm with 3 rotational DoFs where the end effector has to be on a plane. $N=20000, d=3, l=1$.
    % renaming all 6DOF to "Orient"
    \textbf{Orient}: Robot arm with 6 rotational DoFs that has to keep its orientation upright (e.g., transporting a cup). $N=21153, d=6, l=2$.
    %\textbf{Handover}: Robot arm with 6 rotational DoFs and a mobile base with 2 translational DoFs. The manifold is defined as an equality constraint that describes the handover of an object between the two robots. $N=10046, d=8, l=4$. \imr{double check that ecomann learns l=4}

\subsection{Accuracy and precision of learned manifolds} 
\label{sec:experiment1}
%\pe{Is there a different term we could use instead of quality? Maybe accuracy?} \imr{how's that?}
We compare the accuracy and precision of the manifolds learned by {\ecmnn}
with those learned by a variational autoencoder (VAE) \cite{kingma2013AutoEncodingVB}. 
VAEs are a popular generative model that embeds data points as a distribution in a learned latent space, and as such new latent vectors
can be sampled and decoded into new examples which fit the distribution of
the training data. 
We use two metrics: First, the distance $\mu_{\bar{h}_M}$ which measures how far a point is away from the ground-truth manifold $\bar{h}_M$ and which we evaluate for both the training data points and randomly sampled points, and second,
the percent $P_{\bar{h}_M}$ of randomly sampled points that are on the manifold $\bar{h}_M$.
%\pe{I would use a different symbol for the GT manifold, maybe something like $\bar{h}_M(q)$}.
%
%$\mu_{\bar{h}_M}$ is computed by taking the distance between a set of points and the ground truth manifold.
%$P_{\bar{h}_M}$ is calculated by the percent of a set of points which lie within \imr{insert threshold here} of the ground truth manifold. 
We use a distance threshold of $0.1$ to determine success when calculating $P_{\bar{h}_M}$.
For {\ecmnn}, randomly sampled points are projected using gradient descent with the learned implicit function until convergence. 
For the VAE, latent points are sampled from $\mathcal{N}(0,1)$ and decoded into new configurations.

We sample 1000 points for each of these comparisons. 
We report results in Table \ref{table:projection} and a visualization of the test phase in Fig. \ref{fig:samples}. 
We also plot the level set and the normal space eigenvector field of the {\ecmnn} trained on the sphere and plane constraint dataset in Fig. \ref{fig:contourplot_vecfield}.
In all experiments, we set the value of the augmentation magnitude $\augmagnitude$ to the square root of the mean eigenvalues of the approximate tangent space, which we found to work well experimentally.
With the exceptions of the embedding size and the input size, which are set to the same dimensionality $l$ \imr{double check this} as the constraint learned by {\ecmnn} 
and the ambient space dimensionality $d$ of the dataset, respectively,
the VAE has the same parameters for each dataset: 
4 hidden layers with 128, 64, 32, and 16 units in the encoder and the same but reversed in the decoder; the weight of the KL divergence loss $\beta = 0.01$; using batch normalization; and trained for 100 epochs.

Our results show that for every dataset except Orient, {\ecmnn} out performs the VAE in both metrics. 
{\ecmnn} additionally outperforms the VAE with the Orient dataset in the testing phase, which suggests more robustness of the learned model. 
We find that though the VAE also performs relatively well in most cases, it cannot learn a good representation of the 3D Circle constraint and fails to produce any valid sampled points. 
{\ecmnn}, on the other hand, can learn to represent all four constraints well.
%The mean distance for Orient is higher than for the others, perhaps because this dataset is more complex.

\begin{table}[H]
  \caption{Accuracy and precision of learned manifolds averaged across 3 instances. 
 %The mean and standard deviation of the distance of points to the ground truth
 %and the percentage of points within \imr{insert threshold here} of the manifold are reported. 
 ``Train" indicates results on the on-manifold training set;  ``test" indicates $N=1000$ projected (\ecmnn) or sampled (VAE) points.}
  \label{table:projection}
  \centering
  \resizebox{\columnwidth}{!}{%
%   \begin{tabular}{c||ccc|ccc}
%     \toprule
%           & \multicolumn{6}{c}{Method} \\
%      Dataset & \multicolumn{3}{c}{\ecmnn} & \multicolumn{3}{c}{VAE} \\
%      \cmidrule{2-7}
%               & $\mu_{\bar{h}_M}$ (train) & $\mu_{\bar{h}_M}$ (test) & $P_{\bar{h}_M}$
%               & $\mu_{\bar{h}_M}$ (train) & $\mu_{\bar{h}_M}$ (test) & $P_{\bar{h}_M}$
%                 \\
% \midrule
%       Sphere 
%       & $0.025\pm 0.005$ & $0.025 \pm 0.006$ & $95.667 \pm 4.190$ 
%       & $0.105\pm 0.088$ & $0.161 \pm 0.165$ & $46.867 \pm 18.008$
%       \\
%       3D Circle     
%       & $0.027 \pm 0.010$ & $0.027 \pm 0.010$ & $71.333 \pm 20.854$ 
%         & $0.894 \pm 0.074$ & $0.902 \pm 0.069$ & $0.0 \pm 0.0$   \\
%       Plane  
%       & $0.022 \pm 0.010$ & $0.022 \pm 0.010$ & $85.000 \pm 19.131$ 
%         & $0.053 \pm 0.075$ & $0.112 \pm 0.216$  & $77.733 \pm 7.721$ \\
%       Orient     & $0.059\pm 0.005$ & $0.058 \pm 0.005$ & $69.500 \pm 11.500$
%         & $0.010 \pm 0.037$ & $0.085 \pm 0.237$ & $85.9 \pm 1.068$   \\
%     %   Handover     & x & x & x 
%         % & $0.112 \pm 0.055$ & $0.224 \pm 0.192$ & $25.633 \pm 6.563$  \\
%       \bottomrule
%   \end{tabular}
\begin{tabular}{c||ccc|ccc}
    \toprule
          & \multicolumn{6}{c}{Method} \\
     Dataset & \multicolumn{3}{c}{\ecmnn} & \multicolumn{3}{c}{VAE} \\
     \cmidrule{2-7}
              & $\mu_{\bar{h}_M}$ (train) & $\mu_{\bar{h}_M}$ (test) & $P_{\bar{h}_M}$
              & $\mu_{\bar{h}_M}$ (train) & $\mu_{\bar{h}_M}$ (test) & $P_{\bar{h}_M}$
                \\
\midrule
      Sphere 
      & $0.024\pm 0.009$ & $0.023 \pm 0.009$ & $100.0 \pm 0.0$ 
      & $0.105\pm 0.088$ & $0.161 \pm 0.165$ & $46.867 \pm 18.008$
      \\
      3D Circle     
      & $0.029 \pm 0.011$ & $0.030 \pm 0.011$ & $78.0 \pm 22.0$ 
        & $0.894 \pm 0.074$ & $0.902 \pm 0.069$ & $0.0 \pm 0.0$   \\
      Plane  
      & $0.020 \pm 0.005$ & $0.020 \pm 0.005$ & $88.5 \pm 10.5$ 
        & $0.053 \pm 0.075$ & $0.112 \pm 0.216$  & $77.733 \pm 7.721$ \\
      Orient     & $0.090\pm 0.009$ & $0.090 \pm 0.009$ & $73.5 \pm 6.5$
        & $0.010 \pm 0.037$ & $0.085 \pm 0.237$ & $85.9 \pm 1.068$   \\
    %   Handover     & x & x & x 
        % & $0.112 \pm 0.055$ & $0.224 \pm 0.192$ & $25.633 \pm 6.563$  \\
      \bottomrule
  \end{tabular}
  }
\end{table}



\begin{figure}
    \centering
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[trim={0cm 0cm 0cm 0cm}, clip, height=0.8\textwidth]{ecomann_figures/contourplot_vecfield_sphere.png}
        % \caption{Sphere Manifold}
        \label{sfig:contourplot_vecfield_sphere}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[trim={0cm 0cm 0cm 0cm}, clip, height=0.8\textwidth]{ecomann_figures/contourplot_vecfield_3dof_traj.png}
        % \caption{Plane Manifold}
        \label{sfig:contourplot_vecfield_3dof_traj}
    \end{subfigure}
    \caption{Trained {\ecmnn}’s level set contour plot and the normal space eigenvector field, after training on the sphere constraint dataset (left) and plane constraint dataset (right).}
    \label{fig:contourplot_vecfield}
\end{figure}

%Metrics:
%\begin{itemize}
%    \item train/test error on learned manifold
%    \item projection success rate measured on learned and ground-truth manifold
%\end{itemize}

\begin{figure}[H]
    \centering
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[height=0.9\textwidth]{ecomann_figures/3dof_success_rate.pdf}
        % \caption{}
        \caption{}
        \label{fig:3dof_success_rate}
    \end{subfigure}
    % \hfill
    \hspace{2em}
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[height=0.9\textwidth]{ecomann_figures/hourglass.png} 
        % \vspace{-10pt}
        \caption{}
        % \caption[width=0.20\textwidth]{Path on the learned manifold (red) and path on the ground truth manifold (black).}
        % \vspace{-40pt}
        \label{fig:ecomann_hourglass}
    \end{subfigure}
    \caption{The graph on the left shows the {\ecmnn} success rate on the Orient dataset over number of training iterations. On the right, a path planned on the learned manifold (red) and path on the ground truth manifold (black) are visualized.}
\end{figure}

\subsection{Ablation study of \ecmnn}
In the ablation study, we compare $P_{\bar{h}_M}$ across 4 different {\ecmnn} setups: 1) no ablation;
2) without data augmentation; 3) without siamese losses during training;  and 4) without orthogonal subspace alignment (OSA) during data augmentation. Results are reported in Table \ref{tab:ablation_table}. 
For this ablation test we use {\ecmnn} with 4 hidden layers of size 36, 24, 18, and 10.
The data suggest that all three parts of the training process are essential for a high success rate during projection. 
Of the three features tested, data augmentation appears to have the most impact.
%
This makes sense because without augmented data to train on, any configuration that does not already lie on the manifold will have undefined output when evaluated with {\ecmnn}. 
% \imr{I feel like there is a better way to phrase this but I don't know how -- feel free to edit}

\begin{table}[ht]
    \centering
    % \caption{Projection Success Rate w.r.t. Analytical Manifold}
    \caption{Percentage of projection success rate for a variety of ablation on {\ecmnn} components.}
% \begin{footnotesize}
% \scalebox{0.95}{
    \begin{tabular}{ |c||c|c|c| }
        \hline
        Ablation Type         & Sphere                  & 3D Circle               & Plane \\
        \hline
        \hline
        % No Ablation           & (94.00 $\pm$ 8.49) \% & (100.00 $\pm$ 0.00) \% & (92.33 $\pm$ 10.84) \% \\
        % w/o Data Augmentation & (10.33 $\pm$ 1.70) \% & (13.67 $\pm$ 1.25) \% & (1.67 $\pm$ 1.25) \% \\
        % w/o Siamese Losses    & (19.67 $\pm$ 3.09) \% & (71.33 $\pm$ 22.51) \% & (33.33 $\pm$ 6.13) \% \\
        % w/o OSA               & (55.67 $\pm$ 15.15) \% & (28.00 $\pm$ 20.83) \% & (58.00 $\pm$ 9.42) \% \\
        No Ablation           & (98.67 $\pm$ 1.89) \% & (100.00 $\pm$  0.00) \% & (92.33 $\pm$ 10.84) \% \\
        w/o Data Augmentation & ( 9.00 $\pm$ 2.45) \% & ( 16.67 $\pm$  4.64) \% & ( 3.67 $\pm$  3.30) \% \\
        w/o Siamese Losses    & (17.33 $\pm$ 3.40) \% & ( 65.67 $\pm$ 26.03) \% & (35.67 $\pm$  5.56) \% \\
        w/o Siamese Loss $\siamreflectionloss$ & (92.67 $\pm$ 4.03) \% & (  9.67 $\pm$  2.05) \% & (38.00 $\pm$ 16.87) \% \\
        w/o Siamese Loss $\siamfracloss$       & (88.33 $\pm$ 8.34) \% & ( 99.67 $\pm$  0.47) \% & (85.33 $\pm$ 16.68) \% \\
        w/o Siamese Loss $\siamsimilarloss$    & (83.00 $\pm$ 5.10) \% & ( 70.67 $\pm$ 21.00) \% & (64.33 $\pm$  2.62) \% \\
        w/o OSA               & (64.33 $\pm$ 9.03) \% & ( 33.33 $\pm$ 17.13) \% & (61.00 $\pm$  6.16) \% \\
        \hline
    \end{tabular}
    % }
    % \caption{\small A}
    \label{tab:ablation_table}
    % \end{footnotesize}
\end{table}

\subsection{Learning {\ecmnn} on noisy data}
We also evaluate {\ecmnn} learning on noisy data. We generate a noisy unit sphere dataset and a noisy 3D unit circle with additive Gaussian noise of zero mean and standard deviation 0.01. After we train {\ecmnn} on this noisy sphere and 3D circle datasets, we evaluate the model and obtain (82.00 $\pm$ 12.83) \% and (89.33 $\pm$ 11.61) \%, respectively, as the $P_{\bar{h}_M}$ metric.\footnote{The small positive scalar $\augmagnitude$ needs to be chosen sufficiently large as compared to the noise level, so that the data augmentation will not create inconsistent data w.r.t. the noise.}

\subsection{Relationship between the number of augmentation levels and the projection success rate}
%
Moreover, we also perform an experiment to study the relationship between the number of augmentation levels --i.e. the maximum value of the positive integer $\augidx$ in the off-manifold points $\augjointposition = \jointposition + \augidx \augmagnitude \randunitvec$-- and the projection success rate. As we vary the maximum value of $\augidx$ at 1, 2, 3, and 7 on the sphere dataset, the projection success rates are (5.00 $\pm$ 2.83) \%, (12.33 $\pm$ 9.03) \%, (83.67 $\pm$ 19.01) \%, and (97.33 $\pm$ 3.77) \%, respectively, showing that the projection success rate improves as the number of augmentation levels are increased.

\subsection{Motion planning on learned manifolds}
%
In the final experiment, we integrate {\ecmnn} into the sequential motion planning framework described in Section \ref{subsec:smp}. 
We mix the learned constraints with analytically defined constraints and evaluate it for two tasks. 
The first one is a geometric task, visualized in Figure \ref{fig:ecomann_hourglass}, where a point starting on a paraboloid in 3D space must find a path to a goal state on another paraboloid. 
The paraboloids are connected by a sphere, and the point is constrained to stay on the surfaces at all times.
In this case, we give the paraboloids analytically to the planner, and use {\ecmnn} to learn the connecting constraint using the Sphere dataset.
Figure \ref{fig:ecomann_hourglass} shows the resulting path where the sphere is represented by a learned manifold (red line) and where it is represented by the ground-truth manifold (black line). While the paths do not match exactly, both paths are on the manifold and lead to similar solutions in terms of path lengths. The task was solved in \SI{27.09}{\s} on a 2.2 GHz Intel Core i7 processor. The tree explored $1117$ nodes and the found path consists of $24$ nodes.


The second task is a robot pick-and-place task with the additional constraint that the transported object needs to be oriented upwards throughout the whole motion. 
For this, we use the Orient dataset to learn the manifold for the transport phase and combine it with other manifolds that describe the pick and place operation. The planning time was \SI{42.97}{\s}, the tree contained $1421$ nodes and the optimal path had $22$ nodes. Images of the resulting path are shown in Figure \ref{fig:pickandplace}. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.19\textwidth]{ecomann_figures/pick_place_2.png}
    \includegraphics[width=0.19\textwidth]{ecomann_figures/pick_place_4.png}
    \includegraphics[width=0.19\textwidth]{ecomann_figures/pick_place_6.png}
    \includegraphics[width=0.19\textwidth]{ecomann_figures/pick_place_8.png}
    \includegraphics[width=0.19\textwidth]{ecomann_figures/pick_place_10.png}
    \caption{The images visualize a path that was planned on a learned orientation manifold.}
    \label{fig:pickandplace}
\end{figure}


%===============================================================================

\section{Discussion and conclusion}
\label{sec:ecomann_conclusion}
In this paper, we presented a novel method called {\ecmnnlong} for learning equality constraint manifolds from data.
{\ecmnn} works by aligning the row and null spaces of the local PCA and network Jacobian, which results in approximate learned normal and tangent spaces of the underlying manifold, suitable for use within a constrained sampling-based motion planner.
In addition, we introduced a method for augmenting a purely on-manifold dataset to include off-manifold points and several loss functions for training.
This improves the robustness of the learned method while avoiding hand-coding the labels for the augmented points. We also showed that the learned manifolds can be used in a sequential motion planning framework for constrained robot tasks.

While our experiments show success in learning a variety of manifolds, there are some limitations to our method.
First, {\ecmnn} by design can only learn equality constraints. Although many tasks can be specified with such constraints, inequality constraints are also an important part of many robot planning problems. 
Additionally, because of inherent limitations in learning from data, {\ecmnn} does not guarantee that a randomly sampled point in configuration space will be projected successfully onto the learned manifold.
This presents challenges in designing asymptotically complete motion planning algorithms, and is an important area of research.
In the future, we plan on further testing {\ecmnn} on more complex tasks, and in particular on tasks which are demonstrated by a human rather than from simulation.



==> multirobot.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}

% Motivation - Why it matters
% \begin{itemize}
%     \item biologists study natural environments and use robots to help do surveys
%     \item one flexible way of describing what areas the robot should investigate is by assigning quantiles
%     \item biologists are also collaborative and do studies with other labs, and/or may have more than one robot that they can use at a time
%     \item in a collaborative study, this approach would also be desirable
%     \item generally more robots is assumed to always be better
%     \item it is unclear how it would scale to multiple robots and whether it would be beneficial at all/until what point the benefit drops off
%     \item Robots are really expensive (cite \$20k for matrice etc) and number of required people for operation increases 
%     \item we present a study on the impact of multiple robots on a quantile estimation task of natural aquatic environments
%     \item We believe that this study can influence purchasing and deployment decisions in studies where we can direct the efforts of researchers
% \end{itemize}

Scientists who study natural environments have used robots to assist in surveying or exploring regions of interest, for example to monitor harmful algal blooms \cite{kemna_pilot_2018,harmful2022}. To describe such phenomena both flexibly and in an interpretable manner, it has been proposed to specify quantiles of interest that robots can target during exploration \cite{rayas2022informative}. Previous work on quantile estimation in this context has focused on single-robot adaptive surveys; in this work, we study multi-robot surveys, motivated by groups that may have more than one robot available, and by collaborative surveys between groups that would like to pool their robot resources to maximize scientific output from a survey. 
Though the naive assumption may be that more robots will always be better, in this work, we aim to investigate, in a principled manner,  under what conditions this is true.
Deploying a robot in the environment can be expensive since more resources are typically required with more robots deployed, and it is unclear how having more robots in such a use case will scale.
This study assesses the impact of team size, starting location, planning budget, and communication between robots for quantile estimation tasks in field environments. We believe it is an important step toward principled decisions regarding robot deployments for field robotics in aquatic biology.

Our contributions are as follows:
\begin{itemize}
    \item We present the first study that investigates multirobot quantile estimation;
    \item we present quantitative results on the effect of team size on performance on real-world aquatic datasets;
    \item we present quantitative results on the effect of parameters including initial location spread, exploration budget, and inter-robot communication on performance, giving insight into what matters for a multirobot study;
    \item we discuss the results in the context of field applications and how they may transfer to different experimental setups.
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{multirobot_figures/mr_qtiles_hero.png}
    \caption{Some variations of multirobot plannning approaches.
    Top row shows initial spread $\spread = 0$: All robots start in the center.
    Bottom row shows initial spread $\spread = 0.5$: Robots start spread in an area 50\% length and width of entire workspace.
    Left column shows no communication: Robots have no knowledge of the others; equivalent to each robot planning as if it were the only one.
    Middle column shows stochastic communication: Robots attempt to share observations but messages fail stochastically based on inter-robot distance.
    Right column shows full communication: Robots share the same environment model; equivalent to centralized planning.
    }
    \vspace{-10pt}
    \label{fig:multirobot-hero}
\end{figure}


\section{Background}
In this section, we present relevant background on the motivating problem and place our contributions in the context of previous work in these areas.
In this work, we are interested in the problem of multirobot quantile estimation.
Specifically, we ask whether and under what conditions a multirobot approach to this problem is effective. 
\imr{move to multirobot}
Here, we build upon the work in \cite{rayas2022informative}, but there are several differences.
First, \cite{rayas2022informative} seeks to produce, as a final output, a set of locations at which the desired quantile values can be found, while our goal is to accurately estimate the desired quantile values.
Second, we generalize the problem to the multirobot domain, where \cite{rayas2022informative} only considers one robot.
Finally, where \cite{rayas2022informative} proposes new objective functions for planning that is tailored to the quantile estimation problem, our focus is on investigating the impact of team size and other factors on quantile estimation accuracy, and thus we adopt just one of the previously proposed objective functions in all our experiments.
\imr{move to multirobot}
Here, we seek to investigate the effect of using multiple homogeneous robots specifically on the task of quantile estimation in natural environments, with the aim of understanding how to most effectively use resources for challenging and resource-constrained field work problems.

\imr{move to multirobot}
Our work differs from these (multirobot ipp) in that it explicitly addresses the question of different team sizes and other factors' impact on performance. Further, the task we study is to improve the estimates of an arbitrary set of quantiles, rather than coverage or hotspots which has typically been the focus of other work.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Methods}
The problem considered in this paper is that of accurately estimating a set of quantiles of a distribution of interest, such as algae concentration in a lake, 
by exploring a finite 2D workspace with $\nrobots$ robots that take measurements at the locations they visit.

Formally, we discretize the planning space to $\gtlocations \subset
\mathbb{R}^2$, the set of locations that robots can visit defined by a grid.
Robots can move in either the positive or negative $x$ or $y$
directions. In this work, each robot is a drone that flies at a fixed height
above the environment and takes measurements via a downward pointing
hyperspectral camera.  Robots can take a picture at each location with
measurement resolution finer than $\gtlocations$, so $\gtsensedlocations$
represents the set of locations that a robot can measure by taking a picture at
each $\gtlocation \in \gtlocations$, and $\gtsensedvalues$ represents the actual
values at those locations.

The quantiles of interest are assumed to be given from the scientists or operators as $\quantiles$, and their true values are
defined as $\quantilevalues = \textit{quantiles}(\gtsensedvalues,\quantiles)$.
There are $\nrobots$ homogeneous robots collaborating on the estimation task
with a planning step budget of $B_T$. The locations at which a robot has taken a
measurement up to time $t$ and the corresponding values measured are represented
by $\sensedlocations_{0:t}$ and $\sensedvalues_{0:t}$, respectively.  Each robot
$n$ maintains an estimate of the quantile values which is given by
\begin{equation}
    \estimatedquantilevalues_n = quantiles(\mu^{(n)}_{GP_t}(\gtsensedlocations),\quantiles)
\end{equation}
where $\mu^{(n)}_{GP_t}(\gtsensedlocations)$ is the estimate of all possible locations
using the GP conditioned on $\sensedlocations_{0:t}$ and $\sensedvalues_{0:t}$. 
Note that, for clarity, we will omit the $(n)$ superscript in the remainder of the section.

For a given $\nrobots$ and $B_T$, our problem is to select a complete path
$\boldsymbol{P}^*$ composed of paths $P_n$ for each robot $n$ within a planning
budget constraint: 

\begin{equation}
\boldsymbol{P}^* = \argmax_{\boldsymbol{P}} f(\boldsymbol{P})
\end{equation}

where
\begin{equation}
   \boldsymbol{P} = \bigcup_{n \in \nrobots} P_n 
\end{equation}

\begin{equation}
   \qquad \forall n \in N :~\textit{length}(P_n) \leq B_n
\end{equation}
and $f$ is the objective function used during planning. 
In this work, we are interested in estimating the value of the underlying
concentration at quantiles $Q$. Note that our goal is not finding the highest
value in the environment nor optimizing model accuracy at every location.

To this end, we use the quantile standard error objective function to evaluate a
proposed location \cite{rayas2022informative}, which measures the difference in
standard error of the estimated quantile values using a robot's current environment
model $\mu_{GP_{i-1}}$, compared to using its current model updated with the
expected new measurements at the proposed location $\mu_{GP_{i}}$.
It additionally includes a term that encourages exploration of locations with
high model variance weighted by the parameter $c$, called the
\textit{exploration bias}.

\begin{equation}
\label{eq:objective}
    \objectivefunction(\sensedlocations_i) =
\frac{d}{\numtiles} +
\sum_{\sensedlocation_j \in \sensedlocations_i} c\sigma^2(\sensedlocation_j)
\end{equation}

\begin{equation}
    d =
\|se(\mu_{GP_{i-1}}(\gtsensedlocations),\quantiles) -
se(\mu_{GP_{i}}(\gtsensedlocations),\quantiles) \|_{1}
\end{equation}

We formulate the planning problem as a POMDP, as described in 
\Cref{ssec:ipp} \cite{rayas2022informative} and defined in \Cref{tab:BayesianSearchAndPOMDPs}, and solve the planning problem using a POMCPOW solver
\cite{sunberg2018online}.  

% \begin{table}[]
% %\vspace{2pt}
% \begin{tabular}{c|c}
% \textbf{POMDP} & \textbf{Informative Path Planning}        \\ \hline
% States         & Robot position $\location_t$, Underlying unknown function $GT$ \\ \hline
% Actions        & Neighboring search points                     \\ \hline
% Observations   & Robot position $\location_t$, Measured location(s) $\sensedlocations_t = o(\location_t)$   \\ 
%                & Measured value(s) $\sensedvalues_t = GT(\sensedlocations_t) + \mathcal{N}(0,\sigma_\textrm{noise})$ \\\hline
% Belief         & GP conditioned on previously measured     \\ 
% & locations  $(\sensedlocations_{0:t-1})$ and values $(\sensedvalues_{0:t-1})$ \\ \hline
% Rewards        & $\objectivefunction(\sensedlocations_t)$
% \end{tabular}
% \caption{Informative Path Planning as a POMDP \cite{rayas2022informative}.}
% \label{tab:BayesianSearchAndPOMDPs}
% %\vspace{-0.25in}
% \end{table}

At each planing step, the robot selects the next
location to travel to based on the measurements it has collected and its
corresponding environment model. After moving to the next location, the robot
takes an image, collecting a set of (noisy) point measurements, which it feeds back into
its GP model.
In this work, we assume a straight-line low-level motion planner for generating
trajectories from one location to the next.
We additionally enable a best-effort communication system between
robots and compare to two other communication formulations, which are further
described in \Cref{sssec:comms}. The planning process continues with each of the
$\nrobots$ robots until the allotted budgets have been reached, at which point
planning is complete and the robots can return to the base.

% describe how final quantiles are computed
% At this time, final quantile value estimates are computed as follows:
%  \begin{equation}
%      \estimatedquantilevaluesfinal = quantiles(\bigcup_{n \in \nrobots} \mu_{GP_{B_n}}(\gtsensedlocations),\quantiles)
%  \end{equation}
% At this time, all measurements from all robots are compiled. %, and since measurements are noisy, any locations that were measured multiple times take on their average value.
% We then condition a new GP model on these aggregated data and use it to produce $\estimatedquantilevaluesfinal$ as follows:
% \begin{equation}
%     \estimatedquantilevaluesfinal = quantiles(\mu_{GP_\textrm{aggregate}}(\gtsensedlocations),\quantiles)
% \end{equation}
At this time, all measurements from all robots are compiled and used to produce $\estimatedquantilevaluesfinal$ as follows:
\begin{equation}
    \estimatedquantilevaluesfinal = quantiles(\sensedvalues_\textrm{aggregate},\quantiles)
\end{equation}


We now introduce several variations on the multirobot approach which we compare
in our experiments, as illustrated in \Cref{fig:multirobot-hero}.
In the single robot
case, the formulation is the same, simply with $\nrobots = 1$; however, the
communication and initial spread variations have no effect on the implementation or
execution of the planning.

\subsection{Initial Location Spread}
During informative path planning, teams of robots will not cover the entire area
possible and are naturally affected by their starting area.  To this end, we
define an initial location spread parameter $\spread$ which varies from 0 (all robots
start at the same location) to 1 (robots are spread around the
entire workspace).  At spread 0.5, for example, the robots would be started evenly
spaced in a rectangle half the size of the entire workspace. We choose initial locations for robots following a variation of Lloyd's algorithm \cite{lloyd1982least} which iteratively computes the centroids of an approximate Voronoi tessellation of the space and reassigns the locations to those centroids.
We perform the process for $100$ iterations using $100 \nrobots$ randomly sampled points. The result is $\nrobots$ locations approximately uniformly spread in the allotted workspace.


\subsection{Communication}
\label{sssec:comms}
To investigate the impact of communication on the effectiveness of multirobot
planning, we distinguish between three versions of information sharing.

\textit{Full communication} assumes perfect, instantaneous communication,
which translates to every robot using the same shared GP model of the
environment. This is a centralized formulation of the planning problem. After
every measurement that any robot takes, the shared GP is updated and is available immediately to other robots for planning.

At the other extreme is \textit{no communication}. In this case, each robot has its own environment model.
Essentially, this implementation is equivalent to
$\nrobots$ robots planning in the environment independently, with no knowledge of the
others; when new measurements are taken, they are only used to update that
robot's GP and motion is not coordinated at all.
We believe a comparison to no communication provides a valuable baseline to understand how much improvement arises due solely to information sharing. 
In a practical sense, if separate research groups come together to pool their robots, implementing coordinating mechanisms can demand significant cost of time and effort. 
In that case, deploying the available robots with no behavioral changes may be simplest.

The third variation, \textit{stochastic communication}, lies in the middle.
After taking measurements, a robot attempts to transmit the information to
every other robot. We model each attempt as a Bernoulli trial and
assume messages are successfully transmitted with sigmoidal probability $p_{\textrm{success}}$,
following \cite{clark2021queue} and where $distance$ is the distance between the
two robots, $\eta$ is a constant defining the sigmoid steepness,
and $r$ is the distance at which communication quality degrades past a threshold:
\begin{equation}
\label{eq:comms-probability}
    p_{\textrm{success}} = \frac{1}{1 + e^{\eta (distance - r)}}
\end{equation}
We assume that if communication is successful between robots $n$ and $m$ at time
step $i$, all $\sensedlocations_i$ are received by $m$ (i.e., there are no partial
or corrupted measurements transmitted).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth, height=0.25\linewidth]{multirobot_figures/transmission_modedl.pdf}
  %
  \caption{
  Visualization of the message transmission success probability based on inter-robot distance (\Cref{eq:comms-probability}).
}
  \label{fig:comms-probability}
\end{figure}

\section{Experimental Setup}
In our experiments, we evaluate performance on two different real-world datasets. 
The datasets
% , A and B, 
are collected using a hyperspectral camera mounted on a drone that flies over a freshwater lake. 
Each dataset is collected in the same area of the lake but on different days, leading to different algae distributions.
The robots are bounded in an area of approximately $80 \times 60$ meters.
We use the 400nm channel from the datasets as a proxy for algae and normalize the measured pixel intensity ($0-255$) to $[0, 1]$.
We test two sets of quantiles of interest in our experiments: quartiles $\quantiles = (0.25, 0.5, 0.75)$ and extrema $\quantiles = (0.9, 0.95, 0.99)$.
For each combination of parameters in all experiments, we run 2 seeds.
The available workspace is discretized into a 25x25 grid $\gtlocations$. The environment is unknown ahead of time to the robots.
We assume a communication model as described in \Cref{sssec:comms} with $\eta = 0.5$ and $r = 10$, and a visualization of \Cref{eq:comms-probability} with these parameters is shown in \Cref{fig:comms-probability}. 
We additionally add zero-mean Gaussian noise with $\sigma_\textrm{noise} = 0.05$ to each measurement taken by a robot.
In the POMCPOW solver, we set number of rollouts per step to 100,
rollout depth to 4, and the planner discount factor to 0.8. 
The lengthscale for the GP is 12. We set the drone altitude to 7m and each image
is 25 pixels (measurements).

In order to better understand under what conditions multirobot teams are beneficial for quantile estimation,
we select several parameters to vary in order to investigate their impact on
performance. 
These are listed in \Cref{tab:params}.
As a measure of performance, we report the root mean squared error (RMSE) between the ground
truth quantile values $\quantilevalues$ and the estimated quantile values
$\estimatedquantilevaluesfinal$ at the end of the robot surveys.

\begin{table}[t]
  \begin{tabular}{lc} 
    \textit{Parameter} & \textit{Tested values} \\ 
    \hline 
    Initial location spread ($\spread$) & 0.0, 0.33, 0.66, 1.0 \\ 
    Total budget ($B_T$) & 10, 15, 30 \\
    Budget type  & \textit{complete, shared} \\
    Communication type &  \textit{none, stochastic, full, partitioned} \\ 
  \end{tabular}
  \caption{Parameters studied in our experiments}
  \label{tab:params}
\end{table}

\subsection{Initial Location Spread}
\label{ssec:alpha-expt}
In this experiment, we vary $\spread = \{0.0, 0.33, 0.66, 1.0\}$.
Each variation is tested on team sizes $\nrobots = \{2, 4, 8\}$, and 
we keep the budget constant at $ B_T = 15$. 
We additionally compare each $\spread$ with no communication and with stochastic communication, but do not consider the single robot case, as $\spread$ and communication have no effect with only one robot.
To quantify the significance of the performance differences observed, we report results from the Wilcoxon signed-rank test \cite{wilcoxon1992individual}, which is a nonparametric version of the t-test and tests whether two paired samples originate from different distributions.

\subsection{Planning Budget}
\label{ssec:budget-expt}
Next, we investigate the effect of the planning budget on performance.
To this end, we first vary $B_T = \{10, 15, 30\}$, setting $\spread$ to the constant value of $0.66$. 
When varying $B_T$, we only consider stochastic communication, and in addition to the multirobot teams, we also consider $\nrobots = 1$.

To control for the fact that a team with more robots will in practice simply
have more planning steps, and for a fairer comparison to a single robot baseline,
we additionally implement a variation on the budget constraint which we call
\textit{shared budget}. Here, we set $B_T = 15$ and split the total planning budget between robots,
i.e.  $\forall n \in \nrobots : B_n = B_T / \nrobots$.  When $(B_T \hspace{-3px}
\mod{\nrobots}) \neq 0$, the remainder is split evenly among the most robots
possible.
We compare this to the default of a \textit{complete budget}, which gives each robot
the full budget, i.e. $\forall n \in \nrobots : B_n = B_T$.
For both shared and complete budgets, we enable stochastic communication between the robots.

\subsection{Team Size and Communication}
\label{ssec:comms-expt}
Here, we compare performance with different values of $\nrobots$
across different levels of communication: full, stochastic, and none (see
\Cref{sssec:comms}).
Note that now we hold previous parameters constant: $\spread = 0.66; B_T = 15$, and use the same robot team sizes as before $\nrobots = \{1, 2, 4, 8\}$.
We additionally investigate the performance when the area is split up into regions by comparing against the \textit{partitioned} case.
This uses a Voronoi partition of the workspace based on the initial locations (with $\spread = 1.0$) and restricts each robot to stay within its assigned region at all times.
No communication is enabled between the partitioned robots.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Results}
We now present results from our experiments and include a discussion on their implications for real-world multirobot field work.
%
Boxplots show final RMSE between the estimated quantile values $\estimatedquantilevaluesfinal$ and the ground truth quantile values $\quantilevalues$ on the Y axis for an experiment, both aggregated across and refined by team sizes. 
Bars above indicate the Wilcoxon signed-rank significance levels for paired experiment groups \cite{florian_charlier_2022_7213391}.

\subsection{Initial Location Spread}
\label{ssec:alpha-results}
\begin{figure}[t!]
  \centering
  % Aggregate, no comms
 \includegraphics[width=\boxwidth,height=\boxheight]{multirobot_figures/boxplots/alpha_all-expts,CommsFalse,statsWilcoxon_greater,adjacent,RMSE-measuredYs.pdf}
   %
  % Not aggregate, no comms
 \includegraphics[width=\boxwidth,height=\boxheight]{multirobot_figures/boxplots/alpha_all-expts,CommsFalse_bynrobots,statsWilcoxon_greater,adjacent,RMSE-measuredYs.pdf}
  %
  % Aggregate, with comms
 \includegraphics[width=\boxwidth,height=\boxheight]{multirobot_figures/boxplots/alpha_all-expts,CommsTrue,statsWilcoxon_greater,adjacent,RMSE-measuredYs.pdf}
  %
  % Not aggregate, with comms
 \includegraphics[width=\boxwidth,height=\boxheight]{multirobot_figures/boxplots/alpha_all-expts,CommsTrue_bynrobots,statsWilcoxon_greater,adjacent,RMSE-measuredYs.pdf}
  %
  \caption{
  \textbf{Error vs. Initial location spread ($\spread$).}
  Top: No communication.
  Bottom: stochastic communication. 
  Right column shows results further separated by team size. 
  Bars above indicate significance under the one-sided Wilcoxon signed-rank test; ***: $\pppsig$, *: $\psig$, ns: no significance.
}
  \label{fig:alpha}
\end{figure}

\Cref{fig:alpha} shows the results of the experiments on $\spread$ using a one-sided Wilcoxon signed-rank test.
We observe that, in general, performance tends to improve (error decreases) with increasing $\spread$.
In particular, in the absence of stochastic communication as seen on the top row of \Cref{fig:alpha}, 
we see a statistically signficant performance improvement between $\spread = 0.33$ and $0.66$ ($\wpres{266}{0.001}$).
On the top right, further separated by $\nrobots$, we similarly observe 
a statistically significant improvement in performance between $\spread=0.33$ and $\spread=0.66$ for both $\nrobots=2$ and $\nrobots=4$ ($\wpres{33}{0.05}$, $\wpres{32}{0.05}$, respectively), 
but we do not see such an improvement between $\spread=0.66$ and $\spread=1.0$ in those cases.
In general, we also see that $\spread$ has a more drastic effect on performance the more robots there are, indicated by the decreasing maximum errors as $\nrobots$ increases.
However, in general, there appear to be diminishing returns with bigger $\spread$.
% These two results suggest that first, spreading robots out in the environment does lead to lower error when coordination is not possible, 
% but they also suggest that doing so may not be as valuable if there are few robots deployed.
% Second, if robots cannot communicate, a moderate spread will do reasonably well.

The bottom row of \Cref{fig:alpha} shows results when robots communicate stochastically with each other at different initial location spreads.
Although we see the same general trend on left, in this case, we do not see a statistically significant drop in error. 
%
When controlled for team size on the right, we again see increasing $\spread$ resulting in improved performance 
as indicated by lower median and maximum errors.
Compared to the case where there is no communication, we do not notice the same dependency on $\nrobots$ for the effect of $\spread$; in other words, the decrease in error due to $\spread$ appears relatively similar across different values of $\nrobots$ (shown by relative median and maximum errors).
We additionally note that for $\nrobots=8$, there is a statistically significant drop in error from $\spread = 0.33$ to $0.66$ ($\wpres{33}{0.05}$).
Based on these results, 
if robots must be deployed near each other but cannot communicate, then a small robot team may do just as well as a larger team, and vice versa; a small team that cannot communicate does not need to be spread very far to be effective.
On the other hand, a larger spread combined with a large team size will be beneficial in the absence of inter-robot communication, but there will be marginal returns with larger spread.
If communication is enabled, a larger spread will generally always be beneficial (although again with marginal returns), regardless of the team size.


\subsection{Planning Budget}

\begin{figure}
  \centering
  % Aggregate
 \includegraphics[width=\boxwidth,height=\boxheight]{multirobot_figures/boxplots/budget_all-expts,RMSE-measuredYs.pdf}
  %
  % By N robots
 \includegraphics[width=\boxwidth,height=\boxheight]{multirobot_figures/boxplots/budget_all-expts_bynrobots,RMSE-measuredYs.pdf}
  % This one includes the significant result
  % \includegraphics[width=\boxwidth, height=\boxheight]{multirobot_figures/boxplots/budget_all-expts_bynrobots stats: Wilcoxon_greater, RMSE (measured Ys).pdf}
  \caption{
  \textbf{Error vs. Budget (number of planning steps $B_T$).} 
  Right shows results further separated by team size. 
  % Bars above indicate significance under the one-sided Wilcoxon signed-rank test; **: $\ppsig$, *: $\psig$, ns: no significance.
  }
  \label{fig:budget}
\end{figure}

\begin{figure}
  \centering
  % Aggregate
 \includegraphics[width=\boxwidth,height=\boxheight]{multirobot_figures/boxplots/parallel_all-expts,RMSE-measuredYs.pdf}
  %
  % By N robots
 \includegraphics[width=\boxwidth,height=\boxheight]{multirobot_figures/boxplots/parallel_all-expts_bynrobots,RMSE-measuredYs.pdf}
  \caption{\textbf{Error vs. Budget Type (Shared and Complete).}
  Here, $B_T=15$.
  Left: Shared budget means the combined budget is $B_T$ for any $\nrobots$, while complete budget means it is $\nrobots \cdot B_T$. Note $\nrobots=1$ data not included here since budget type has no effect.
  Right: Results further separated by team size. 
  $\nrobots=1$ (blue) shown for comparison.
  % Bars above indicate significance under the one-sided Wilcoxon signed-rank test; **: $\ppsig$, *: $\psig$, ns: no significance.
  }
  \label{fig:complete-budget}
\end{figure}

Observing both the median and maximum errors on the left side of \Cref{fig:budget} suggests that in general,
a larger budget results in better performance. 
This is expected, as with a larger budgets, robots have more time to explore the environment and gather information, 
and we see a similar trend on the right when controlled for team size.
The improvements are not entirely consistent, however, as we see that $B_T = 30$ is not always better than $B_T = 15$.
This is somewhat surprising, as we would expect improvement with more steps given the results on the left.
What we observe on the right, rather, is that the performance improvement comes from an increase in $\nrobots$, indicated by lower median error for higher $\nrobots$.

To investigate this further, we control for total path length $\sum_n B_n$ and show results for shared and complete budgets on the right of
\Cref{fig:complete-budget}.
Recall that with a shared budget, $\forall n \in \nrobots : B_n = B_T / \nrobots$,
and for a complete budget, $\forall n \in \nrobots : B_n = B_T$
(see \Cref{ssec:budget-expt}).
With $B_T = 15$ and $\spread = 0.66$ in this experiment, we see similar performance between shared and complete budgets, which is again counterintuitive, as we would generally expect improvement given more steps.
However, we uncover the real effect when we further control for $\nrobots$, shown on the right. 
Even when the budget is shared, there is a notable improvement in maximum error when using more than $1$ robot.
This is particularly remarkable, because in the $\nrobots = 8$ case, this equates to each robot taking at most 2 sets of measurements.
With a complete budget, more robots (i.e., more steps) leads to better performance as well, as expected. 
What is notable is that, although we see similar median errors for all cases, the improvement in maximum error is also observed when the total path length is held constant.
Given these results, it appears that having more robots, even with restricted budgets (e.g., time, path length), is preferable to having one robot with a larger budget.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Team Size and Communication}

\begin{figure}
  \centering
    % Comms, aggregate
  \includegraphics[width=\boxwidth,height=\boxheight]{multirobot_figures/boxplots/comms_all-expts,RMSE-measuredYs.pdf}
    % Comms, by N
  \includegraphics[width=\boxwidth,height=\boxheight]{multirobot_figures/boxplots/comms_all-expts_bynrobots,RMSE-measuredYs.pdf} 
  \caption{
  \textbf{Error vs. Communication type.}
  Left: Aggregated across different $\nrobots$.
  Note that results for $\nrobots = 1$ are not included, since they are not affected by the variations.
  Right: Same results, further separated by team size. $\nrobots=1$ included for comparison.
  % Bars above indicate significance under the one-sided Wilcoxon signed-rank test; **: $\ppsig$, *: $\psig$, ns: no significance.
  }
  \label{fig:comms}
\end{figure}


\Cref{fig:comms} shows the quantile estimation error results when the robot team uses different communication styles. 
Note that on the right, we include the single robot version as a baseline.

On the left, we see that overall, 
all communication types have a median performance around the same as no communication.
We see that more communication does, however, lead to improved performance, indicated by smaller upper quartile errors. 
This is likely due to the fact the robots can avoid multiple measurements of locations that are not of interest.

% On the right, we see that, in general, communication and partitioning do not have much of an effect for $\nrobots= 2$ or $4$, as seen in the similar median and worst case performance.
On the right, we see that stochastic communication does not have much of an effect compared to no communication when $\nrobots= 2$ or $4$, as seen in the similar median and upper quartile errors.
At $\nrobots = 8$, we see that although the median performance between no, stochastic, and full communication is similar,  both the upper quartile error and the maximum error for no communication is much higher. 
This suggests that enabling communication is more beneficial for larger teams for reducing error and improving performance.
% We also see that the median and worst case error for partitioning is significantly lower, suggesting that partitioning is only an effective strategy for large teams.
We also see that in general, partitioning achieves similar median error as when there is stochastic or full communication, as well as maximum error particularly for larger teams. 
Given that in this experiment, the partitioned case used $\spread = 1.0$ rather than $0.66$, this suggests that partitioning the space is an effective strategy if the entire area is accessible for deploying robots but communication is not possible.
Based on these results, performance improvement can be achieved by enabling inter-robot communication, even when the communication is imperfect, and it is particularly beneficial with large teams.


% Raster Plots
Finally, we show some example plans produced during these experiments as a visualization of the task in \Cref{fig:raster-increase-budget,,fig:raster-shared-budget,,fig:raster-partition}.
The robots are shown in different colors and the paths they produce are shown as connected crosses.
The initial locations are marked in black. If the robots were partitioned, the assigned regions are designated with white lines.
The background of the figures is the orthomosaic of the hyperspectral images
previously collected by drones in real aquatic environments.

\begin{figure}
  \centering
  % Does increasing budget result in longer paths?
  % N=4. B=10 vs B=30.
  \includegraphics[trim={0.5cm 3cm 0.5cm 3.5cm}, clip, width=\boxwidth]{multirobot_figures/rasters/budget_all-expts_EnvA_Extrema_step40_a0.66_c1e-08_seed0_N4_comms3Stochastic_Parallel_Independent__visitedsensedraster.pdf}
  \includegraphics[trim={0.5cm 3cm 0.5cm 3.5cm}, clip, width=\boxwidth]{multirobot_figures/rasters/budget_all-expts_EnvA_Extrema_step120_a0.66_c1e-08_seed0_N4_comms3Stochastic_Parallel_Independent__visitedsensedraster.pdf}
  \caption{
  Example paths of a four-robot team with $B_T=10$ (left) and $B_T=30$ (right).
  % Visited robot locations are shown as colored crosses, start location indicated in black, and the background is the hyperspectral image of the lake environment.
  }
  \label{fig:raster-increase-budget}
\end{figure}


\begin{figure}
  \centering
  % Shared budget path comparison -  one longer path vs. many short paths
  % Shared budget. N=1 vs. N=8
  \includegraphics[trim={0.5cm 3cm 0.5cm 3.5cm}, clip, width=\boxwidth]{multirobot_figures/rasters/parallel_all-expts_EnvA_Extrema_step15_a0.66_c1e-08_seed0_N1_comms2None_Parallel_Independent__visitedsensedraster.pdf}
  \includegraphics[trim={0.5cm 3cm 0.5cm 3.5cm}, clip, width=\boxwidth]{multirobot_figures/rasters/parallel_all-expts_EnvA_Extrema_step15_a0.66_c1e-08_seed0_N8_comms3Stochastic_Serial_Independent__visitedsensedraster.pdf}
  \caption{
  Example paths of a single robot with $B_T=15$ (left) and an 8-robot team with a shared budget of $B_T=15$ (right).
  % Visited robot locations are shown as colored crosses, start location indicated in black, and the background is the hyperspectral image of the lake environment.
  }
  \label{fig:raster-shared-budget}
\end{figure}

\begin{figure}
  \centering
  % How do Partition and No communication compare? do non-communicating teams overlap organically? (yes as seen in other plots but compare directly to partition)
  % Alpha=1.0. Partition vs. No comms
  \includegraphics[trim={0.5cm 3cm 0.5cm 3.5cm}, clip, width=\boxwidth]{multirobot_figures/rasters/comms_all-expts_EnvA_Extrema_step120_a1.0_c1e-08_seed0_N8_comms1Partitioned_Parallel_Independent_Partition_visitedsensedraster.pdf}
  \includegraphics[trim={0.5cm 3cm 0.5cm 3.5cm}, clip, width=\boxwidth]{multirobot_figures/rasters/alpha_all-expts_EnvA_Extrema_step120_a1.0_c1e-08_seed0_N8_comms2None_Parallel_Independent__visitedsensedraster.pdf}
  \caption{
  Example paths of an 8-robot team under partitions (left) and no communication (right).
  % Visited robot locations are shown as colored crosses, start location indicated in black, and the background is the hyperspectral image of the lake environment.
  }
  \label{fig:raster-partition}
\end{figure}


\section{Discussion}
We now summarize the main conclusions drawn from the presented results and discuss further areas of interest based on them.

With regards to the initial location spread, a large spread appears to be beneficial when $\nrobots$ is large, but not when $\nrobots$ is small.
Additionally, past a certain point between $0.33$ and $0.66$, a larger spread results in marginal improvement in error.
This may be particularly valuable information when planning real-world field deployments, when there are time and monetary costs to getting many robots to spatially diverse areas; avoiding unnecessary costs is crucial.
In addition, if $\spread$ is restricted to very low values by the survey resources or setup, then using more robots may help regain some performance.

Notably, in terms of budget $B_T$, a larger budget in and of itself does not significantly improve performance for a fixed $\nrobots$ (assuming a moderate initial spread). What we observe instead is a stronger dependency on $\nrobots$ itself; therefore, a larger number of robots, each with a restricted budget, will likely produce better quantile estimates than a single robot with a $B_T$ equal to the total budget of all of them.

Our results also indicate that enabling communication is generally beneficial to the quantile estimation problem, and in particular for larger groups. 
We note that partitioning the space into disjoint areas and restricting each robot to one area can be an effective alternative strategy,
particularly if inter-robot communication is not an option.

Looking forward, we would like to further investigate the role that communication plays in this task.
For the purposes of this study, we restricted the communication frameworks to somewhat basic implementations; it would be interesting to consider how results may change given a more intelligent communication protocol that takes into account the potential utility of a message, or with more nuanced communication models based on particular hardware capabilities.

We are also interested in how this scales to team sizes beyond 8 robots.
In the context of lake monitoring for algae and other environmental monitoring tasks, swarms are not typically deployed;
however, for large-scale studies, it may be useful to understand the impact of teams larger than 8.
Based on our results in this study, we would expect to see lower error with more robots up to a certain point. 
Our results support what previous work has found in terms of diminishing returns with more robots.
We generally observe a larger decrease in error between $\nrobots = 2$ and $4$ than between $4$ and $8$.
Extrapolating from this, doubling $\nrobots$ from $8$ to $16$ robots or more would likely not be able to achieve 0 error, but would be significantly more resource-intensive.

In practice, scientist teams will need to weigh the benefit of lower estimation error with the practicality of acquiring, coordinating, and deploying more robots for their specific application.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% The following command should be issued somewhere in the first column 
%%% of the final page of your paper.
% \balance

\section{Conclusion}
In this work, we have presented the first study on multirobot quantile estimation
for environmental analysis. We investigate the impact of multiple robots on
quantile estimation accuracy, as well as the effect of initial location spread, planning budget, and communication.
We measure how well different combinations of parameters perform in terms of error in quantile value estimates, 
and we further provide statistical results quantifying the significance of the differences observed.
This work is an important step toward characterizing the elements of an effective
multirobot system for environmental analysis and has potential to help
scientists interested in larger scale or collaborative survey projects to better
understand the benefits and drawbacks of different experiment design choices. In
turn, this may improve environmental monitoring and conservation
efforts.



==> psm.tex <==
\section{Introduction}
\label{sec:psm_introduction}
% motivation
Sampling-based motion planning (SBMP) considers the problem of finding a collision-free path from a start configuration to a goal configuration. Probabilistic roadmaps \cite{kavraki1994randomized} or rapidly exploring random trees \cite{lavalle1998rapidly} generate plans for such motions while providing theoretical guarantees regarding probabilistic completeness. Optimal algorithms like RRT$^*$ \cite{karaman2011sampling} additionally minimize a cost function and achieve asymptotic optimality. However, many tasks in robotics 
%have a more complex structure that 
require the incorporation of additional objectives like subgoals or constraints.
%into the planning problem. 
%
SBMP methods are difficult to directly apply to such problems because they require splitting the overall task into multiple planning problems that fit into the SBMP structure.
%
A disadvantage of this approach is that a goal in the configuration space needs to be specified for each subtask, and each selected subgoal will affect the future subtasks. 
%
%\remove{Task and motion planning (TAMP) is a common way to address such more complex problems} \cite{kaelbling2013integrated, hauser2011randomized, toussaint2018differentiable}. \remove{TAMP algorithms plan collision-free paths and also reason about selecting and ordering actions to complete a higher-level task, which makes them more difficult to solve than SBMP problems.}
%

We consider a %problem 
formulation for sequential motion planning where a problem is represented as a fixed sequence of manifolds.
% This formulation is based on the more general multi-modal problem structure proposed by \cite{hauser2011randomized} where each manifold describes a subgoal or constraint. 
% and we require that the robot traverses this sequence in order to solve the overall task.
% why is the problem important / why can't current methods solve it
%\remove{State-of-the-art trajectory optimization methods} \cite{toussaint2017newton, schulman2013finding, ratliff2015understanding} \remove{can handle task descriptions via costs and constraints. However, they strongly depend on the path initialization and suffer from poor local optima for long-horizon tasks.}
\begin{figure}[t]
	\centering
 	\includegraphics[width=.4\textwidth]{psm_graphics/hourglass.png}
	\caption{3D Point on Geometric Constraints -- The surfaces visualize the level sets of the three constraints. The task is to move from the start point (red dot) to the goal point (blue dot) while fulfilling the constraints. The line shows a solution found by \smp~that fulfills these constraints and the magenta points are the found intersection vertices.}
	\label{fig:psm_hourglass}
% 	\vspace{-0.25in}
\end{figure}
% assumptions and summary of our method
We propose \smplong~(\smp), an algorithm that searches for an optimal path that starts at an initial configuration, traverses the manifold sequence, and converges when the final manifold is reached. 
%We solve this problem by growing a single tree over the manifold sequence. 
Our solution is to grow a single tree over the manifold sequence.
This tree consists of multiple subtrees that originate at the intersections between pairs of manifolds. We propose a novel steering strategy that guides the robot towards these manifold intersections. After an intersection is reached, a new subtree is initialized with the found intersection points and their costs. 
%This approach allows us to use dynamic programming over optimal intersection points and %scales well to long horizon tasks since a new subtree is initialized for every manifold. 
We use dynamic programming over optimal intersection points which scales well to long horizon tasks since a new subtree is initialized for every manifold.
The algorithm is applicable to a class of problems we call \emph{intersection point independent}, specified by a property which restricts how the free configuration space changes across subtasks (see \sect \ref{sec:problem_formulation}).

% Example task and manifold sequence 
A running example in this paper is the task of using a robot arm to transport a mug from one table to another while keeping the orientation of the mug upright, a task involving multiple phases and constraints described informally as follows.
First, the arm moves to pick up the mug. In this subtask, the arm can move freely in space and only needs to avoid collisions with obstacles. The second subtask is to grasp the mug. The third subtask is for the arm to transfer the mug with the constraint of always keeping the mug upright. The final subtask is to place and release the mug which requires the base of the mug to be near the table. 
%for the gripper to successfully release the mug. 
In \sect \ref{sec:psm_experiments}, we demonstrate the performance of \smp~on similar sequential kinematic planning problems that involve multiple robots and compare it to alternative planning strategies.

% contributions
% \begin{itemize}
%     \item identification of the problem class of intersection point independent motion planning problems (\sect \ref{sec:problem_formulation}), which is a subclass of the more general multi-modal motion planning problem \cite{hauser2011randomized}, 
%     \item  an algorithm, \smp, 
%     that explores intersection points reachable from the start by growing a single tree over a given sequence of manifolds (\sect \ref{sec:method}),
%     \item experimental evaluation of our method on various transportation tasks involving multiple robots and on a pouring task with a real Panda robot (\sect \ref{sec:psm_experiments}), and comparisons to other methods,
%     \item proofs of probabilistic completeness and asymptotic optimality (\sect \ref{ssec:comp-optimal}) of \smp.
% \end{itemize}

\subsection{Background}
Our proposed method builds on the methods introduced in \Cref{ch:motion-planning-background} and extends them towards sequential tasks where the active constraints change during the motion.
We use a modified version of RRT$^*$ in the inner loop of \smp~that can handle goals defined in terms of equality constraints instead of a goal configuration. 
Restricting the problem class to intersection point independent problems (\sect \ref{ssec:ipip}) allows us to grow a single tree over a sequence of manifolds on which rewiring operations can still be performed. 
We show that \smp~inherits the probabilistic completeness and asymptotic optimality guarantees of RRT$^*$ (\sect \ref{ssec:comp-optimal}).
%Our procedure is used to solve sequential motion planning problems where the free space changes throughout the motion.

Our approach is perhaps closest to the CBiRRT algorithm. 
A main difference is that our method assumes a different problem formulation where the task is given in terms of a fixed sequence of manifolds where the intersections between manifolds describe subgoals that the robot should reach. 
This formulation allows us to define a more structured steering strategy that guides the robot towards the next subgoals. 
Another difference is that CBiRRT does not search for optimal paths, while we employ RRT$^*$ to minimize path lengths. We compare our method \smp~to CBiRRT in \sect \ref{sec:psm_experiments}.

Our work also shares similarities with others in the task and motion planning (TAMP) problem area, in that we consider planning over multiple manifolds where changes in the configuration space occur due to picking or placing objects. 
However, our work differs in several key ways. First, TAMP approaches assume the task sequence is unknown in advance, and thus selecting the transition to the next constraint is part of the planning problem. Here we specify our problem formulation over a fixed and known sequence of constraints, focusing our algorithm on optimizing the transition points between constraints to find an optimal path. 
Additionally, we do not assume direct sampling of modes or switches is possible; rather, our algorithm is designed to find the mode-switching configurations during exploration toward manifold intersections. 
Importantly, because we build one search tree, these configurations are guaranteed to be connected to the start. This eliminates sampling of configurations that are disconnected from the viable solution space.
Further, we differ by applying \smp~in the domain of intersection point independent problems, 
which we specify for sequential planning problems based on the free space transformation at each manifold intersection (\sect \ref{ssec:ipip}).
These problems do not include foliated manifolds and are efficiently solvable by growing a single tree.

Finally, in contrast to trajectory optimization, our approach only requires the sequential order of tasks and does not make any assumption of specific time points or durations of subtasks.

\section{Problem Formulation and Application Domain}
\label{sec:problem_formulation}
We consider kinematic motion planning problems in a configuration space $C\subseteq \R^k$. A configuration $q\in C$ describes the state of one or multiple robots with $k$ degrees of freedom in total. 
%
We represent a manifold $M$ as an equality constraint $h_{M}(q)=0$ where $$h_{M}(q) : \R^{k} \to \R^{l}$$
and $l$ is the intrinsic dimensionality of the constraint ($l \leq k$). The set of robot configurations that are on a manifold $M$ is given by $$C_{M} = \{q\in C ~|~ h_{M}(q) = 0\}\period$$
%
We define a projection operator $$q_\t{proj} =  \textit{Project}(q, M)$$
that takes a robot configuration $q\in C$ and a manifold $M$ as inputs and maps $q$ to a nearby configuration on the manifold $q_\t{proj}\in C_M$. 
We use an iterative optimization method, similar to \cite{kingston2019ijrr, berenson2011task, stilman2007task}, that iterates 
$$q_{n+1} = q_n - J_{M}(q_n)^+ h_{M}(q_n)$$
until a fixed point on the manifold is reached, which is checked by the condition $||h_M(q_\t{proj})|| \leq \ge$. The matrix $J_{M}(q)^+$ is the pseudo-inverse of the constraint Jacobian $$J_{M}(q) = \frac{\partial }{\partial q} h_{M} (q)\period$$

We are interested in solving tasks that are defined by a sequence of $n+1$ such manifolds 
$\mathcal{M} = \{M_1, M_2, \dots, M_{n+1}\}$
\new{where the number and order of manifolds is given,} and an initial configuration $q_\t{start}\in C_{M_1}$ that is on the first manifold.
%
The goal is to find a path from $q_\t{start}$ that traverses the manifold sequence $\mathcal{M}$ and reaches a configuration on the goal manifold $M_{n+1}$.
%
A path on the $i$-th manifold is defined as $$\tau_i : [0, 1] \to C_{M_i}$$
and $J(\tau_i)$ is a cost function of a path
$${J} : \mathcal{T} \to \R_{\geq 0}$$
where $\mathcal{T}$ is the set of all non-trivial paths. 

In the following problem formulation, we consider the scenario where the free configuration space $C_\t{free}$ changes during the task (e.g., when picking or placing objects).
%
We define an operator $\Upsilon$ on the free configuration space $C_\t{free}$, which describes how $C_\t{free}$ changes as manifold intersections are traversed. 
$\Upsilon$ takes as input the \new{endpoint of a} path $\tau_{i-1}(1)$ on the previous manifold $M_{i-1}$ and its associated $C_\t{free}$, which we denote as $C_{\t{free}, i-1}$. $\Upsilon$ outputs an updated free configuration space 
$$C_{\t{free}, i} = \Upsilon(C_{\t{free}, i-1}, \tau_{i-1}(1))$$
that accounts for the geometric changes due to transitioning to a new manifold. 
\new{Here, we assume these changes only occur at the transition between two manifolds.}
\new{We define $\Upsilon$ in this way rather than with the configuration spaces of the robot and the objects in the environment because our formulation does not have a notion of ``objects"; any object in the world is either an obstacle, or it becomes part the robot system itself.}
% The $q$ superscript refers to the fact that the free space for paths on a manifold $M_{i}$ depends on the geometry of the robot, which may be different depending on which configuration $q$ was traversed during the previous intersection (i.e., the first point of $\tau_i$).
% For simplicity, we may omit the $q$ superscript when $C_{\t{free}, i}$ is accompanied by a path $\tau$ (and thus the $q$ is implied) or if a particular geometry is not specified for that manifold (in which case $q$ is not meaningful).
% Note that the final configuration $q_i = \tau_i[0] = \tau_{i-1}[1]$ of the path is on both $M_i$ and the previous manifold $M_{i-1}$, since we use the operator on manifold intersections.
%

We assume access to a collision check routine
$$\textit{CollisionFree}(q_a, q_b, C_{\t{free}, i}) \to \{0,1\}$$ that returns $1$ if the path between two configurations on the manifold $q_a, q_b \in C_M$ is collision-free, $0$ otherwise. Note that here, we use the straight-line path in ambient space between two nearby points. 
However, other implementations for the collision check are possible, such as a path on the manifold.

%$$\textit{CollisionFree} ~:~C_{M} \times C_{M} \to \{0,1\}$$ that returns $1$ if the path between two configurations on the manifold is collision-free, $0$ otherwise.

 % which is consistent with the constraints defined by ${M}_{i}$ and with the configuration specified by $q_i = \tau_i[0]$.
% In general, $C_\t{free}$ may change arbitrarily from $i$ to $i+1$, as traversing to a new manifold may represent changing the geometry of the robot arbitrarily, e.g. by requiring that the robot pick up or put down an object.
% We assume that when an object is grasped, it becomes a rigid addition to the rest of the robot body geometry.
Returning to our illustrative example, we can now describe one of its constraints more precisely. A simple grasp constraint can be described with \mbox{$h_M(q) = x_g - f_{\t{pos}, e}(q)$} where $f_{\t{pos}, e}$ is the forward kinematics function of the robot end effector point $e$ and $x_g$ is the grasp location on the mug. 
This constraint can be fulfilled for multiple robot configurations $q$, which correspond to different hand orientations that will affect the free configuration space for the subsequent tasks. For example, a mug grasped from the side will have a different free space during the transport phase than a mug grasped from the top. 


% Here, the robot has $k$ degrees of freedom, the goal location is $x_g$, and $x_g$ and $x_b$ are the forward kinematics of the gripper and the mug, respectively:
% \begin{enumerate}
%     \item Free motion; $q \in \R ^n$ 
%     \item Gripper grasps mug; $h(q) = \mat{c}{||x_g - x_b|| \\ \theta(x_b) \\ \psi(x_b)}$ 
%     \item mug sits on 2$^\t{nd}$ table; $h(q) = ||x_b - x_t||$
%     \item Free motion; $q \in \R ^n$
% \end{enumerate}

\subsection{Problem Formulation}
We formulate an optimization problem over a set of paths $\v\tau = (\tau_1, \dots, \tau_{n})$ that minimizes the sum of path costs under the constraints of traversing $\mathcal{M}$ and of being collision-free. The \emph{planning on sequenced manifolds problem} is
\begin{align} %
	\begin{alignedat}{2} %	
	\label{eq:smp_problem}
	\v\tau\opt =~ &\argmin{\v\tau} \sum_{i=1}^n J(\tau_i) &&\\
	\text{s.t.}\quad &\tau_1 (0) = q_\t{start} &\\
	&\tau_i(1) = \tau_{i+1}(0)  &&\forall_{i=1,\dots,n-1} \\ 
	&C_{\t{free}, i+1} = \Upsilon(C_{\t{free}, i}, \tau_{i}(1))~~~~ &&\forall_{i=1,\dots,n}\\
	&\tau_i(s) \in C_{M_i} \cap C_{\t{free}, i} &&\forall_{i=1,\dots,n}~ \forall_{s \in [0, 1]}\\
	&\tau_{n}(1) \in C_{M_{n+1}} \cap C_{\t{free}, n+1} &&
	\end{alignedat} %
\end{align}
The second constraint ensures continuity such that the endpoint of a path $\tau_i(1)$ is the start point of the next path $\tau_{i+1}(0)$. The third constraint captures the change in the collision-free space defined by the operator $\Upsilon$. The last two constraints ensure that the path is collision free and on the corresponding manifolds. The endpoint of $\tau_{n}$ must be on the goal manifold $M_{n+1}$, which denotes the successful completion of the task.
\new{Note that this problem can be seen as a special case of the multi-modal motion planning problem presented in \cite{hauser2011randomized} where the manifolds are provided in their sequential order.}

\new{There are several advantages to formulating the problem with manifolds in this way.} 
One is that it is not necessary to choose a specific target configuration in $C$ and thus a wider range of goals 
%(e.g., in the robot end effector space) 
can be described in the form of manifolds. 
Another is that it is possible to describe complex sequential tasks in a single planning problem, not requiring the specification of subgoal configurations. 
The algorithm proposed in \sect \ref{sec:method} searches for a path that solves this optimization problem for the problem class described in the next section.

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{psm_graphics/tree_initialization.pdf}
    \caption{Initialization of a new subtree (steps \ref{alg:newtreeinit_start}--\ref{alg:newtreeinit_end} of \alg \ref{alg:smp}). The reached goal nodes at the intersection $M_1\cap M_2$ are used to initialize the next tree where $q_\t{root}$ is a synthetic root node that maintains the tree structure.}
    \label{fig:tree_init}
    % \vspace{-0.25in}
\end{figure}

\subsection{Intersection Point Independent Problems}
\label{ssec:ipip}
We now use the problem formulation in 
\eqref{eq:smp_problem} to describe robotic manipulation planning problems in which the manifolds describe subtasks for the robot to complete (e.g., picking up objects). The solution is an end-to-end path across multiple manifolds.
%
% In manipulation tasks, geometry commonly changes throughout the motion due to picking or placing objects. Here, we assume these changes only occur at the transition between two manifolds. For example, changing the grasp of a mug would only occur at points during the task when it is picked up or placed.

% Note that though there is no part of the formulation that prevents defining the free space operator $\Upsilon$ for two consecutive parts of any trajectory whose common point does not bridge a manifold intersection, the only nontrivial transformations of $C_\t{free}$ occur during these bridges, and thus in this work we will always assume $\Upsilon$ to be referring to such an instance.


For a certain class of sequential manifold planning problems, the following property holds: For each manifold intersection \mbox{${M}_{i} \cap {M}_{i+1}$}, the free space output by $\Upsilon$ is set-equivalent for every possible path $\tau_{i}$. In other words, the precise action taken to move the configuration from one constraint to the next does not affect the feasible planning space for the subsequent subtask. When this property holds for all intersections, we call the problem \emph{intersection point independent}. The condition for this class of problems is
\begin{align}
	\begin{alignedat}{2} %	
		\label{eq:ip_independence}
		&\forall i \in [0, n] ~\forall \tau_i, \tau_i' \in \mathcal{T} : \tau(1), \tau'(1) \in C_{M_i} \cap C_{M_{i+1}} \\
		&\Rightarrow\Upsilon(C_{\t{free}, i}, \tau(1)) \equiv \Upsilon(C_{\t{free}, i}, \tau'(1))
	\end{alignedat}
\end{align}
where $\equiv$ denotes set-equivalence. In this work, we focus on the intersection point independent class of motion planning problems, which encompass a wide range of common problems.
For grasping constraints, a notion of object symmetry about the grasp locations results in intersection point independent problems. If the object to be grasped is a cylindrical can, for example, allowing grasps to occur at any point around the circumference but at a fixed height would be intersection point independent. Any two grasps with the same relative orientation of the gripper result in the same free configuration space of the system (robot + can).
However, suppose the grasps can occur at any height on the can. Now, a grasp near the top of the can and a grasp in the middle of the can result in different free configuration spaces, and thus this would be an intersection point dependent problem.

Focusing on intersection point independent problems allows us to define an efficient algorithm that grows a single tree over a sequence of manifolds. The more general intersection point dependent problem covers a wider class of problems. However, they are more difficult to solve because they require handling foliated manifolds \cite{kim2014randomized} (e.g., every grasp leads to a different manifold). 
Our illustrative example is one such problem, since the grasp on the handle and the grasp from the top of the mug result in different free spaces. We plan to address this more complex problem class in future work and provide some insights in \sect \ref{sec:psm_conclusion} how the proposed algorithm could be used to tackle them.




\section{\smplong}
\label{sec:method}
% \begin{figure}[t]
% 	\centering
% \begin{tabular}{|c|l|}
% 	\hline
% 	\textbf{Symbol} & \textbf{Description}\\
% 	\hline
% 	$\ga$ & Max step size of an edge in the tree\\
% 	$\gb$ & Probability of SteerConstraint step\\
% 	$\gr$ & Min distance between intersection nodes\\
% 	$\ge$ & Threshold for a point to be on a manifold\\
% % 	$\gd$ & Collision check resolution\\
% 	$r$ & Max manifold intersection projection distance\\
% % 	$\gg_\t{RRT*}$ & RRT$^*$ rewiring parameter\\
% 	\hline
% \end{tabular}
% \caption{Algorithm parameters and their description.}
% \label{tab:parameter}
% % \vspace{-0.25in} 
% \end{figure}
We now present the algorithm \smp~that solves the problem formulated in \eq \eqref{eq:smp_problem} \new{for tasks that fulfill the intersection point independent property defined in \eq \eqref{eq:ip_independence}}.
The algorithm searches for an optimal solution to the constrained optimization problem, which is a sequence of paths $\v\tau = (\tau_1, \dots, \tau_{n})$ where each $\tau_i$ is a collision-free path on the corresponding manifold $M_i$. 

The steps of \smp~are outlined in \alg \ref{alg:smp}.
The input to the algorithm is a sequence of manifolds $\mathcal{M}$, an initial configuration \mbox{$q_\t{start}\in M_1$} on the first manifold, 
\new{and the hyperparameters of the algorithm $(\ga, \gb, \gr, \ge, r, m)$ (see Table \ref{tab:exp_parameter}).
$V, E$ are the vertices and edges, respectively, in the tree that the algorithm builds, while $C$ is the robot configuration space and $C_{\t{free}, 1}$ is the initial free configuration space.}

The overall problem is divided into $n$ subproblems, \new{which correspond to the number of manifold intersections in $\mathcal{M}$.} Each subproblem \new{can be broadly thought of as growing a tree between two consecutive manifold intersections.} We give a high-level summary here.
In the inner loop (lines \ref{alg:innerloop_start}--\ref{alg:innerloop_end}; see \sect \ref{ssec:phase12}), a tree is iteratively grown from a set of initial nodes toward the intersection with the next manifold.
First, a new constraint-adhering configuration $q_\t{new}$ is found by sampling a point, steering, and projecting it (steps \ref{alg:steer_start}--\ref{alg:steer_project_step}).
Second, in steps \ref{alg:check_proj}--\ref{alg:extend_end}, the point is checked for validity before being added to the tree as well as the set of intersection points (if applicable).
\new{After the inner loop completes}, the algorithm initializes the next subproblem with the found intersection points in steps \ref{alg:newtreeinit_start}--\ref{alg:next_freespace} (see \sect \ref{ssec:phase3}). It returns the optimal path that traverses all manifolds in $\mathcal{M}$.

% The overall problem is divided into $n$ subproblems. In each subproblem $i$, a tree is grown from a set of initial nodes toward the intersection of the current and next manifold $M_i \cap M_{i+1}$.
%The inner loop of the algorithm  is similar to RRT$^*$. 
%The main differences with respect to RRT$^*$ are in the extension and projection steps, as described below.



\subsection{Inner Loop: Growing a Tree to the Next Manifold}
\label{ssec:phase12}
The first phase of the inner loop focuses on producing a new candidate configuration $q_\t{new}$ which lies on the constraint manifold $M_i$ and adding it to the tree. 
The \smp \_STEER routine in \alg \ref{alg:steer_project} computes $q_\t{new}$.
%
Instead of targeting a single goal configuration as in general SBMP, we propose two novel steering strategies that steer toward the intersection between manifolds $M_i\cap M_{i+1}$. 
In steps \ref{alg:steer_start}--\ref{alg:steer_end} of \alg \ref{alg:smp}, a new target point $q_\t{rand}$ in the configuration space is sampled and its nearest neighbor $q_\t{near}$ in the tree is computed. Next, in \alg \ref{alg:steer_project} one of the following two steering strategies is selected to find a direction $d$ in which to extend the tree:
% \begin{enumerate}
%     \item \new{$\t{\textbf{SteerPoint}}(q_\text{near}, q_\text{rand}, M_i)$} extends the tree from \mbox{$q_\text{near}\in C_{M_i}$} towards $q_\text{rand}\in C$ while staying on the current manifold $M_i$.
%     \item \new{$\t{\textbf{SteerConstraint}}(q_\text{near}, M_i, M_{i+1})$} extends the tree from $q_\text{near}\in C_{M_i}$ towards the intersection of the current and next manifold $M_i\cap M_{i+1}$.
% \end{enumerate}

% \subsection{$\t{SteerPoint}(q_0, q_1, M_i)$}
\subsubsection{\new{$\t{SteerPoint}(q_\t{near}, q_\t{rand}, M_i)$}}
\label{sec:steer_point}
In this extension step, the robot is at $q_\t{near}\in C_{M_i}$ and should step towards the target configuration $q_\t{rand}\in C$ while staying on the manifold $M_i$. We formulate this problem as a constrained optimization problem of finding a curve $\gg ~:~ [0,1]\to C$ that
\begin{align}
    \begin{alignedat}{2}
    	&\minimize{\gg} &&||\gg(1) - q_\t{rand}||^2\\
		&\subjectto~~&&\gg(0) = q_\t{near},\quad \int_{0}^1 ||\dot{\gg}(t)|| ~\mathrm{d}s \leq \ga\\
		& & &h_{M_i}(\gg(s)) = 0 \quad\qquad \forall~ s\in [0,1]
	\label{eq:steer_point}
	\end{alignedat}
\end{align}
% $$\min{\gg} ||\gg(1) - q_\t{rand}||^2$$ \st $$\gg(0) = q_\t{near}, h_{M_i}(\gg(s)) = 0$$ $$\quad \forall~s\in [0,1] \quad and 
% 	\int_{0}^1 ||\dot{\gg}(s)|| ~ds \leq \ga$$ \label{eq:steer_point}\\
This problem is hard to solve due to the nonlinear constraints. Since the steering operations are called many times in the inner loop of the algorithm, we choose a simple curve representation and only compute an approximate solution to this problem. We parameterize the curve as a straight line $\gg(s) = q_\t{near} + s\ga \frac{d}{||d||}$ with length $\ga$
\new{where the direction $d$ is chosen as orthogonal projection of $q_\t{rand}-q_\t{near}$ onto the tangent space of the manifold at $q_\t{near}$.}
We apply a first-order Taylor expansion of the manifold constraint $h_{M_i}(q_\t{near} + d) \approx h(q_\t{near}) + J_{M_i}(q_\t{near}) d$, which reduces the problem to
%The problem is reduced to finding a direction $d$ that
% \begin{align}
% 	\min{d} \frac{1}{2} ||q_\t{near} + d - q_\t{rand}||^2 \qquad
% 	\st\quad h_{M}(q_\t{near} + d) = 0\period
% \end{align}
%  to get the simplified problem 
\begin{align}
	\begin{alignedat}{3}
	&\minimize{d} &&\frac{1}{2} ||d  - (q_\t{rand}-q_\t{near})||^2\\
	&\subjectto~~ &&J_{M_i}(q_\t{near}) d = 0
	\end{alignedat}
\end{align}
The optimal solution of this problem is
\begin{align}
	% a=0, A=J, b=(q_n-q_\t{near}), B=I, \mathcal{B}=I, X=I, x=(q_n-q_\t{near})\\
	% \gd=(I - X\inv A\T (AX\inv A\T)\inv A) X\inv x\\
	\begin{alignedat}{2}
	d &=(I -  J_{M_i}\T (J_{M_i} J_{M_i}\T)\inv J_{M_i}) (q_\t{rand}-q_\t{near})\\
	&= V_{\bot} V_{\bot}\T (q_\t{rand}-q_\t{near})
	\label{eq:steer_point_sol}
	\end{alignedat}
\end{align}
where $V_{\bot}$ contains the singular vectors that span the right nullspace of $J_{M_i}$ \cite{ratliff2014multivariate}. We normalize $d$ later in the algorithm, and thus do not include the constraint $||d||\leq \alpha$ in the reduced optimization problem. The new configuration $q_\t{near} + \alpha \frac{d}{||d||}$ will be on the tangent space of the manifold at configuration $q_\t{near}$, so that only few projection steps will be necessary before it can be added to the tree. \new{Note that projection may fail to converge, and if this occurs the sample is discarded.}


\begin{algorithm}[t]
\begin{algorithmic}[1]
	\algrenewcommand\algorithmicindent{1.5em}%
	\State $V_1 = \{q_{\t{start}}\}$; $E_1 = \emptyset$; $n=\text{len}(\mathcal{M})-1$
% 	\State Initialize $C, C_{\t{free}, 1}$
	\For{$i=1$ to $n$}
		\State $V_\t{goal} = \emptyset$
		\For{$k = 1$ to $m$} \label{alg:innerloop_start}
			\State $q_\t{rand} \leftarrow \t{Sample}(C)$  \label{alg:steer_start}
			\State $q_\t{near} \leftarrow \t{Nearest}(V_i, q_\t{rand})$
			\State{$q_\t{new} \leftarrow \t{\smp\_STEER} (\alpha, \beta, r, q_\t{near}, M_i, M_{i+1}$)} \label{alg:steer_project_step}
% 	\State{\new{// check if projection was successful}} 
	\If{\new{$||h_{M_{i}} (q_\t{new})|| > \ge$}} \label{alg:check_proj}
	    \State continue
	\EndIf
			\If{RRT$^*$\_EXTEND$(V_i, E_i, q_\text{near}, q_\text{new}, C_{\text{free},i})$} \label{alg:extend_start}
				\If{$||h_{M_{i+1}} (q_\t{new})|| < \ge$ \label{alg:next_manifold} \textbf{and}\\ $\hspace{5.5em} ||\t{Nearest}(V_\t{goal}, q_\t{new}) - q_\t{new}|| \geq \gr$} \label{alg:avoid_duplicates}
					\State $V_\t{goal} \leftarrow V_\t{goal} \cup q_\t{new}$
				\EndIf
			\EndIf \label{alg:extend_end}
			% \If{$\t{CollisionFree}(q_\t{near}, q_\t{new}, \gd)$}
				% \State $V_t \leftarrow V_t \cup \{q_{\t{new}} \},\quad E_t \leftarrow E_t \cup \{(q_\t{near}, q_\t{new} )\}$
			% \EndIf
        \EndFor \label{alg:innerloop_end}
		% \vspace{.3em}
% 		\State{// return path with lowest cost when $M_{n+1}$ is reached}
% 		\If{$i=n$}
% 			\State \textbf{return} $\mathrm{OptimalPath}(V_{1:n}, E_{1:n}, q_\t{start}, M_{n+1})$
% 		\EndIf
		% \vspace{.3em}
		\State{// initialize next tree with the intersection nodes}
		\State $q_\t{root}=\t{null}, V_{i+1} = \{q_\t{root}\}; E_{i+1}=\emptyset$ \label{alg:newtreeinit_start}
		\For{$q \in V_\t{goal}$}
			\State $V_{i+1} \leftarrow V_{i+1} \cup \{q \}; E_{i+1} \leftarrow E_{i+1} \cup \{(q_\t{root}, q )\}$
		\EndFor\label{alg:newtreeinit_end}
% 		\State{\new{// compute free space for next tree}}
% 		\State{\new{$\tau_i \leftarrow \mathrm{OptimalPath}(V_i, E_i, q_\t{root}, M_{i+1})$}}
		\State{\new{$C_{\t{free},i+1} \leftarrow \Upsilon(C_{\t{free},i}, V_\t{goal}[0])$}} \label{alg:next_freespace}
	\EndFor
	\State \textbf{return} $\mathrm{OptimalPath}(V_{1:n}, E_{1:n}, q_\t{start}, M_{n+1})$
\end{algorithmic}
\caption{\smp~$(\mathcal{M}, q_{\t{start}}, \ga, \gb, \ge, \rho, r, m)$}
\label{alg:smp}
\end{algorithm}

\begin{algorithm}[t]
\begin{algorithmic}[1]
	\algrenewcommand\algorithmicindent{1.0em}%
	\If{\new{$\t{Sample}(\mathcal{U}(0,1)) < \gb$}}
		\State $d \leftarrow \t{SteerConstraint}(q_\t{near}, M_i, M_{i+1})$ %\hfill // \eq \eqref{eq:steer_constraint_sol}
		% \State $d \leftarrow -J_{M_{i}}(q_\t{near}) J_{M_{i}}\T(q_\t{near}) J_{M_{i+1}}\T(q_\t{near}) h_{M_{i+1}}(q_\t{near})$
	\Else
		\State $d \leftarrow \t{SteerPoint}(q_\t{near}, q_\t{rand}, M_i)$
		% \State $d \leftarrow J_{M_{i}}(q_\t{near}) J_{M_{i}}\T(q_\t{near}) (q_\t{rand} - q_\t{near})$
	\EndIf
	\State $q_\t{new} \leftarrow q_\t{near} + \alpha \frac{d}{||d||}$ \label{alg:steer_end}
	\If{$||h_{M_{i+1}} (q_\t{new})|| <$ \new{$ \t{Sample}(\mathcal{U}(0,r))$}} \label{alg:project_start}
		\State $q_\t{new} \leftarrow \t{Project}(q_\t{new}, M_{i} \cap M_{i+1})$
	\Else
		\State $q_\t{new} \leftarrow \t{Project}(q_\t{new}, M_{i})$
	\EndIf \label{alg:project_end}
	\State \textbf{return} $q_\t{new}$
\end{algorithmic}
\caption{$\t{\smp\_STEER} (\alpha, \beta, r, q_{\t{near}}, M_i, M_{i+1})$}
\label{alg:steer_project}
\end{algorithm}


\subsubsection{\new{$\t{SteerConstraint}(q_\t{near}, M_i, M_{i+1})$}}
\label{sec:steer_constraint}
This steering step extends the tree from $q_\t{near}\in C_{M_i}$ towards the intersection of the current and next manifold $M_i\cap M_{i+1}$, which can be expressed as the optimization problem
\begin{align}
\begin{alignedat}{2}
	&\minimize{\gg} &&||h_{M_{i+1}}(\gg(1))||^2 \\
	&\subjectto\quad &&\gg(0) = q_\t{near},\quad \int_{0}^1 ||\dot{\gg}(t)|| ~\mathrm{d}s \leq \ga\\ 
	&&&h_{M_i}(\gg(s)) = 0 \quad\qquad \forall~ s\in [0,1]
	\end{alignedat}
\end{align}
The difference from problem \eqref{eq:steer_point} is that the loss is now specified in terms of the distance to the next manifold $h_{M_{i+1}}(\gg(1))$. This cost pulls the robot towards the manifold intersection. Again, we approximate the curve with a line $\gamma(s)$ and apply a first-order Taylor expansion to the nonlinear terms, which results in the simplified problem
\begin{align}
\begin{alignedat}{2}
	&\minimize{d} &&\frac{1}{2}||h_{M_{i+1}}(q_\t{near}) + J_{M_{i+1}}(q_\t{near})d||^2\\
	&\subjectto~~&&J_{M_i}(q_\t{near}) d = 0\period
	\end{alignedat}
\end{align}
A solution $d$ can be obtained by solving the linear system
\begin{align}
    \label{eq:steer_constraint_sol}
    \mat{c c}{J_{M_{i+1}}\T J_{M_{i+1}} & J_{M_{i+1}}\T \\ J_{M_{i}} & 0} \mat{c}{d\\ \gl} = \mat{c}{-J_{M_{i+1}}\T h_{M_{i+1}}\\ 0}
\end{align}
where $\gl$ are the Lagrange variables. The solution is in the same direction as the steepest descent direction of the loss projected onto the tangent space of $M_i$.
Similar to the goal bias in RRT, a parameter $\gb\in[0,1]$ specifies the probability of selecting the SteerConstraint step rather than SteerPoint. 



% A reference implementation of this algorithm in Python is made available on GitHub.

% An alternative way of computing a solution is by taking the steepest descent direction of the loss and projecting it onto the tangent space of the current manifold, which results in
% \begin{align}
% 	\hat{d}= -V_{\bot} V_{\bot}\T J_{M_{i+1}}\T h_{M_{i+1}} \label{eq:steer_constraint}
% % 	&-\left[I - (J_{M_{i+1}}\T J_{M_{i+1}})\inv J_{M_i}\T (J_{M_i}(J_{M_{i+1}}\T J_{M_{i+1}})\inv J_{M_i}\T)\inv J_{M_i}\right]\\
% % 	&(J_{M_{i+1}}\T J_{M_{i+1}})\inv J_{M_{i+1}}\T h_{M_{i+1}}\\
% % 	?&= 
% \end{align}
% The solutions of \eq \eqref{eq:steer_system} and \eqref{eq:steer_constraint} are equivalent after normalizing them.

% \begin{comment}
% \subsection{Projection on Row Space of Future Manifolds}
% In this section, we provide an extension to the previously proposed steering strategy that incorporates additional information on future manifolds. The goal of this modification is to achieve a more goal-directed exploration by projecting the direction $d$ onto the row space of future manifolds. While this change increases the overall performance on many planning problems (see \sect \ref{sec:psm_experiments}), it comes with the caveat of a smaller solution class.

% We define a matrix that stacks all the Jacobians of the \mbox{$k$} future manifolds
% \begin{align}
% 	\tilde{J}_{i,k} (q) = \bmat{c}{J_{i+2}(q)\\ J_{i+3}(q)\\ \vdots\\ J_{i+2+k}(q)}
% \end{align}
% and project the vector $d$ after step 10 in Algorithm 1 onto the row space of $\tilde{J}_{i,k}$ by replacing the computation in \eq \eqref{eq:steer_point_sol} with
% \begin{align}
% 	d = (V_{\bot} V_{\bot}\T) (\tilde{V}_{//}\tilde{V}_{//}^T) (q_1-q_0)
% \end{align}

% In the case of steering towards the next constraint (step 8), we first compute $d$ with \eq \eqref{eq:steer_constraint} and afterwards project it towards future manifold intersections and onto the orthogonal space of $d$ with
% \begin{align}
% 	&\t{\textbf{for} }o\in \{2,\dots,k \}\t{ do:} \nonumber\\
% 	&\qquad d = d + \left(I - \frac{d d\T}{d\T d}\right) J_{M_{i+o}}\T h_{M_{i+o}} \\
% 	&\t{\textbf{end for}} \nonumber
% \end{align}
% In the experiments, we evaluate the effect of various $k$ on the planning problem.
% \end{comment}


% This is done by taking a step in direction $d$ from $q_\t{near}$ with the maximum step size $\ga\in \R_{>0}$ and then projecting it onto a manifold (steps \ref{alg:project_start}--\ref{alg:project_end}). 
After the steering strategy is determined and $d$ is computed, $q_\t{new}$ is projected either on $M_i$ or on the intersection manifold $M_i \cap M_{i+1}$ depending on the distance to the intersection of the manifolds measured by $||h_{M_{i+1}} (q_\t{new})||$ (step \ref{alg:project_start} of \alg \ref{alg:steer_project}).
The threshold for this condition is sampled uniformly between $0$ and $r$, where the parameter $r\in \R_{>0}$ describes the closeness required by a point around $M_{i+1}$ to be projected onto $M_i \cap M_{i+1}$. 
This randomization is necessary in order to achieve probabilistic completeness that is discussed in \sect \ref{ssec:comp-optimal}, which also gives a formal definition of $r$. 

At this point, $q_\t{new}$ has been produced and the algorithm attempts to add it to the tree using the extend routine from RRT${}^*$ \cite{karaman2011sampling}, which we outline in Appendix \ref{sec:rrt_extend}.

% RRT$^*$\_EXTEND routine (described in the supplementary material), which is a straightforward adaptation of the extension step in RRT$^*$ to this problem.
%(\alg \ref{alg:rrt_extend}).
% \new{This routine checks the newly projected $q_\t{new}$ configuration for collision with the current free configuration space $C_{\t{free},i}$, performs rewiring steps, and eventually adds it as a node to the tree. 
% The rewiring step is equivalent to the one in RRT$^*$ \cite{karaman2011sampling}, which checks if any nearby points can be reached with a shorter distance and updates its parent nodes if that is the case.
% It uses a distance function $c(q_0, q_1)\in \R_{\geq 0}$ between two nearby configurations and a function \emph{Cost}$(q)$ that stores the path costs from the root of the tree to a node $q$ in order to reconnect a new node $q$ to its neighbor that results in the shortest path from root $q_\t{start}$ to $q$.
% Note that, $c(q_0, q_1) \triangleq J(\overline{q_0q_1})$, where $\overline{q_0q_1}$ denotes the geodesic \cite{Boothby:107707} joining points $q_0$ and $q_1$ on the current manifold.
% }

\new{The final step in each inner iteration of \alg \ref{alg:smp} is to check two necessary conditions to determine if the point should also be added to the set of intersection nodes $V_\t{goal}$: 
1) The point $q_\t{new}$ has to be on the next manifold $h_{M_{i+1}}$ (step \ref{alg:next_manifold}); 
2) $V_\t{goal}$ does not already contain the point $q_\t{new}$ or a point in its vicinity (step \ref{alg:avoid_duplicates}).
For the second condition, we introduce the parameter $\gr \in \R_{\geq 0}$ that is the minimum distance between two intersection points. As we will discuss in the theoretical analysis, $\gr$ must be $0$ in order to achieve probabilistic completeness and asymptotic optimality. In practice, we usually select $\gr > 0$, which results in a better performance since it avoids having a large number of nearby and duplicate intersection points.}


\subsection{Outer Loop: Initializing the Next Subproblem}
\label{ssec:phase3}
After the inner loop of \smp~completes, a new tree is initialized in steps \ref{alg:newtreeinit_start}--\ref{alg:newtreeinit_end} with all the intersection nodes in $V_\t{goal}$ and their costs so far. Initializing a new tree only with the intersection nodes has the advantage that subsequent planning steps focus on these relevant nodes, which results in a lower computation time and more goal-directed growing of the tree towards the next manifold. To keep the tree structure, we add a synthetic root node $q_\t{root}$ as parent node for all intersection nodes (\fig \ref{fig:tree_init}). In line \ref{alg:next_freespace}, the free configuration space is updated based on the reached intersection node. Convergence of the algorithm can be defined in various ways. We typically set an upper limit to the number of nodes or provide a time limit for the inner loop. After reaching the convergence criteria, the algorithm returns the path with the lowest cost that reached the goal manifold $M_{n+1}$.

\subsection{Completeness and Optimality}
\label{ssec:comp-optimal}
Under the assumption that $\rho$ is 0, \smp~is provably probabilistically complete and asymptotically optimal. Here, we outline our approach to proving these properties. Probabilistic completeness is proved in two steps. First we prove probabilistic completeness of \smp~on a single manifold. We claim subsequently that almost surely the tree grown on a manifold can be expanded onto the next manifold as the number of samples tends to infinity. The calculations related to the first step are based on \cite[Theorem 1]{Kleinbort2019}. Theorem 1 in the supplemental material proves the subsequent claim. 

Proving the asymptotic optimality of \smp~relies on three lemmas (Lemma 2, 3 and 4 in the supplementary material). Lemma 2 shows that for any weak clearance path \cite{karaman2011sampling} there exist a sequence of paths with strong clearance \cite{karaman2011sampling} that converges to a path with weak clearance. Our analysis assumes that the optimal path has weak clearance. Hence, there exist a sequence of strong clearance paths that converges to the optimal path.  Using Lemma 3 and Lemma 4, we prove that with an appropriate choice of the parameter $\gr$, the \smp~tree grown on the sequenced manifolds contains the paths which are arbitrarily close to any strong clearance path in the sequence of paths that converges to the optimal path. Finally using continuity of the cost function, we prove that \smp~is asymptotically optimal.

Detailed  proofs of the probabilistic completeness and asymptotic optimality can be found in Appendices \ref{sec:Probabilistic completeness} and \ref{sec:Asymptotic optimality}.

%\rag{As mentioned in the introduction, we have proved the probabilistic completeness and asymptotic optimality of \smp. In this section we outline our approach to proving these properties of \smp~ and defer the detailed  proofs to the supplemental material for ease of readability. The probabilistic completeness is proved in two steps. In the first step, we  prove the probabilistic completeness of \smp~ on a single manifold. Subsequently we claim that, almost surely the tree grown on a manifold can be expanded onto the next manifold as the number of samples tends to infinity. The calculations related to the first step are based on \cite[Theorem 1]{Kleinbort2019}. Theorem 1 in the supplemental material proves the claim in subsequent step. Proving the asymptotic optimality of \smp ~relies on three lemmas referred as Lemma 2, 3 and 4 in the supplementary material. Lemma 2 shows that for any weak clearance path  \cite{karaman2011sampling} there exist a sequence of path with strong clearance \cite{karaman2011sampling} that converge to path with weak clearance. In our analysis it is assumed that the optimal path has weak clearance. Hence, there exist a sequence of strong clearance paths that converges to the optimal path.  Using Lemma 3 and Lemma 4, we prove that with an appropriate choice of the parameter $\gamma$, the \smp ~  tree grown on the sequenced manifold contain the paths which are arbitrarily close to any strong clearance path in the sequence of paths that converges to the optimal path. Finally using continuity of cost function, we prove that \smp ~is asymptotically optimal.}  




\section{Evaluation}
\label{sec:psm_experiments}
In the following experiments, we solve kinematic motion planning problems where the cost function measures path length. We compare the following methods with each other:

% the proposed method \textbf{\smp} (\alg \ref{alg:smp}) with three alternative methods:
\begin{itemize}[leftmargin=*]
    \item \textbf{\smp}: The method proposed here -- \alg \ref{alg:smp}.
    %
    \item \textbf{\smp~(Greedy)}: Algorithm \ref{alg:smp} with the modification that only the node with the lowest cost in $V_\t{goal}$ is selected to initialize the next tree (steps \ref{alg:newtreeinit_start} -- \ref{alg:newtreeinit_end} of \alg \ref{alg:smp}).
    %
    \item \textbf{\smp~(Single Tree)}: This method grows a single tree over the manifold sequence without splitting it into individual subtrees. The algorithm uses $\rho=0$. It is explained in detail in Algorithm 3 in Appendix \ref{sec:smp_single_tree}.
    %
    \item {\textbf{RRT$^*$+IK}}: This method consists of a two-step procedure that is applied to every manifold in the sequence. First, a goal point on the manifold intersection is generated via inverse kinematics by randomly sampling a point in $C$ and projecting it onto the manifold intersection. Next, RRT$^*$ is applied to compute a path on the current manifold towards this node \cite{kingston2019ijrr}. This procedure is repeated until a point on the goal manifold is reached.
    %
    \item {\textbf{Random MMP}}: The Randomized Multi-Modal Motion Planning algorithm \cite{hauser2011randomized} was originally developed for the more general class of motion planning problems where the sequence of manifolds is unknown. Here, we apply it to the simpler problem where the sequence is given in advance and use RRT$^*$ to connect points between mode transitions.
    %
    \item {\textbf{CBiRRT}: The Constrained Bidirectional Rapidly-Exploring Random Tree algorithm \cite{berenson2009manipulation, berenson2011task} grows two trees towards each other with the RRT Connect strategy \cite{kuffner2000rrt}. In each steering step, the sampled configuration is projected onto the manifold with the lowest level set function value. Since CBiRRT does not optimize an objective function, we apply a short cutting algorithm as a post-processing step.}
\end{itemize}
We compare these methods on the following criteria:
\begin{itemize}[leftmargin=*]
    \item \textbf{Path length} -- The length of the found path in $C$ space.
    \item \textbf{Success rate} -- The number of times a collision-free path to the goal manifold is found for different random seeds.
    \item \textbf{Computation time} -- Time taken to compute a path. All experiments are run on a 2.2 GHz Quad-Core Intel Core i7.
\end{itemize}
\new{The parameter values $\alpha, \beta, \epsilon, \rho, r, m$ for the individual experiments were chosen experimentally and are summarized in Table \ref{tab:exp_parameter}.}
\subsection{3D Point on Geometric Constraints}
\label{ssec:geom_exp}
\new{We demonstrate the planning performance and properties of the individual methods on a simple point that can move in a 3D space.} The point needs to traverse three constraints defined by geometric primitives. The configuration space is limited to $[-6, 6]$ in all three dimensions.
%
The initial state is \mbox{$q_\t{start}=(3.5, 3.5, 4.45)$} and the sequence of manifolds is
\begin{enumerate}
	\item Paraboloid: $$h_{M_1}(q) = 0.1 q_1^2 + 0.1 q_2^2 + 2 - q_3$$
	\item Cylinder: $$h_{M_2}(q) = 0.25 q_1^2 + 0.25 q_2^2 - 1.0$$
	\item Paraboloid: $$h_{M_3}(q) = -0.1 q_1^2 - 0.1 q_2^2 - 2 - q_3$$
	\item Goal point:  $$h_{M_4}(q) = q - q_\t{goal}$$ with the goal configuration \mbox{$q_\t{goal}=(-3.5, -3.5, -4.45)$}.
\end{enumerate}
We evaluate the algorithms on two variants of this problem: an obstacle-free variant (\fig \ref{fig:psm_hourglass}), and a variant that contains four box obstacles placed at the intersections between the manifolds (\fig \ref{fig:psm_hourglass_paths}). In \fig \ref{fig:psm_hourglass}, $q_\t{start}$ is drawn as red point and $q_\t{goal}$ as blue point. The intersection nodes $V_\t{goal}$ are shown as magenta points and a solution path from \smp~is visualized as a line. 

\new{
The results on success rate, path length and computation time are given in Table \ref{tab:comparison_results}. All the methods are consistently able to find a path for all $10$ random seeds. \smp~and \smp~(Single Tree) consistently achieve the lowest cost in both scenarios. \smp~(Single Tree) has a higher computation time, because it keeps all nodes in a single tree whereas \smp~splits them into individual trees per manifold. CBiRRT does not optimize an objective function and immediately converges when it finds a feasible path, which achieves the overall lowest computation time. However, the mean cost and standard deviations are higher compared to \smp. RRT${}^*$+IK and Random MMP only optimize over the individual paths, but do not optimize the intersection point selection, which results in higher costs and standard deviations. 
\smp~(Greedy) is better in terms of computation time since it only takes one intersection point as initial point for the next tree, but achieves an overall lower performance compared to \smp. 
The results also show that only \smp~and \smp~(Single Tree) are consistently able to find the intersection regions between the obstacles in which the optimal path lies. The other methods mainly select the intersection regions that are discovered first in the exploration. \fig \ref{fig:psm_hourglass_paths} shows a set of found paths on the variant with obstacles.}

\new{In \fig \ref{fig:psm_hourglass_rho_cost}, the path costs $J(\tau)$ of \smp~are compared for various values of $\gr$. This parameter specifies the minimum distance between two intersection points, which influences the number of intersection points created during planning (step \ref{alg:avoid_duplicates} in \alg \ref{alg:smp}). As a reference, we visualize the path costs of \smp~(Greedy) and \smp~(Single Tree). The results show that the computed paths of \smp~with a small $\gr$ value are very similar to the ones of \smp~(Single Tree) whereas for larger $\gr$ values, \smp~converges to the same performance as \smp~(Greedy) since only a single intersection point is considered. Therefore, $\gr$ can be seen as a trade-off between planning faster and achieving lower path costs. \fig \ref{fig:psm_hourglass_samples_cost} compares the path costs for different samples $m$. All methods improve with an increasing amount of samples and \smp~and \smp~(Single Tree) converge to similar cost values.}


\begin{figure}[t]
	\centering
	\includegraphics[width=.45\textwidth]{psm_graphics/hourglass_paths2.pdf}
	\caption{Samples of found paths on the \textit{3D point on w/ obstacles} problem (\sect \ref{ssec:geom_exp}).}
	\label{fig:psm_hourglass_paths}
% 	\vspace{-0.25in}
\end{figure}


\begin{table}[t]
\centering
\renewcommand{\tabcolsep}{4pt}
    \begin{tabular}{|l|c|c|c|}
\hline
                                 & \textbf{Success} & \textbf{Path length} & \textbf{Comp. time [s]} \\
 \hline
 \textbf{3D point w/o obstacles} &                  &                      &                     \\
 PSM${}^*$                       & $10 / 10$        & $\mathbf{14.47\pm 0.04}$      & $10.64\pm 0.16$     \\
 PSM${}^*$ (Single Tree)         & $10 / 10$        & $14.47\pm 0.05$      & $13.72\pm 0.18$     \\
 PSM${}^*$ (Greedy)              & $10 / 10$        & $16.20\pm 0.05$      & $10.36\pm 0.10$     \\
 RRT${}^*$+IK                    & $10 / 10$        & $17.84\pm 2.23$      & $28.35\pm 13.50$    \\
 Random MMP                      & $10 / 10$        & $17.33\pm 1.28$      & $34.75\pm 17.21$    \\
 CBiRRT                          & $10 / 10$        & $14.70\pm 0.71$      & $\mathbf{5.04\pm 0.30}$      \\
 \hline
 \textbf{3D point w/ obstacles}  &                  &                      &                     \\
 PSM${}^*$                       & $10 / 10$        & $15.95\pm 0.13$      & $13.74\pm 0.51$     \\
 PSM${}^*$ (Single Tree)         & $10 / 10$        & $\mathbf{15.87\pm 0.18}$      & $20.42\pm 0.86$     \\
 PSM${}^*$ (Greedy)              & $10 / 10$        & $19.69\pm 0.27$      & $12.89\pm 0.51$      \\
 RRT${}^*$+IK                    & $10 / 10$        & $21.56\pm 3.05$      & $30.21\pm 7.55$     \\
 Random MMP                      & $10 / 10$        & $22.15\pm 2.20$      & $42.09\pm 17.22$     \\
 CBiRRT                          & $10 / 10$        & $16.66\pm 1.34$      & $\mathbf{3.34\pm 0.25}$      \\
 \hline
 \textbf{Robot transport A}      &                  &                      &                     \\
 PSM${}^*$                       & $10 / 10$        & $\mathbf{7.76\pm 0.84}$       & $7.22\pm 0.81$      \\
 PSM${}^*$ (Single Tree)         & $9 / 10$         & $8.53\pm 1.19$       & $11.56\pm 0.41$     \\
 PSM${}^*$ (Greedy)              & $10 / 10$        & $8.18\pm 0.91$       & $\mathbf{7.03\pm 0.09}$      \\
 RRT${}^*$+IK                    & $10 / 10$        & $11.83\pm 3.23$      & $74.65\pm 28.86$    \\
 Random MMP                      & $10 / 10$        & $11.62\pm 2.36$      & $85.45\pm 25.66$    \\
 \hline
 \textbf{Robot transport B}      &                  &                      &                     \\
 PSM${}^*$                       & $10 / 10$        & $\mathbf{14.73\pm 1.27}$      & $\mathbf{14.19\pm 0.76}$     \\
 PSM${}^*$ (Single Tree)         & $0 / 10$         & --                   & --                  \\
 PSM${}^*$ (Greedy)              & $9 / 10$         & $15.41\pm 2.38$      & $14.75\pm 0.53$     \\
 RRT${}^*$+IK                    & $2 / 10$         & $45.14\pm 0.58$      & $89.84\pm 11.00$    \\
 Random MMP                      & $10 / 10$        & $16.96\pm 4.59$      & $163.26\pm 37.80$   \\
 \hline
 \textbf{Robot transport C}      &                  &                      &                     \\
 PSM${}^*$                       & $10 / 10$         & $\mathbf{27.07 \pm 2.58}$      & $\mathbf{275.83 \pm 19.73}$   \\
 PSM${}^*$ (Single Tree)         & $0 / 10$         & --                   & --                  \\
 PSM${}^*$ (Greedy)              & $10 / 10$         & $31.75 \pm 2.51$                   & $311.81\pm 9.79$                  \\
 RRT${}^*$+IK                    & $0 / 10$         & --                   & --                  \\
 Random MMP              & $0 / 10$         & --                   & --                  \\
 \hline
\end{tabular}
\caption{Results of the 3D point and robot transport problems. We report the mean and one unit standard deviation over $10$ runs with different random seeds.}
    \label{tab:comparison_results}
    % \vspace{-0.25in}
\end{table}

\subsection{Multi-Robot Object Transport Tasks}
In this experiment, we evaluate \smp~on various object transportation tasks involving multiple robots. The overall objective is to transport an object from an initial to a goal location. We consider three variations of this task:
\begin{itemize}[leftmargin=*]
    \item \textbf{Task A}: A single robot arm mounted on a table with $k=6$ degrees of freedom. The task is to transport an object from an initial location on the table to a target location. This task is described by $n=3$ manifolds.
    \item \textbf{Task B}: This task consists of two robot arms and a mobile base consisting of $k=14$ degrees of freedom. The task is defined such that the first robot arm picks the object and places it on the mobile base. Then, the mobile base brings it to the second robot arm that picks it up and places it on the table. This procedure is described with $n=5$ manifolds.
    \item \textbf{Task C}: In this task, four robots are used to transport two objects between two tables. Three arms are mounted on the tables and another arm with a tray is mounted on a mobile base. Besides transporting the objects, the orientation of the two objects needs to be kept upright during the whole motion. This task is described with $n=12$ manifolds and the configuration space has $k=26$ degrees of freedom.
\end{itemize}
The initial states of the three tasks are visualized in \fig \ref{fig:robot_tasks} where the target locations of the objects are shown in green. The geometries of the objects were chosen such that the tasks are intersection point independent (\sect \ref{ssec:ipip}). Three types of constraints are used to describe the tasks. Picking up an object is defined with the constraint
$h_M(q) = x_g - f_{\t{pos}, e}(q)$
where $x_g\in\R^3$ is the location of the object and $f_{\t{pos}, e}(q)$ is the forward kinematics function to a point $e\in\R^3$ on the robot end effector. The handover of an object between two robots is described by
$h_M(q) = f_{\t{pos}, e_1}(q) - f_{\t{pos}, e_2}(q)$
where $f_{\t{pos}, e_1}(q)$ is the forward kinematics function to the end effector of the first robot and $f_{\t{pos}, e_2}(q)$ is that of the second robot.
%
The orientation constraint is given by an alignment constraint
$h_M(q) = f_{\t{rot}, z}(q) \T e_z - 1$
where $f_{\t{rot}, z}(q)$ is a unit vector attached to the robot end effector that should be aligned with the vector $e_z=(0,0,1)$ to point upwards.
These constraints are sufficient to describe the multi-robot transportation tasks. The parameters of the algorithms are summarized in Table \ref{tab:exp_parameter}.

The costs of the algorithms are reported in Table \ref{tab:comparison_results}. \new{CBiRRT could not be applied to this task since it requires a goal configuration at which the backward tree originates, which is not available for these tasks.} On task A, nearly all methods robustly find solutions. However, when task complexity increases, RRT$^*$+IK, \smp~(Single Tree), and Random MMP have difficulties to solve to the problem. Only \smp~and \smp~(Greedy) were able to find solutions of task C with the given parameters. The cost and computation time of \smp~is lower compared to \smp~(Greedy). A found solution of \smp~for Task C is visualized in \fig \ref{fig:robot_task_c}.

\subsection{Pick-and-Pour on Panda Robot}
\label{ssec:robot_exp}
In this experiment, we demonstrate \smp~on a real Panda robot arm with seven degrees of freedom. The task description consists of $n=7$ manifolds, which describe the individual grasp, transport, and pouring motions. We assume the position of the objects in the scene are known. The parameters are the same as in the robot transport experiments (Table \ref{tab:exp_parameter}) and the planning time was 131.65 seconds. \fig \ref{fig:panda_pour} shows a found path executed on the real robot. The resulting motions of the task are shown in the supplementary video.

\begin{figure*}
	\centering
	\subfloat[\label{fig:psm_hourglass_rho_cost}]{\includegraphics[width=.5\textwidth]{psm_graphics/hourglass_rho_cost.pdf}}
	\subfloat[\label{fig:psm_hourglass_samples_cost}]{\includegraphics[width=.5\textwidth]{psm_graphics/hourglass_sample_cost.pdf}}
	
	\caption{Path costs over variations of the parameter $\gr$ (left) and the number of samples $m$ (right) on the \emph{geometric constraints w/o obstacles} problem (\sect \ref{ssec:geom_exp}). The graphs show the mean and unit standard deviation over $10$ trials. Figure (a) shows the costs increase for higher values of $\gr$, meaning fewer intersection points are considered during planning. 
	In (b), the performance of all methods improves with larger $m$ values where \smp~and \smp~(Single Tree) converge to similar path costs.}
	\label{fig:psm_hourglass_eval}
\end{figure*}


\begin{figure*}
    \centering
    \subfloat[Task A]{\includegraphics[height=0.205\textwidth]{psm_graphics/robot_task1.png}}
    \hspace{0.0in}
    \subfloat[Task B]{\includegraphics[height=0.205\textwidth]{psm_graphics/robot_task2.png}}
    \hspace{0.0in}
    \subfloat[Task C]{\includegraphics[height=0.205\textwidth]{psm_graphics/robot_task3.png}}
    \caption{Start states of the object transport tasks where the goal is to place the red and blue object to the green target locations.}
    \label{fig:robot_tasks}
\end{figure*}



\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{psm_graphics/task_c.png}
\caption{Snapshots of the resulting motion that \smp~found for Task C.}
    \label{fig:robot_task_c}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{psm_graphics/task_pour.png}
    \caption{Snapshots of the pouring task motion.}
    \label{fig:panda_pour}
\end{figure*}
\begin{table}[t]
\centering
\renewcommand{\tabcolsep}{4pt}
    \begin{tabular}{|c|c|c|c|}
        \hline
        \textbf{Parameter name} & \textbf{Symbol} & \specialcell{\textbf{3D point}\\ (Sec. \ref{ssec:geom_exp})} & \specialcell{\textbf{Robot transport}\\ (Sec. \ref{ssec:robot_exp})}\\
        \hline
        max step size & $\alpha$ & $1.0$ & $1.0$\\
        goal bias probability & $\beta$ & $0.1$ & $0.3$\\
        constraint threshold & $\epsilon$ & $0.01$ & 1e-5\\
        duplicate threshold & $\rho$ & $0.1$ & $0.5$\\
        projection distance & $r$ & $1.5$ & $0.5$\\
        number of samples & $m$ & $1200$ & $2000$\\
        \hline
    \end{tabular}
    % \hspace{2em}
    \caption{Parameters of the \textit{3D Point on Geometric Constraints} and \textit{Multi-Robot Object Transport} experiment.}
    \label{tab:exp_parameter}
    % \vspace{-0.25in}
\end{table}



\section{Discussion}
\label{sec:psm_conclusion}
We proposed the algorithm \smp~to solve sequential motion planning 
posed as a constrained optimization problem, where the goal is to find a collision-free path that minimizes a cost function and fulfills a given sequence of manifold constraints.
The algorithm is applicable to a certain problem class that is specified by the intersection point independent property, which says that the change in free configuration space is independent of the selected intersection point between two manifolds. 
\smp~uses RRT$^*$'s extend method with a novel steering strategy that is able to discover intersection points between manifolds.
We proved that \smp~is probabilistically complete and asymptotically optimal and demonstrated it on multi-robot transportation tasks.
 
Restricting the problem class to intersection point independent planning problems allowed us to develop efficient solution strategies like growing a single tree over a sequence of manifolds. An interesting question for future research is how to extend the strengths of \smp~to a larger problem class; specifically, how \smp~can be used for problems that do not fulfill the intersection point independent property. For such problems, the choice of intersection points influences the future parts of the planning problem, which results in a more complex problem. An interesting aspect that our future work will address is the effect of an intersection point on subsequent manifolds and how solutions for one intersection point can be reused and transferred to other intersection points without replanning from scratch.
Further, we plan to investigate the reduction of such problems to the simpler intersection point independent problem class, for example, by morphing object geometries into simpler shapes such that the intersection point independent property is satisfied. \smp~could be applied to the reduced problem and provide a good initial guess for solving the original problem.


% Another interesting research direction is the combination of this work with trajectory optimization techniques \cite{Pavone-RSS-19} that define the motion planning problem in a similar manner. Trajectory optimization methods could be integrated into the steering strategy of \smp~or the solution of the proposed method could be used as an initialization for trajectory optimization to achieve faster convergence.
 
\imr{remove/edit this par}
A future direction we already have begun exploring is the integration of learning techniques into the motion planner \cite{sutanto2020learning}. Here we assumed the user has the knowledge and capability to write the constraint manifolds for the entire task sequence. However, this may not always be the case, or it may be more convenient to give demonstrations of a task such that the constraints can be automatically extracted for future planning. To this end, we are beginning to explore neural network models that are able to learn manifold constraints from robot demonstrations. We train these networks to represent level-set functions of the constraint by aligning subspaces in the network with subspaces of the data. We integrated such learned manifolds together with analytically specified manifolds into a planning problem that was solved with \smp.




==> quantiles.tex <==
\section{Introduction}

\begin{figure}[h!]
\centering
    \includegraphics[width=\columnwidth]{ipp_figures/hero3.pdf}
    \caption{\textbf{Full system.}
    First, the parameters for the robotic survey are chosen, such as the area bounds and the quantiles for specimen collection.
    The robot performs informative path planning using our proposed objective functions, creating an environment model and an estimate of the quantile values.
    The quantile locations are then selected by minimizing our proposed loss function. These quantile locations correspond to physical locations which, when measured, have the estimated quantile values.
    After the quantile locations are chosen, humans go to them to collect field specimens which they later analyze in a laboratory setting. 
    This work focuses on the steps shown in the blue shaded boxes.
    }
    \label{fig:quantiles-hero}
\end{figure}


%%MOTIVATION

%Biologists take samples
In order to understand biological phenomena, scientists take a small number of physical specimens for later analyses to characterize the biological community and the contextual environmental conditions at the site.
% For example, marine biologists may be interested in using the concentration of chlorophyll present in a body of water to guide physical sampling of algal blooms, or agricultural scientists may be interested in using crop health to guide physical sampling of plants.
A marine biologist may capture water in a container or filter media at a location for later analysis, and an agricultural scientist may capture a small portion of a plant.
Scientists later analyze these captured portions of the environment in a detailed laboratory setting.
It is often expensive to collect these physical specimens as the scientist must go to the location and use a physical reagent, such as a container or filter media, which are limited in the field. 
%They don't do a good job because they use heuristics
Traditionally, expert heuristics underpin the selection of locations for scientific analysis. 
These expert heuristics generally attempt to spread out the analysis locations in the phenomena of interest in order to take specimens with differing concentrations for characterization of heterogeneity~\cite{ysi_whitepaper}.
The heuristics may make use of robotic surveys, but currently most robotic surveys use either pre-programmed paths~\cite{ysi_whitepaper}, or autonomy which seeks maxima~\cite{Marchanta} or to cover the area spatially~\cite{kemna_pilot_2018,guestrin_near-optimal_2005}, and do not directly plan for the specimen collection tasks.
%We propose that they should choose quantiles, not necessarily evenly spaced, and the amount of which is the number of samples they can take
In contrast, we propose performing an adaptive robotic survey to find locations of interest for scientific analysis.
To specify these locations, we propose calculating the quantiles of the distribution of interest so that scientists can capture specimens at varied locations in the environment based on differing values of some phenomenon of interest to them. 
%In the case of algae bloom sampling, if you are doing a generic study and can take 10 samples maybe you want deciles, or if you only care about bad part take 3 samples at .9 95 99
For instance, if a marine biologist is interested in taking 9 physical water specimens that are spread over a range of chlorophyll concentrations, they may choose to use the deciles of the concentration. 
If only a small number of locations can be analyzed and the upper extrema values are of interest, they may choose to perform analysis at the locations of the $(0.90, 0.95, 0.99)$ quantiles.
The quantiles of interest are a flexible way to describe the objective of specimen collection that is largely invariant to the exact phenomena being measured.

%%WHAT WE DO
%Explore a region of interest
Our goal is to select locations for detailed analysis by scientists in two steps. 
We use a robot to perform an adaptive survey, and then find locations to suggest for specimen collection based on the measurements it takes.
Specifically, we first aim to find the desired quantile values of the measurement distribution by adaptively selecting robot measurement locations that maximize an objective function designed to estimate quantile values, and then we produce suggested locations for specimen collection that are likely to contain these values.
\Cref{fig:quantiles-hero} summarizes the approach, showing how our objective function for informative path planning and our loss function for location selection fit into an overall physical specimen collection pipeline.

% We develop our method using an informative path planning formulation
% and show that it outperforms entropy- and sequential Bayesian optimization-based objective baselines. 
Our contributions are:

\begin{itemize}
    \item A planner with custom objective functions that adaptively improve the quality of estimated quantile values;
    \item A general loss function, which can be used with any optimizer, for selecting spatial locations for physical specimen collection which have the values estimated for the quantiles;
    \item Quantitative evaluation of our method on point and camera sensors with previously collected aquatic datasets;
    \item A demonstration of our method on a robot in a real-world crop health estimation task.
\end{itemize}

\section{Background}
We pose our problem as an IPP problem, where the overall goal is to minimize error in the estimate of a given set of quantiles of a distribution in the environment, and we use a GP to model the environment.
\imr{move to quantiles} We use these works (IPP as a POMDP) to formulate and solve the IPP problem.
For these reasons, we use the POMDP formulation to solve our IPP problem in this work.
 
\imr{move to quantiles} We approximately solve this POMDP to select actions to take measurements for maximizing the objective function.

\imr{move to quantiles}
In this work, we use a GP as the environment model to estimate the value $\mu(\sensedlocation)$ and variance $\sigma^2(\sensedlocation)$ at a specific location $\sensedlocation$.

\imr{move to quantiles}
Our works differs from these by instead focusing on improving estimates for specific quantiles instead of broad understanding of the spatial makeup of a distribution.

\imr{move to quantiles}
While these works have similarities with quantile estimation tasks, they require specifying a single quantile or are restricted to finding the extrema, as opposed to a set of arbitrary quantiles.
\imr{move to quantiles}
Our work differs from such works as we do not seek to only find maximal concentration areas, but seek to find a variety of concentration values specified by the quantiles. 
\imr{move to quantiles}
Here we use a Gaussian kernel density estimator for quantile standard error when planning.
Other estimation methods include the \mjci method~\cite{maritz_note_1978}, and the bootstrap or jackknife methods which involve calculating the quantiles over repeatedly sampled subsets of the data. 
These last two methods can be slow for large datasets and require many iterations to converge.

\imr{move to quantiles}
We use these methods (continuous non-convex gradient-free optimization) to select the analysis locations by minimizing our proposed loss function once the IPP survey is completed (see \cref{sec:location}).


\section{Formulation}
%\vspace{-1px}
We use a grid-based representation of the planning space, $\gtlocations$, which defines the set of locations that the robot could visit.
For a robot that moves in $\mathbb{R}^d$, $\gtlocations \subset \mathbb{R}^d$.
%$\locations$ is the set of locations that the robot has visited. 
$\gtsensedlocations$ is the set of locations the robot could measure. 
If the robot sensor has finer resolution than $\gtlocations$,
e.g. if the robot uses a camera sensor or takes measurements while traversing between grid points,
then $|\gtsensedlocations| > |\gtlocations|$.
We define $\sensedlocations_{0:t}$ as the locations the robot has measured up to time $t$ and $\gtsensedvalues$ and $\sensedvalues_{0:t}$ as the values at all possible measured locations, and the values the robot has measured up to time $t$, respectively, such that $|\gtsensedlocations| = |\gtsensedvalues|$ and $|\sensedlocations| = |\sensedvalues|$.



We define the ground truth quantile values as 
$\quantilevalues = 
quantiles(\gtsensedvalues,\quantiles)$
where $quantiles$ is the function described in \Cref{sec:quantile-estimation} which computes the values $V$ of the quantiles $\quantiles$ of a set of measurements, in this case $\gtsensedvalues$.
To define the robot's estimated quantile values, we compute 
$\estimatedquantilevalues = quantiles(\mu(\gtsensedlocations),\quantiles)$
that is, the quantile values of the predicted values from the robot's current GP for all locations the robot could sense.
This is done  to prevent the number of measurements from which the quantile values are estimated from changing as the robot explores (instead of, e.g. using $\mu(\sensedlocations)$).
By doing this, we ensure we always estimate the quantiles across the entire measurable area.
% To assess estimation accuracy, we compute the error using $RMSE (\estimatedquantilevalues , \quantilevalues)$.
During planning, we aim to minimize this error by taking actions which maximize an objective function $\objectivefunction$ that minimizes the error in the quantile value estimate.

To suggest locations for the quantile values, we aim to find a set of $\numtiles$ locations $\quantilespatiallocations$ in the continuous space whose values at those locations are equal to the quantile ground-truth values. 
A set of locations is defined as $\quantilespatiallocations \in \quantilespatiallocations^\#$ where $\quantilespatiallocations^\# \subset \mathbb{R}^{d \times |Q|}$ and $\quantilespatiallocations^\#$ is continuous over the space of $\gtsensedlocations$.
% We define any one set of suggested locations with $\quantilespatiallocations \in \quantilespatiallocations^*$.
% There may be multiple possible such $\quantilespatiallocations$ that satisfy this goal; we are interested in finding one of them.
In practice, the robot only has access to $\estimatedquantilevalues$ (not $\quantilevalues$) during the selection process, so the problem of finding the estimated quantile spatial locations $\estimatedquantilespatiallocations$ can be stated as shown in \cref{eq:point_selection} with some selection loss function $\score$ (see \cref{eq:ps_loss}).
\begin{equation}\label{eq:point_selection}
    \estimatedquantilespatiallocations = \argmin_{\quantilespatiallocations' \subset \quantilespatiallocations^\#}  \score (\estimatedquantilevalues, \quantilespatiallocations')
\end{equation} 



\section{Approach}
Figure \ref{fig:quantiles-hero} illustrates our method.
We separate our approach into two steps: the survey, and the suggestion of locations.
When performing the survey using IPP (\Cref{sec:planning}), the robot takes measurements of the environment to improve its estimate of the quantiles.
After the survey has concluded, location selection (\Cref{sec:location}) produces locations for scientists to visit to perform specimen collection.

 
\subsection{Informative Path Planning}\label{sec:planning}
To plan which locations to measure, the robot uses a POMDP formulation of IPP. 
In order to generate a policy, we use the partially observable Monte Carlo planner (POMCP)~\cite{silver2010pomcp}.
POMCP uses Monte Carlo tree search to create a policy tree. 
To expand the tree and estimate rewards, the tree is traversed until a leaf node is reached.
From the leaf node, the reward conditioned on that action is estimated by a random policy rollout which is executed until the discounted reward is smaller than some value $\epsilon$.
We modify the rollout reward to be fixed horizon, giving a reward of zero after a certain number of random policy steps.
We adopt the t-test heuristic for taking multiple steps from a POMCP plan for IPP to improve performance of the planner with fewer rollouts~\cite{denniston_icra_2020}.
We define $GP_{i-1} = GP(\sensedlocations_{0:i-1},\sensedvalues_{0:i-1}; \theta )$
as a GP conditioned on the previous locations ($\sensedlocations_{0:i-1}$) and measurements ($\sensedvalues_{0:i-1}$) before measuring a proposed value, and 
$GP_i = GP(\sensedlocations_{0:i-1} \cup \sensedlocations_i, \sensedvalues_{0:i-1} \cup \sensedvalues_i; \theta )$ 
as a GP conditioned on the previous and proposed locations ($\sensedlocations_i$) and measurements ($\sensedvalues_i$), where $\theta$ are GP parameters and $\sensedvalues_i = GP_{i-1}(\sensedlocations_i)$.
Because the observations $GT(x)$ for unseen locations are not known during planning, the predicted mean from $GP_{i-1}$ is used~\cite{Marchanta}.
%IPP using GPs suffers from the standard drawbacks of an $O(n^3)$ GP step, which can be alleviated by sparse GP approximations. In our case, \cref{eq:quantile_change,eq:standard_error} each require computing the mean value over $\sensedlocations$ twice.
%
% In this work, we modify the rollout reward to be a fixed horizon rollout, shown in 
% \begin{equation}\label{eq:max_depth}
%     R(\sensedlocation_i) = 
%      \begin{cases} 
%       0 & i\geq H \\
%       \objectivefunction(\mu(\sensedlocation_i)) 
%   \end{cases}
% \end{equation}
% where $i$ is the depth from the root node, $H$ is the fixed horizon parameter, $\objectivefunction$ is the objective function, and $\mu$ is the predicted output of the GP conditioned on the previous observations at $\location_i$.
% This fixed horizon objective function is used to allow the execution of expensive objective functions.


\textbf{Objective Functions for Quantile Estimation}
We develop two novel objective functions to improve the quality of quantile value estimates.
Both compare a measure of the quality of the quantiles estimated by the GP before and after adding a measurement to the GP,
and include an exploration term $c_{plan}\sigma^2(\sensedlocation_i)$ inspired by the upper confidence bound objective function~\cite{Marchanta}, where $c_{plan}$ is a chosen constant.
For both proposed objective functions we use \cref{eq:general_objective}, where $\delta$ is defined by the objective:
\begin{equation}\label{eq:general_objective}
    \objectivefunction(\sensedlocations_i) = \frac{\delta(\sensedlocations_i)}{\numtiles} +  \sum_{\sensedlocation_j \in \sensedlocations_i} c_{plan}\sigma^2(\sensedlocation_j), 
\end{equation}



The first objective function, which we call \textit{quantile change}, is based on the idea of seeking out values which change the estimate of the quantile values by directly comparing the estimated quantiles before and after adding the measured values to the GP.
The idea behind this is that a measurement which changes the estimate of the quantiles indicates that the quantiles are over- or under-estimated.
This can be seen in in \cref{eq:quantile_change}:
% \begin{align}\label{eq:quantile_change}
% \begin{split} 
%   \delta  &= ||quantile(\mu_{PRE}(\gtsensedlocations),\quantiles) - \\
%   & \hphantom{||qua} quantile(\mu_{POST}(\gtsensedlocations),\quantiles) ||_{1} \\
% %   \objectivefunction_\t{qc}(\sensedlocation_i) &= \frac{\delta}{\numtiles} + c \sigma^2(\sensedlocation_i) \\ 
% \end{split}
% \end{align}
\begin{align}
\begin{split}\label{eq:quantile_change}
  \delta_\t{qc}(\sensedlocations_i) = \|&quantile(\mu_{GP_{i-1}}(\gtsensedlocations),\quantiles) - \\ &quantile(\mu_{GP_{i}}(\gtsensedlocations),\quantiles) \|_{1} \\
%   \objectivefunction_\t{qc}(\sensedlocation_i) &= \frac{\delta}{\numtiles} + c \sigma^2(\sensedlocation_i) \\ 
\end{split}
\end{align}
The second objective function we develop, which we call \textit{quantile standard error}, is based on the change in the estimate of the standard error for the estimated quantiles.
It draws from the same idea that if the uncertainty in the quantile estimate changes after observing a measured value, then it will change the estimate of the quantile values, shown in \cref{eq:standard_error}:
\begin{align}\label{eq:standard_error}
\begin{split} 
   \delta_\t{se}(\sensedlocations_i) &= \|se(\mu_{GP_{i-1}}(\gtsensedlocations),\quantiles) - se(\mu_{GP_{i}}(\gtsensedlocations),\quantiles) \|_{1} \\
%   \objectivefunction_\t{se}(\sensedlocation_i) &= \frac{\delta}{\numtiles} + c \sigma^2(\sensedlocation_i) \\
\end{split}
\end{align}
$se$ is an estimate of the standard error of the quantile estimate for quantiles $\quantiles$. 
$se$ uses a Gaussian kernel density estimate (we found it faster and more stable than other standard error estimators).
%Other estimation methods include the \mjci method~\cite{maritz_note_1978}, and the bootstrap or jackknife methods which involve calculating the quantiles over repeatedly sampled subsets of the data. 
%These last two methods can be slow for large datasets and require many iterations to converge.
% To compute the objective function over a set of measured points, we average the objective function at each point.

\textbf{Baseline Objective Functions}
We compare against two baselines, one which maximizes spatial coverage of a phenomena and another which seeks maximal areas. 

\textit{Entropy} is a common objective function for IPP when only good spatial coverage of the environment is desired~\cite{kemna_pilot_2018,guestrin_near-optimal_2005,denniston_comparison_2019}. 
It provides a good baseline as it is often used when the specific values of the underlying concentration are unknown.
Entropy is defined \cref{eq:entropy}:

\begin{equation}\label{eq:entropy}
   \objectivefunction_\t{en}(\sensedlocations_i) = \sum_{\sensedlocation_j \in \sensedlocations_i}\frac{1}{2} \log(2 \pi e \sigma^2(\sensedlocation_j))
\end{equation}


Another objective function we compare against is \textit{expected improvement} (EI), which is widely used in Bayesian optimization and sequential Bayesian optimization for finding maxima~\cite{jones_efficient_1998, qin_improving_2017}.
EI favors actions that offer the best improvement over the current maximal value, with an added exploration term $\xi$ to encourage diverse exploration.
The EI objective function is defined according to \cref{eq:ei}:

\begin{equation}\label{eq:ei}
     f_{ei}(\sensedlocations_i) = \sum_{\sensedlocation_j \in \sensedlocations_i} I\Phi(Z) + \sigma(\sensedlocation_j)\phi(Z) \\
\end{equation}
where $Z =\frac{I}{\sigma^2(\sensedlocation_j)}$,  $I = \mu(\sensedlocation_j) - \max(\mu(\gtsensedlocations)) - \xi$, and $\Phi$ and $\phi$ are the CDF and PDF of the normal distribution, respectively.


\subsection{Location Selection}\label{sec:location}
% describe goal of point selection and how it fits into the overall problem 
Our final goal is to produce a set of $\numtiles$ locations $\quantilespatiallocations$, at which the concentration values will be equal to $\quantilevalues$, the values of the quantiles $\quantiles$. 
The selection process can be done offline as it does not affect planning.
% challenges of it
Finding locations that represent $\quantiles$ is difficult because the objective function over arbitrary phenomena in natural environments will likely be non-convex, and in a real-world deployment, the robot will only have an estimate $\estimatedquantilevalues$ of the $\quantilevalues$ it searches for.


With the location selection problem formulation as in \Cref{eq:point_selection}, we propose the loss function 
\begin{equation}\label{eq:ps_loss}
\score(\estimatedquantilevalues, \estimatedquantilespatiallocations) = \|\estimatedquantilevalues - \mu(\estimatedquantilespatiallocations)\|_{2} + c_{select} \sigma^2(\estimatedquantilespatiallocations),
\end{equation}
where $c_{select} \sigma^2(\estimatedquantilespatiallocations)$ is an added penalty for choosing points that the GP of collected measurements is not confident about\footnote{The parameters $c_{plan}$ and $c_{select}$ are distinct.}, and $\score$ can be used in any optimization scheme.
%; $c_{plan}$ is an exploration bonus for reducing uncertainty during the planning phase, while $c_{select}$ is a penalty for choosing uncertain points during the location selection phase.}}.
%
During optimization, \cref{eq:ps_loss} is evaluated using $\estimatedquantilevalues$ and returns the suggested specimen collection locations $\estimatedquantilespatiallocations$. 
We compare three optimization methods in our experiments to determine which best minimizes our selection loss function (\cref{eq:ps_loss}).
%
A strength of these types of optimization methods is that the formulation allows for suggesting points that may be spatially far from locations the robot was able to measure if they have values closer to the quantile values of interest.

\begin{figure}[t]
    \centering
        \begin{subfigure}{\threeboxplot}
                \centering
                \includegraphics[width=\textwidth,height=\boxplotheight,trim={.8cm 0 .5cm 0},clip]{ipp_figures/boxplots/Env_A,Deciles.pdf}
        \end{subfigure}
        \begin{subfigure}{\threeboxplot}
                \centering
                \includegraphics[width=\textwidth,height=\boxplotheight,trim={.8cm 0 .5cm 0},clip]{ipp_figures/boxplots/Env_A,Quartiles.pdf}
        \end{subfigure}
        \begin{subfigure}{\fourboxplot}
                \centering
                \includegraphics[width=\textwidth,height=\boxplotheight,trim={.8cm 0 .5cm 0},clip]{ipp_figures/boxplots/Env_A,Extrema.pdf}
        \end{subfigure}
        \begin{subfigure}{\threeboxplot}
                \centering
                \includegraphics[width=\textwidth,height=\boxplotheight,trim={.8cm 0 .5cm 0},clip]{ipp_figures/boxplots/Env_B,Deciles.pdf}
                
        \end{subfigure}
        \begin{subfigure}{\threeboxplot}
                \centering
                \includegraphics[width=\textwidth,height=\boxplotheight,trim={.8cm 0 .5cm 0},clip]{ipp_figures/boxplots/Env_B,Quartiles.pdf}
        \end{subfigure}
        \begin{subfigure}{\fourboxplot}
                \centering \includegraphics[width=\textwidth,height=\boxplotheight,trim={.8cm 0 .5cm 0},clip]{ipp_figures/boxplots/Env_B,Extrema.pdf}
        \end{subfigure}
        \caption{\textbf{Simulated drone planning experiments with real data.} Error between ground truth quantile values and estimated quantile values. Datasets A and B collected using a hyperspectral camera in Clearlake, California.
        Units are 400nm channel pixel intensity ($0-255$).  Each dataset and objective function pairing is run three times.
        }\label{fig:clearlake_planning_results}
        \vspace{-0.2in}
\end{figure}

\begin{figure}[b!]
    \centering
    \includegraphics[trim={0.2cm .2cm 0.3cm 0.3cm}, clip, width=.45\columnwidth,height=2.6cm]{ipp_figures/Environment_values_Drone.pdf}
    \includegraphics[trim={0.2cm .2cm 0.25cm 0.3cm}, clip, width=.45\columnwidth,height=2.6cm]{ipp_figures/Environment_values_AUV.pdf}
    \caption{
    Experimental dataset distributions. Drone data is measured in pixel intensity; AUV data in $\mu g/L$ chlorophyll.
    }
    \label{fig:environment_distributions}
    \vspace{-7pt}
\end{figure}

% Simulated annealing is a local search method which seeks to improve a single solution by moving to local solutions.
% The starting solution is selected heuristically. 
% This heuristic is the set of points the robot measured that are closest in value to $\estimatedquantilevalues$ for each quantile.

% Bayesian optimization and cross-entropy are both global search methods which maintain a distribution over the search space and update the distribution iteratively.
% These methods differ in the type of distribution over solutions they maintain and their search strategy.



\section{Experiments}
To evaluate our approaches for planning and for location selection, we compare against baselines in two different informative path planning tasks in simulation using four datasets collected in the real world.

In the first task, a simulated drone with a virtual camera gathers data from orthomosaics (a single image produced by combining many smaller images, called orthophotos) collected of a lake using a hyperspectral sensor. 
The orthomosaics, A and B, are taken in the same location but on different days and times.
The drone collects many measurements from one location, where each is a pixel in a downsampled image. 
As a proxy for chlorophyll concentration, we measure the 400nm channel pixel intensity ($0-255$).
The drone maintains a constant altitude and moves in a 2D plane with a north-fixed yaw, moving in either the $x$ or $y$ direction per step.

In the second task, an autonomous underwater vehicle (AUV) explores an environment.
Two AUV surveys, C and D, which were taken in the same reservoir but at different times and different areas, were conducted in a 3D lawnmower pattern using a chlorophyll sensor
and are interpolated using a GP to $\gtsensedlocations$.
At each step, the AUV moves in one $x$, $y$, or $z$ direction and takes five evenly spaced measurements when moving between locations.


We evaluate each task on their two respective datasets (A/B, C/D) and three different quantiles: deciles $(0.1, 0.2, \dots , 0.8, 0.9)$, quartiles $(0.25,0.5,0.75)$, and upper extrema $(0.9,0.95,0.99)$. See \Cref{fig:environment_distributions} for a summary of the dataset distributions.



\begin{figure}[t]
    \centering
                \begin{subfigure}{\threeboxplot}
                \centering
                \includegraphics[width=\textwidth,height=\boxplotheight,trim={.8cm 0 .5cm 0},clip]{ipp_figures/boxplots/Env_C,Deciles.pdf}
        \end{subfigure}
        \begin{subfigure}{\threeboxplot}
                \centering
                \includegraphics[width=\textwidth,height=\boxplotheight,trim={.8cm 0 .5cm 0},clip]{ipp_figures/boxplots/Env_C,Quartiles.pdf}
        \end{subfigure}
        \begin{subfigure}{\fourboxplot}
                \centering
                \includegraphics[width=\textwidth,height=\boxplotheight,trim={.8cm 0 .5cm 0},clip]{ipp_figures/boxplots/Env_C,Extrema.pdf}
        \end{subfigure}
        \begin{subfigure}{\threeboxplot}
                \centering
                \includegraphics[width=\textwidth,height=\boxplotheight,trim={.8cm 0 .5cm 0},clip]{ipp_figures/boxplots/Env_D,Deciles.pdf}
                
        \end{subfigure}
        \begin{subfigure}{\threeboxplot}
                \centering
                \includegraphics[width=\textwidth,height=\boxplotheight,trim={.8cm 0 .5cm 0},clip]{ipp_figures/boxplots/Env_D,Quartiles.pdf}
        \end{subfigure}
        \begin{subfigure}{\fourboxplot}
                \centering \includegraphics[width=\textwidth,height=\boxplotheight,trim={.8cm 0 .5cm 0},clip]{ipp_figures/boxplots/Env_D,Extrema.pdf}
        \end{subfigure}
        \caption{\textbf{Simulated AUV planning experiments with real data.} Error between ground truth quantile values and estimated quantile values. Datasets C and D collected from a reservoir in California using an underwater robot with a chlorophyll fluorescence sensor.
        Units are $\mu g/L$ chlorophyll.
        Each dataset and objective function pairing is run three times.}\label{fig:ecomapper_planning_results}
         \vspace{-0.2in}
\end{figure}


\begin{figure}[b]
    \centering
    \includegraphics[width=0.8\columnwidth,height=2.4cm,trim={.2cm .5cm .5cm .5cm},clip]{ipp_figures/coverage/Env_B,Deciles.pdf}
    \caption{Comparison between quantile standard error with POMDP solver and Spiral-STC coverage planner~\cite{coverage} on Drone Environment B estimating deciles, each over 3 trials.}
    \label{fig:coverage_expr}
    \vspace{-7pt}
\end{figure}




\subsection{Informative Path Planning: Objective Functions}
\label{ssec:ipp_experiments}
To evaluate how well our proposed IPP objective functions estimate the ground truth quantile values in real environments, we compare quantile change (\cref{eq:quantile_change}) and quantile standard error (\cref{eq:standard_error}) against a baseline entropy objective function (\cref{eq:entropy}).
For the upper extrema quantiles, we also compare against expected improvement (\cref{eq:ei}), as it is similar to a sequential Bayesian optimization based IPP task.





\subsubsection{Setup}
In the planner, we use $\gamma = 0.9$, and each trial is run over 3 seeds.
The objective $c_{plan}$ parameter is set to the approximate magnitude of the rewards seen for each environment, which we found experimentally to be an adequate value.
The GP mean was set to 0 and the datasets were normalized, while the lengthscale was set to 12. The exploration constant $c_{plan}$ was set to $1E-6$ for quantile change and $1E-2$ for quantile standard error.
To compare the performance of the approaches, we use the RMSE between the ground truth quantiles, $\quantilevalues$, and estimated quantile values after performing a survey, $\estimatedquantilevalues$. 
% We choose this metric rather than, e.g., comparing the error between the estimated concentration $\mu(\gtsensedlocations)$ and the ground truth concentration  $GT(\gtsensedlocations)$ because the objective of the task specifically focuses on getting the highest accuracy for the quantile values, and does not optimize for overall concentration accuracy.


\textbf{Drone with Camera}
The drone is allowed to take 30 simulated pictures out of a grid with about 300 positions. 
Each picture is downsampled to $8\times 5$ pixels ($40$ measurements) with $37.1^{\circ}$ by $27.6^{\circ}$ field of view, similar to the drone used in the field trial reported in \cref{sec:field_trial}.
%At each step, the drone collects $40$ measurements.
While this is downsampled from the true image, it captures the coarse trends of the concentration, which is both still scientifically useful and performant for GP evaluations.
For each trial, the GP is seeded with 100 evenly spaced measurements across the workspace, as prior data. %given by a remote sensor, such as a satellite.
The planner uses $300$ rollouts per step, and the maximum planning depth is 7.
%For quantile change $c=10^{-6}$ and for quantile standard error $c=10^{-3}$.

\textbf{AUV with Chlorophyll Sensor}
The AUV is simulated for 200 steps in a $12 \times 14 \times 2$ grid.
The planner uses $130$ rollouts per step and a maximum depth of $10$.
The GP is seeded with measurements from 50 locations.

\subsubsection{Discussion}
Overall, our results are robust across multiple experimental environments as well as robot sensor types.
We find that planning with the quantile standard error objective function has a 10.2\% mean reduction in median error across all environments when compared to using entropy. 
This shows that an objective function tailored to estimating a set of quantiles will outperform a coverage planner, such as entropy, that would typically achieve low overall error in reconstructing the entire environment model.
The focus of our approach is to estimate the quantiles in a
targeted way rather than to achieve uniform coverage.


\begin{figure}[t]
    \centering
        \begin{subfigure}{\thirdcolumn}
                \centering
                \includegraphics[width=\textwidth,height=\boxplotheight,trim={.8cm 0 .5cm 0},clip]{ipp_figures/PS_boxplots/ecomapper_results_final_Deciles_ps_boxplots.pdf}
        \end{subfigure}
        \begin{subfigure}{\thirdcolumn}
                \centering
                \includegraphics[width=\textwidth,height=\boxplotheight,trim={.8cm 0 .5cm 0},clip]{ipp_figures/PS_boxplots/ecomapper_results_final_Quartiles_ps_boxplots.pdf}
        \end{subfigure}
        \begin{subfigure}{\thirdcolumn}
                \centering
                \includegraphics[width=\textwidth,height=\boxplotheight,trim={.8cm 0 .5cm 0},clip]{ipp_figures/PS_boxplots/ecomapper_results_final_Extrema_ps_boxplots.pdf}
        \end{subfigure}
                \begin{subfigure}{\thirdcolumn}
                \centering
                \includegraphics[width=\textwidth,height=\boxplotheight]{ipp_figures/PS_boxplots/clearlake_results_Deciles_ps_boxplots.pdf}
        \end{subfigure}
        \begin{subfigure}{\thirdcolumn}
                \centering
                \includegraphics[width=\textwidth,height=\boxplotheight]{ipp_figures/PS_boxplots/clearlake_results_Quartiles_ps_boxplots.pdf}
        \end{subfigure}
        \begin{subfigure}{\thirdcolumn}
                \centering
                \includegraphics[width=\textwidth,height=\boxplotheight]{ipp_figures/PS_boxplots/clearlake_results_Extrema_ps_boxplots.pdf}
        \end{subfigure}
        
        \caption{\textbf{Quantile location selection results.} 
        RMSE between the ground truth values at the selected locations and the corresponding true quantile values.
        Units are $\mu g/L$ chlorophyll for AUV, 400nm channel pixel intensity ($0-255$) for Drone.
     }
     \label{fig:ecomapper_ps_boxplots}
    \vspace{-0.2in}
\end{figure}



\Cref{fig:clearlake_planning_results,fig:ecomapper_planning_results} show the results of planning with the proposed objective functions for the drone and AUV experiments, respectively. 
In the drone tasks (A/B),
quantile change and quantile standard error outperform the baseline entropy in estimating the deciles and upper extrema.
In quartiles in environment A, both proposed methods perform well, but in environment B entropy outperforms our methods. 
% We believe this because this specific configuration is the most difficult task as each method performs worse at the end than they do at 5 steps.
For the extrema, both methods perform better than expected improvement, and entropy outperforms expected improvement in environment A. 
We believe this is because expected improvement focuses explicitly on improving the (single) maximal value and does not do a good job of localizing high concentration areas, thus overestimating the quantile values.

For the AUV tasks (C/D),
quantile standard error outperforms entropy in environment C when estimating deciles and quartiles, and performs equally well as entropy in all other tasks besides estimating the extrema in environment D.
Expected improvement performs poorly in estimating the extrema due to similar issues as with the drone.
Quantile change performs poorly in most AUV tasks in contrast to the drone tasks, where it performs comparably. 
This may indicate that quantile change performance decreases with point sensors, or it is more sensitive to variation in the absolute measurement values.
Thus, we recommend using quantile standard error unless there are computational constraints, since its performance is more consistent.

We also compare our approach using the proposed quantile standard error objective function to the Spiral-STC coverage planner~\cite{coverage}. 
\Cref{fig:coverage_expr} shows that the proposed adaptive solution is able to reduce the error between the estimated quantiles and the ground truth quantiles more rapidly than the non-adaptive coverage planner.




\subsection{Location Selection}
To evaluate how close the values at locations suggested by our proposed loss function are to the estimated quantile values, we use the optimization algorithms simulated annealing, cross-entropy, and Bayesian optimization 
with the results from the quantile estimation task (\Cref{ssec:ipp_experiments}) using the quantile standard error objective function.
% CE gamma is eta in this paper to avoid confusion with the planner gamma
\subsubsection{Setup}
We compute the error by $RMSE(\quantilevalues,\estimatedquantilespatiallocations) = \|(\quantilevalues - GT(\estimatedquantilespatiallocations))\|_2$.
We set $c_{select}$ to 15 for deciles, 200 for quartiles, and 30 for extrema.
We compare the results against a Best Visited (BV) baseline which selects the location the robot took a measurement at that is closest to each quantile value, i.e. solve $\estimatedquantilespatiallocations^* = \argmin_{\estimatedquantilespatiallocations_{bv} \subset \sensedlocations} \|\estimatedquantilevalues - \mu(\estimatedquantilespatiallocations_{bv})\|_2$.

For SA, we use $T_\t{max} = 5$, $T_\t{min} = 0.001$, and cooling rate $\t{cr} = 0.005$ which leads to approximately 1000 optimization steps, and reset to the best solution every 100 steps. 
We start the optimization using the solution found by the BV baseline.
For CE, we use $\alpha = 0.9$, $\eta = 0.9$, 50 samples per iteration, and 100 iterations.
$\alpha$ is a weighting factor on new samples, which is used to prevent premature convergence.
For BO, we use the expected improvement acquisition function and initialize the GP with 50 randomly selected $\quantilespatiallocations$s as well as the solution found by the Best Visited baseline.
We use 100 iterations and report the best found solution.

\subsubsection{Discussion}
The error between the values at the estimated quantile locations and the true quantile values for the drone and the AUV experiments can be seen in \Cref{fig:ecomapper_ps_boxplots}.
Overall, we find that cross-entropy and Bayesian optimization produced the locations with values closest to the true quantile values.
Both these methods perform a global search in the space of possible locations, indicating that global search optimizes \cref{eq:ps_loss} more effectively.
Simulated annealing had greater variability in performance.
We believe this is because it is a local search method and may fail to escape local optima.
Best Visited produced a good initialization for the other methods, but was easily outperformed.
We find that CE performs the best in three out of six possible scenarios.
In particular, we see a 15.7\% mean reduction in median error using CE with our proposed loss function compared to the BV baseline across all environments when using our proposed quantile standard error optimization function for quantile estimation during exploration.

In general, methods can find the best points when selecting for quartiles or deciles,
while the upper extrema are more difficult.
Because the robot is limited in the amount of environment it can explore, the upper extrema  are less likely to be measured during exploration.
This leads to these quantiles being more challenging to select representative points for.



\begin{figure}[t]
    \centering
    \includegraphics[trim={0.5cm .5cm 0.7cm 0.9cm}, clip, width=.45\columnwidth]{ipp_figures/clearlake_results_deciles_standard_error_CE_contours_with_heatmap.png}
    %\vspace{-10px}
    \includegraphics[trim={0.5cm .5cm 0.5cm 0.9cm}, clip, width=.45\columnwidth]{ipp_figures/clearlake_results_deciles_standard_error_CE_points_raster.png}
    
    \caption{
    \textbf{Physical locations (stars) selected by the cross-entropy optimizer for deciles on the drone experiment.}
    [Left] Black lines: true quantile value contours, overlaid on the absolute error between $\mu(\gtsensedlocations)$ and $GT(\gtsensedlocations)$. Note that the lowest error tends to follow the quantile contour lines.
    [Right] Red crosses: locations the robot visited, overlaid on the ground truth image.
    }
    \label{fig:contours}
    \vspace{-17px}
\end{figure}


%\textbf{Drone with Camera}
%\Cref{fig:clearlake_ps_boxplots} shows 
%$RMSE(\quantilevalues,\estimatedquantilespatiallocations)$
%for the drone experiments for each of the four point selection methods.

Figure \ref{fig:contours} shows results for one seed of the drone task when monitoring deciles.
The suggested locations, shown as stars, align relatively closely with the true quantile values $\quantilevalues$, shown by the contours on the left image.
This demonstrates the ability of the optimizers to produce good location suggestions to guide environmental analysis.

The right part of Figure \ref{fig:contours} shows the same locations on top of the orthomosaic of what the drone could measure during exploration.
This part of the figure highlights the difficulty of the problem of IPP for quantiles. 
The robot could only explore 15\% of the total environment.
With only partial knowledge of the distribution, the robot's model of the phenomenon will vary based on the particular points it visited, which in turn affects the estimates of the quantiles.
%
%\textbf{AUV with Chlorophyll Sensor}
% \Cref{fig:ecomapper_ps_boxplots} shows
% $RMSE(\quantilevalues,\estimatedquantilespatiallocations)$
% for the AUV experiments for each of the four point selection methods.
% Like in the drone experiments, the suggested locations correspond well to $\quantilevalues$ produced by the planner.
% Here, cross-entropy performs best for both the extrema and the deciles, demonstrating the effectiveness of global search.
%
Similarly, \Cref{fig:3d_points} shows the suggested locations for the upper extrema for one seed of the AUV task.
For both tasks, all the optimization methods, with the exception of Best Visited, suggest points that may be spatially far from locations the robot has been able to visit.
This allows for points with values potentially closer to the true quantile values to be selected for scientific analysis.

\begin{figure}
    \centering
    \includegraphics[trim={1cm .5cm 0.8cm 1.5cm}, clip, width=.65\columnwidth]{ipp_figures/ecomapper_results_final_Extrema_standard_error_CE_real_ps_pointsraster.pdf}
    \vspace{1px}
    \caption{\textbf{Physical locations (stars) selected by the cross-entropy optimizer for the upper extrema quantiles with an AUV using a chlorophyll point sensor.}
    Blue/green points are the measured locations $\sensedlocations$.
    }
    \label{fig:3d_points}
    \vspace{-17pt}
\end{figure}


\begin{figure}[b]
    \vspace{-15px}
    \centering
    %\hspace{-10px}
    \includegraphics[trim={4.3cm 2cm 5.1cm 2.3cm}, clip, width=.75\columnwidth, align=c]{ipp_figures/field_results_labels1.png}
    %\hspace{-10px}
    %\includegraphics[trim={80cm 0cm 20cm 0cm}, clip, width=.27\columnwidth, align=c]{ipp_figures/20210907_144213.jpg}
    \includegraphics[trim={14cm 0cm 4.5cm 0cm}, clip, width=.23\columnwidth, align=c]{ipp_figures/drone-pic.png}
    \caption{\textbf{Visualization of a field trial modeling a crop health task.}
    \textit{Left:} Crosses are locations where the drone took images. The drone is limited to only visit 20\% of the possible locations to take images.
    The quantiles of interest are the deciles and the locations are chosen by cross-entropy.
    The 9 stars show locations suggested to collect physical specimen. 
    The measurement of interest is the amount of green in each pixel. 
    \textit{Right:} The drone used in the field trial, in flight.
    }
    \label{fig:field-results}
    \vspace{-15px}
\end{figure}

\subsection{Field trial}\label{sec:field_trial}
The goal of our final experiment is to demonstrate our method on real hardware for a crop health monitoring task in an open, grassy field, where the objective is to estimate the deciles of the green present in each pixel of the images (we use green as a proxy for plant health).

\subsubsection{Setup}
We use a commercial, off-the-the shelf drone with a standard camera to take measurements of the field at a constant height of 3m. 
Similar to the simulated drone, the drone in this experiment moves in a 2D plane with a north-fixed yaw.
The drone has a limited budget of 20 pictures (planning steps) in a $16\times16$ m square grid, where $|\gtlocations| = 10\times10$ locations, and each picture is downsampled to $8 \times 5$ px.
For planning, we use the quantile change objective function because it performs well for camera sensors and is faster than quantile standard error.
We operate the drone with a custom app and use onboard GPS and IMU for localization.

\subsubsection{Discussion}
Figure \ref{fig:field-results} shows the resulting suggested locations using CE based on the 20 steps the robot took. 
We find that, although the robot cannot explore the entire workspace due to its limited budget, and in fact does not visit a large green area, the system is able to suggest varied locations for specimen collection.
Some selected locations (e.g., those representing the $0.3, 0.4, 0.5$ quantiles) are spatially close to each other, which suggests this area contains a large gradient, or those quantile values are similar.
As the goal is to suggest locations that contain the estimated quantile values, such locations may be near one another.

\section{Conclusion}
% \imr{could cut some of the background/motivation here if we need space}
Scientists traditionally collect physical specimens at locations selected using heuristics.
They later analyze these specimens in a laboratory to characterize a phenomenon of interest (e.g., the distribution of algae in the water).
We propose to, instead, choose these specimen collection locations by first performing an informative path planning survey with a robot and then proposing locations which correspond to the quantiles of interest of the distribution.

To accomplish this, we propose two novel objective functions, quantile change and quantile standard error, for improving the estimates of quantile values through informative path planning. 
We test these in three settings: a drone with a camera sensor over lake imagery, an underwater vehicle taking chlorophyll measurements, and a field trial using a drone for a crop health task.
Our objective functions perform well and outperform information-theoretic and Bayesian optimization baselines. 
In our experiments, our proposed quantile standard error objective function has a 10.2\% mean reduction in median error when compared to entropy.
%as the objective function. 
% We show that quantile change works well on a task where a drone takes samples with a camera and that quantile standard error performs well on both tasks. 

We also show that using our proposed loss function with black-box optimization methods can select environment locations for analysis that are representative of a set of quantiles of interests. 
We find that a cross-entropy optimizer using our loss function outperforms a baseline of using the best measured points,
with a 15.7\% mean reduction in median error in values across all environments.

Our approach can be used to guide physical specimen collection in real field scenarios, as demonstrated by our field trial.
In recent work, we have discovered that some computational cost can be alleviated with a randomized sampling approach when evaluating the GP in the objective functions.
We believe combining that and an approximate GP can improve scalability.
Additionally, experimentally finding parameters was difficult for both the baselines and our proposed methodology, particularly for the GP; this is a direction for future work.
We also plan to incorporate our specimen collection location suggestions into a larger field campaign involving multiple scientists.

